Enabling Personalized Video Quality Optimization with VidHoc

The emerging video applications greatly increase the demand in network bandwidth that is not easy to scale. To provide higher quality of experience (QoE) under limited bandwidth, a recent trend is to leverage the heterogeneity of quality preferences across individual users. Although these efforts have suggested the great potential benefits, service providers still have not deployed them to realize the promised QoE improvement. The missing piece is an automation of online per-user QoE modeling and optimization scheme for new users. Previous efforts either optimize QoE by known per-user QoE models or learn a user's QoE model by offline approaches, such as analysis of video viewing history and in-lab user study. Relying on such offline modeling is problematic, because QoE optimization will start late for collecting enough data to train an unbiased QoE model. In this paper, we propose VidHoc, the first automatic system that jointly personalizes QoE model and optimizes QoE in an online manner for each new user. VidHoc can build per-user QoE models within a small number of video sessions as well as maintain good QoE. We evaluate VidHoc in a pilot deployment to fifteen users for four months with the care of statistical validity. Compared with other baselines, the results show that VidHoc can save 17.3% bandwidth while maintaining the same QoE or improve QoE by 13.9% with the same bandwidth.

==> bwallocation.tex <==
\section{System design}
\label{sec:qoeprofiling}
In this section, we will illustrate \name's design, and other baseline designs.

\subsection{Problem description}
The goal of our system is to learn the user video quality preferences and provide user-specific QoE optimization.
The end-to-end procedure of video streaming services is shown in Figure~\ref{?}.
We can deploy \name on the modules where we can allocate the user's bandwidth, such as the bottleneck link on the ISP side or the CDN server.

The main difference between \name and the previous study is that we are not able to directly control the video quality but use the bandwidth knob to indirectly affect the video quality.
Moreover, we need to minimize the user annoyance when we do the whole user study.
Thus, we monitor the user engagement ratio as QoE instead of soliciting the user rating after each video session for making the users give a more natural feedback, and 

At a high-level, \name has two stages:
\begin{itemize}
    \item[1.] Learn per-user QoE model: For a video sessions, we might need to deliberately add quality issues (\eg low bitrate, rebuffering event) for studying the user's preferences to different types of quality issues.
    \item[2.] QoE optimization: Once we obtain per-user QoE model, we can optimize it by exploiting per-user QoE model.
    In general, we need to avoid the quality issues that the users are sensitive to the concisely.
\end{itemize}


\subsection{Baselines of training per-user QoE models}
Previous studies \cite{??} has shown several methods to train per-user QoE models, but they are not suitable for our cases.

\mypara{No customization}
The most straightforward solution is to observe the user engagement in their daily viewing, and then we train the user's QoE model until the model gets converged.
During the training stage, we do not customize the video quality, and in return, the users are unaware of the training process.
However, the main drawback is that, the video quality of the videos might not contribute too much information for training the QoE model (\ie uncertainty).
It might lead to a very long training process, and it hurts user's QoE since the QoE optimization starts late.

\mypara{Naive Active Learning}
Compare with ``No customization", another extreme is to train the per-user QoE model as soon as possible.
We can use active learning to construct the video quality for each video session, which always make the video quality that can provide the most information for QoE model training.
Although it can train the QoE model much faster, it impairs user QoE seriously, since the video sessions that provide the most information usually have bad video quality.
It might not be acceptable for the streaming service providers, because it would discourage the new users to engage in the service.

In summary, the above straightforward solutions either start QoE optimization late or impair user QoE during the training stage, which are not ideal solutions.

\subsection{Balance video uncertainty and quality}
From the lessons of the straightforward methods, we want the user-perceived video quality to be with large uncertainty and QoE, \ie the possible maximal the sum of video uncertainty and QoE.
To solve this problem, we cast it to a regret minimization problem where we try to minimize gap between the video quality pattern we want to construct and the maximal possible video quality and uncertainty.
For each video session, we construct the video quality pattern that can minimize the regret.
The benefit of such a formulation is that we do not need to explicitly separate the modeling training and QoE optimization stage.
As the per-user QoE model receives more video data samples, the QoE model becomes more accurate so that the contribution of the uncertainty part in the regret is being more marginal. 


% \begin{algorithm}
%  \KwData{QoE model $Q$}
%  \KwData{Uncertainty calculator $U$}
%  \KwData{the quality of downloaded chunks $q_1, q_2, \dots, q_{m-1}$}
%  \KwData{Player behavior profile $P$}
%  \KwResult{Downloading bandwidth of chunk}
%  $\mathcal{B}\leftarrow$ the set of all possible combinations of downloading throughput for the future chunks\;
%  minimal regret, bw plan $\leftarrow 0, Null $\;
%  \For{ $B$ in $\mathcal{B}$} {
%     Possible video quality patterns and probability $\leftarrow$ $P(B)$\;
%     expected QoE $\leftarrow 0$\;
%     \For{$v$ in Possible video quality patterns}{
%          expected QoE $+= v_{prob}*(Q(\{q-1, \dots, q_{m-1}, v_{quality}\}) + U(v_{quality}))$\;
%     }
%     \uIf{expected QoE > minimal regret}{
%          minimal regret $\leftarrow$ expected QoE\;
%     }
%  }
%  \textbf{return} The downloading rating for chunk $m$ in bw plan\;
%  \caption{Determine the downloading bandwidth for the chunks}
% \end{algorithm}
% In this algorithm, the player profile $P$ takes the bandwidth as input, and outputs a set of two-element tuples.
% In each tuple, it has $v_{prob}$ and $v_{quality}$ which represents the video quality pattern and its corresponding video quality.

\subsection{Solve the formulation by bandwidth allocation}
In Section~\ref{sec:moti}, we show that we have XX\% chance to get the desired video quality if we change the bandwidth to the bitrate of the desired video quality.
A straightforward solution is that when downloading a chunk, we always set the bandwidth to the bitrate we want to obtain.
If we do so, the perceived video quality might have much larger regret than we expect!
For example, if we want to provide the QoE model with the information about video quality dropping from 720p to 480p, in practice there is a chance to get a rebuffering event instead of a 360p chunk.
If the QoE model already has the information about rebuffering event, such a video quality pattern cannot contribute the uncertainty and good video quality.

Thus, we need to take the player's behavior into account for bandwidth allocation.
Our idea is to change the objective of our formulation from \emph{finding a video quality pattern} to \emph{finding a bandwidth allocation scheme} that can minimize the \emph{expected} regret.

To profile the player's behavior, we can enumerate all kinds of bandwidth change and record the results.
Or we can directly ask the player's designer for the implementation details.
In this paper, we use the first method for convenience. 

\subsection{Save computational cost}
To calculate the expected regret of a bandwidth allocation scheme, we might need to enumerate all possible video quality patterns under this scheme, which will lead to prohibitive computation cost due to the large number of possible patterns.
To save the computational cost, we have two methods:
\begin{itemize}
    \item Reduce looking-ahead horizon: When determining the bandwidth of a chunkd downloading, we do not need to calculate all possible video quality for its subsequent chunks, we only look ahead the recent video chunks for their possible video quality.
    For the rest chunks, we can assume their bitrate to be the same as the bandwidth of downloading.
    \item Map bandwidth allocation directly to QoE: A more aggressive cost-saving method is to build a per-user QoE model which takes the bandwidth allocation as input and output the user QoE prediction.
    Although it do not need to enumerate the possible quality patterns, the drawback is also obvious: the QoE model is player-specific which means a user might different QoE models for different players.
\end{itemize}


==> discussions.tex <==
\xu{
\tightsection{Discussion}

\tightsubsection{Extend \name to ABR algorithm}

We can also extend \name to the adaptive bitrate (ABR) algorithm built in the video players.
Different from bandwidth allocation that has full control over the network bandwidth in \name, ABR algorithms need to make the bitrate selection decision based on the predicted network throughput.
In this case, \name first calculates the video quality sequence with the minimal regret (\ie the maximal sum of the quality and the uncertainty of this sequence) under the predicted by quality pattern.
If \name fails to achieve the desired video quality for a video chunk due to the inaccurate network bandwidth prediction, it recalculates a new video quality sequence to minimize the regret regarding the downloaded video chunks.
We did not implement it in this paper, because YouTube does not open their APIs to change the default ABR algorithm.

\tightsubsection{Model drift}

Throughout the user study, we assume that users' QoE models are stationary, \ie no ``model drift'' during the months of our tests.

We admit that a user's QoE preferences might change during the period of user study.
The possible reasons could be 1) the video viewing context factors, such as video viewing devices and UI~\cite{?}; 2) different video content~\cite{?}.
The model drift problem might cause \name as well as other benchmarks (in \ref{?}) that also leverages per-user QoE model to optimize QoE to be suboptimal.

To mitigate the negative effect caused by model drift, we first make sure the users were using the same device throughout the user study and no significant change in UI (See Appendix~\ref{?}).
For the impact from the video content, unfortunately we are not supposed to have the video content due to the user privacy agreement in our user study, and not able to build per-user QoE model for every type of video content like~\cite{zhang2021sensei}.
But it is still a fair comparison for \name and other benchmarks in~\ref{?} in evaluating their performance.
We use the randomized A/B test to randomly assign the video content to \name and other benchmarks, and thus, the per-user QoE models built in \name and other benchmarks are biased by the training set,  because their training sets have the similar distributions of video content.
}

==> imple.tex <==
\section{Implementation}
\label{sec:impl}

In this section, we introduce the methodology of user study in \name (\S\ref{sec:impl:meth}).
Then, we illustrate the browser extensions that can monitor video quality and control user bandwidth by rate limiting~(\S\ref{sec:impl:plugin}).

\begin{figure}[t]
	\centering
	\includegraphics[width=1.0\linewidth]{graphs/graph/user_study.pdf}
	\caption{Procedure of user study: In the pre-screening test stage, we first send out the questionnaire to crowd workers, and verify their answers by monitoring their video quality. In the next stage, the eligible users are required to install our video quality monitor and bandwidth controller on their browser to evaluate \name.}
	\label{fig:user_study_overview}	
\end{figure}


\begin{table}[t]
\begin{tabular}{l|l}
 \hline
 Gender&  7 female, 8 male \\
 \hline
 Age & 4 of 21-29, 8 of 30-39, 3 of 40+ years old  \\
 \hline
 Internet plan & 12 of 25Mbps, 3 of 50Mbps \\
 \hline
\end{tabular}
\label{tab:userstats}
\vspace{1em}
\caption{User stats}
\end{table}

\subsection{User study methodology}
\label{sec:impl:meth}

In \name, it is hard to compare \name and other baselines, because we cannot control the video content and watching time of the users. 
Since the network condition might vary over time, To make a fair comparison, we make sure the sessions of \name and other baselines have the same average bandwidth.
We set the average bandwidth as $60\%$-fraction of its maximal bandwidth during those video sessions, because we cannot actually increase the user's physical bandwidth.
To mitigate the influence from video content (which are unknown to us), we borrow the idea from A/B test\cite{?}: We randomly determine which strategy we use to optimize QoE when each video session begins.

We test \name and other baselines on the users recruited from two popular crowdsourcing platforms, \ie Amazon Mechanical Turk~\cite{?} and Prolific~\cite{?}.
Figure~\ref{?} shows the procedure of conducting user study to evaluating \name on real human users.
The our user study has two stages:

\mypara{Pre-screening test}
This stage is for recruiting the participants in our study.
First, we publish a questionnaire on the crowdsourcing platforms to solicit the age group, gender, internet plans, frequency of watching online videos, and frequency of suffering quality issues from the potential participants.
The eligible participants should use video streaming services more than $\geq$ XX hours per week and suffers from quality issues frequently, because we have the room to improve their experience.
For evaluate \name on different population, we make sure the participants' diversity in gender and age as in Table~\ref{?}, which are similar to the demographics of YouTube users~\cite{youtubestats}.
To avoid the dishonesty feedback in the questionnaire, we also require the users to install the video quality monitor (See~\S\ref{sec:impl:plu}) on their browser and then confirm their answers in the questionnaire.

\mypara{Strategy evaluation}
In this stage, for evaluating \name, the select users are required to install a browser extensions to report the metrics of their video sessions, including video quality (resolution, rebuffering events), player status (player progress slider, buffer length, etc.) and video session time.
Different from the previous study, to minimize the user annoyance, we observe the video session time as QoE instead of soliciting user feedback by an exit survey that would take tens of seconds for each video session~\cite{?}.


\subsection{Client-side browser extension}
\label{sec:impl:plugin}

In this paper, we only test \name when the users watch YouTube videos. 
We strictly follow the settings in \S\ref{?}: we do not change the user interface (UI) of the video streaming service, the users can freely choose their video content to watch for providing us a more natural feedback, and we do not collect the information about video content.

\mypara{Video quality monitor}
We monitor video quality and video session by appending JavaScript codes to the YouTube webpage.
The appended codes have the access to the objects in the webpages.
Thus, we can access the YouTube player object for extracting video download resolution, playback rate, volume, player slider bar progress by XXX, XXX, and XXX APIs provided by YouTube developers.
But, YouTube does not offer video buffer length information.
To solve this problem, we cast the object of YouTube player to a HTML5 player where we can call its API XXX to read the ranges of the video covered by the buffer.

The length of the video session is calculated the time spend from video session start to the video ends or the session closed (which comes the first).
Since the users are not in a controlled environment, we do not know the user status when the users watch videos.
To make sure they do watch the videos, we also monitor the browser status, \ie whether the browser is on the top of desktop, and whether the video player tab is show up on the top of the browser.
We only use the videos that the users put the browser on the top of the desktop and the video player tab on the top of the browser to train per-user QoE models, because other videos might not reflect the user preferences to the video quality.

This monitor reports to the \name server every XXX seconds in our implementation.
Each report is only XXXKb, and does not introduce too much traffic to \name's server.



\mypara{Dynamic rate limiting}
We limit the video downloading rate by delaying the HTTP requests whose destination is the video player.
When the HTTP requests arrive at the user client, the bandwidth controller holds the request until it meets the requirement of bandwidth throttling by XXXX API provided by Google Chrome browser.
The time length that the controller needs to hold for a target bandwidth is
\begin{align}
	hold\_time &= \frac{size}{target\_bw} - \frac{size}{real\_bw}\notag,
\end{align}
where $size$ is the data size of the HTTP request, $target\_bw$ is the bandwidth we want to achieve, and the $real\_bw$ is the current real bandwidth of the user.
Although we cannot obtain the ground truth of the real bandwidth, we estimate it as the real bandwidth of the last HTTP request.

Another question is how to determine the hold time of the HTTP requests.
The hold time should make sure the target bandwidth the same as the video bitrate.
To obtain the video bitrate, we can parse the headers of the videos that are mostly using fragmented MP4 format~\cite{?}.
In fragmented MP4, the SIDX field in the header has the byte range of each video chunk in the video streaming, and we can use it to calculate the video bitrate.
We can download the video header for every resolution video source to calculate the bitrate of each version of the video streaming.


==> outlines-short.tex <==

% Motivation

\section{Introduction}

\section{Motivation}
In this section, we show 1) the QoE preferences are different across the users; and 2) such a difference is on par with other factors such as video content and viewing devices.

\subsection{Dataset and method}

\subsection{Measuring user heterogeneity}

\subsection{Summary}

% VidHoc design

\section{Design of VidHoc}
We introduce 1) How to train per-user QoE model; 2) VidHoc implementation regarding the inaccurate control over the video bitrate by throttling bandwidth.

\subsection{QoE model training}

\subsubsection{Framework}
The framework of per-user QoE modeling is in Figure~\ref{fig:online-framework}.
This framework contains a logical controller (which could be operated by a service provider or by the player) that determines the video quality during each video session.
At the same time, the controller monitors the QoE (defined shortly) of each session and uses the measurements of QoE (subjective) and the video quality (objective) from each session to update the per-user QoE model maintained by the controller.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{fake_graphs/online-framework.pdf}
    \caption{Framework of online QoE modeling and optimization.}
    \label{fig:online-framework}
\end{figure}

\subsubsection{Requirement of Per-User QoE Modeling}
To make this framework be deployable in the wild, the per-user QoE modeling needs to meet the four properties:
\begin{itemize}
    \item P1: No control on when \& what the user watches
    \item P2: Fast modeling
    \item P3: High QoE during modeling
    \item P4: Accurate per-user QoE modeling
\end{itemize}

Lab-based study cannot meet P1; Offline analysis cannot meet P4, so we need online solutions.
Two strawman online methods.
\mypara{GreedyProfiling} It utilize active learning to construct the video quality pattern that can maximize P2.
It violates P3, so that it might discourage the users to watch the videos.

\mypara{GreedyOptimization} We always use the up-to-date QoE model to optimize the video quality, and update the QoE model after every video session.
It violoates P2 and P4, since we cannot detect some user preferences by adding extra quality issues.


\subsection{VidHoc implementation}

\subsubsection{Setting}
We put VidHoc in the following settings
\begin{itemize}
    \item We do not control video content.
    \item Use user engagement as a metric: The user can freely watch any video they like.
    It is widely-used in the industry. It is cheap and less annoyance compared to collectign user rating. Although it can be affected by many other factors (\eg video content that the users like, video viewing device that stays the same throughout the study period, etc.), we try our best to keep those factors the same in our study, and previous work shows the strong correlation between it and the perceived video quality.
    \item We change the bandwidth to change the video quality, and other than the quality, nothing is affected, such as UI, player setting (vol, playback rate)
\end{itemize}

This setting fits for ISP/CDN/etc. that can control the bottleneck link of the video. transmission.


\subsubsection{Dynamic quality scheduling}
The goal of \name is to maximize both the training speed (measured by uncertainty) and the video quality during training.
\begin{align}
    \max& \quad\quad QoE(v_i)+Uncertainty(v_i), \label{eq:find_patter}\\
   \text{s.t.}&  \quad BandwidthUsage(v_i) < BandwidthLimit\label{eq:bt_limit},
\end{align}
$QoE(v_i)$ is the predicted QoE of the video quality pattern $v_i$, $Uncertainty(v_i)$ is the uncertainty of this prediction, which indicate the training speed, the larger uncertainty per training video pattern, the faster speed of model training, the $BandwidthLimit$ is the pre-determined maximum average bandwidth per session (\eg this can be based on the Internet plan subscribed by the user), and $BandwidthUsage(v_i)$ is calculated by dividing the sum of bitrates of expected watched chunks (the ones within the predicted viewing time $QoE(v_i)*VideoLength$) by the predicted viewing time.

\mypara{Challenges} However, we cannot accurately control over the video bitrate. So what if we get the undesired video quality pattern (this pattern might have low QoE and/or low uncertainty)?

\mypara{Dynamic rate limiting}
To mitigate the problem caused by the inaccurate control over the quality, We need to take the chance of the failure of getting the desired video quality pattern.
We choose the bandwidth allocation plan instead of the video quality, and this plan can maximize the expectation of the sum of QoE and uncertainty.

To get the expectation, we build the profile of the player, and the profile can help us calculate the chance of getting the undesired video quality patter.
Figure~\ref{?} show two examples, where we want to increase the video quality from XXX to XXX, and decrease video quality from XXX to XXX.
It shows that, for more than XXX\% cases, we can still get the desired video quality pattern.

Also, even if we get the undesired video quality pattern, it is still acceptable.
If the resulted video quality pattern has small uncertainty, it is still better that GreedyOpt that does not interfere with the video quality at all.
Because, \name creates more bandwidth fluctuations, and thus there would be more quality issues than GreedyOpt in the video quality patterns, which also leads to a faster training speed than GreedyOpt.
If the resulted pattern has the bad quality, it still has better quality than GreedyOpt.
It happens when we expect a slightly lower quality but get a much worse quality level, \eg we expect a small bitrate degradation but get a large bitrate drop or even a rebuffering event.
In this case, \name could re-calculate the bandwidth allocation plan and allocate more bandwidth to the following chunks for a better regret, and the more bandwidth will lead to a better video quality.
One might concern that the player might not increase the bitrate adapting to the increased bandwidth.
Fortunately, it rarely happens because the goal of the players is to maximize QoE in which bitrate is an important factor.
The previous work \cite{?} (Understanding video streaming algorithms in the wild
) shows that although some ABR algorithms used in industry have a conservative choice on bitrate selection, it will still increase the bitrate for adapting to the bandwidth.


We can reduce controller compute overhead by 1) a short-look ahead horizon; and 2) we coalesce multiple consecutive chunks as longer segments

% User study methodology
\section{User study methodology}

\subsection{Procedure of user study}
We recruit the participants from Prolific and MTurk.
The users are all from US, and diverse in terms of age and gender.

We first published a filtering survey for the pre-screening the users.
The users should watch YouTube and suffer from quality issues frequently.
We then do a fact check by installing a browser extension to monitor their video quality.

We conducted this user study from September to December 2021 on 6 users from Amazon Mechanical Turk and 9 users from Prolific.
Payment is $\$$10 per hour.

\subsection{How to compare different schemes}
for different schemes, the users should watch the videos under the same context, \ie video viewing device and player setting.
Our browser extension can monitor those context factors, and we make sure those schemes were using the same context.

Randomized A/B test: it can mitigate the influence from the video content.

One concern is the model drift that is caused by the QoE preference change during our study.
It does exist, but it still much smaller than the difference between the users.

Implementation limitation: During our user study, we need to use the browser extension to maintain the same level throughput of all video sessions. VidHoc and other bandwidth allocation baselines need the capability of both increasing and decreasing the network bandwidth to affect the video bitrate. Using a 100\% of bandwidth will limit our operation in increasing bandwidth.
So, we use a 60\% throughput capping. It can also help us maintain the average bandwidth within [XX, XXX]Kbps.




% Evaluation
\section{Evaluation}


==> outlines-short_v2.tex <==
% \input{short_intro}
% \input{short_intro_v3}
\input{short_intro_v4}
% \input{short_motivation}
% \input{short_framework}
\input{short_relatedwork}
\input{short_framework_v5}
% \input{short_qoeprofiling}
\input{short_qoeprofiling_v3}
\input{short_eval}




==> outlines.tex <==
% Contributions:
% High-level: We AUTOMATE the whole process.
% Tech-level: Cast it to regret minimization
% 
% Motivation:
% Dataset: simply introduce the data records.Point to implementation for more details
% motivation should have some design points??
% expectation to our system: what information we need?
% Cross datasets validation： waterloo/netflix etc.
% potential gain should have two aspects: 1) the same bandwidth, different the 
% +subsection about summary
%
% System design
% 3.1 should have more settings + where we should put our model (maybe it should be in motivation section?) + who should use this model? + user study tool? (impl section)
% 3.3 should be our idea: introduce regret minimization
% find a place to say different settings compared with previous study
% what players can we work? what we cannot?

\section{Motivation}
\subsection{Users differ in quality preferences}
\begin{itemize}
    \item Dataset: The records in the dataset(s) should have the video quality and the corresponding user's quality rating. We use LSTM-QoE, Waterloo-SQOE4, Sensei, and the dataset we collected. The details about our dataset collection are in Section~\ref{sec:impl}. 
    
    \item The variance of the user sensitivity to the same quality quality is large. Show the users two videos: one is with a quality issue, the other is without this issue. For a user we regard the difference in the QoE of the two videos as the user's sensitivity to this quality issue.
    
    \item Users also have different sensitivity to the same type of quality issue but in different places of the videos.
    
    \item The variance of user difference in quality preference is on par with that of other well-know factors (\eg viewing device, video content).
\end{itemize}


\subsection{Controllability of player by bandwidth}
\begin{itemize}
    \item We learn the user preferences by the user reactions to the videos with different video quality.
    \item We use bandwidth allocation to control the video quality, and it is suitable for network providers, \eg ISP, CDN etc.
    \item Show the probability that we can get the desired video bitrate
    \item Show how much time the player need to adapt to the bandwidth change
    \item In summary, we have XX\% probability to get the desired video quality within XX seconds.
\end{itemize}

\subsection{Potential gain}
\begin{itemize}
    \item Methodology: Use what-if analysis to show the performance gain. Suppose the ground-truth user preference is the QoE model that we train from all the user's data. Under a small bandwidth range, we calculate the gap between the user's QoE (real QoE) and the maximal possible QoE from the eligible video viewing traces (estimated from QoE model).
    \item Show potential gain of QoE.
    \item show potential BW saving.
\end{itemize}


\subsection{Summary}
\begin{itemize}
    \item The differences in video quality preferences are large across users.
    \item Although we are not able to directly control the resolution of every chunk in video player, the video player is controlable.
    \item We have XXX\% improvment in QoE, and XXX\% bandwidth saving
    \item The system we need: Automatically learn user preference and optimize video QoE by changing bandwidth allocation throughout the whole video session.
\end{itemize}


\section{System design}

\subsection{Problem description}
\begin{itemize}
    \item System settings: Learn user preference and optimize user QoE by changing bandwidth. Show the part we are focusing on in the end-to-end video streaming procedure. Different from the previous study (waterloo, netflix, lstm-qoe, etc), we do not directly control the video quality, monitor engagement ratio instead of collecting user rating.
    \item Our implementation (compromised): Throttling user bandwidth on their client. They are allowed to use 60\% bw of their total bandwidth from their first day in our study. More details see Section~\ref{sec:impl}
    \item Objective: We need to train per-user QoE model (training stage), and then optimize the bandwidth allocation by deploying those models. We want to optimize the summed QoE of videos in the training and the optimization stages.
\end{itemize}

\subsection{Baselines}
\begin{itemize}
\item baseline 1: a uniform 40\% bandwidth throttling (with existing ABR) in the training stage + optimization stage starts after we get the per-user QoE model. Cons: no customization, the training stage takes too long to converge.
\item baseline 2: active learning-based bandwidth throttling (with existing ABR) + optimization stage starts after we get the per-user QoE model.
Aggressively find the most uncertain quality pattern and profile it in the training stage. Pros: a highly accurate customized model. Cons: it will result in very bad video quality in the training stage. Show a graph: baselines 1 vs 2 for their performance in their training and optimization stages.
\item based on 1 and 2, one can think of a naive compromise: always optimize QoE by the current form of the QoE model, and the QoE model will be updated after every video session. pros: good QoE in the beginning, no need to separate the training the the optimization stages. Cons: it still takes too long to converge so that the QoE is usually suboptimal. 
\item summary: what seems to be missing is a way to balance the achieving high perceived quality and obtaining more information to customize the qoe model. 
\end{itemize}

\subsection{Our idea}
\begin{itemize}
    \item Balance video quality and uncertainty. Uncertainty is the information gain to the QoE model training. Larger uncertainty usually means lower quality.
    \item We cast this problem to regret minimization. Regret equals to the maximal possible QoE minus the QoE we get through multiple sessions. We minimize $Max\_possible\_QoE - (uncertainty + QoE)$ (the same as maximize $uncertainty + QoE$) for each video.
\end{itemize}


\subsection{Solution to the formulation}
\begin{itemize}
    \item Strawman method: We change the bw to the desired bitrate of the video chunk when we download this chunk. Cons: the player cannot always adapt the video bitrate to the immediately after the bw changes, so we might get some videos that are with bad video quality but no information gain to the QoE video. Show an example of this.
    
    \item We should consider the player's behavior into our formulation. Change our goal to find a bandwidth allocation plan that can maximize the expected uncertainty + QoE for all its possible video quality patterns. Suppose we have an accurate player profile, then the possible video quality patterns and their corresponding probabilities can be calculated by the player profile.
    
\end{itemize}

\subsection{Save computational cost}
\begin{itemize}
    \item Method 1: Reduce the number of possible video quality patterns by looking fewer chunks ahead. The number of all possible video quality patterns is prohibitive given a bandwidth allocation scheme. We don't need to take all of them into account, and we can only look a few chunks in the future and assume the rest chunks with the desired quality.
    \item Method 2: Build a QoE model that directly bandwidth allocation plan to the QoE. Pros: Avoid using player profile, Cons: we are not able to change bw allocation plan in the middle of transmission, so that we cannot respond to the user behaviors \eg skip to some place (usually with buffer clearance).
\end{itemize}

\section{Implementation}

\subsection{User study}
\begin{itemize}
    \item Pre-screening period: We select the users who watch more than XXX min videos a day, and suffer quality issues frequently.
    \item Minimize interference: No pop-up windows, No change on the YouTube UI.
\end{itemize}

\subsection{Video quality monitor}
\begin{itemize}
    \item What we are monitoring: resolution, buffer length, player slider bar
    \item How to achieve it: Inject the codes into the YT player. Report to the quality data to our server every XX seconds.
\end{itemize}

\subsection{Bandwidth controller}
\begin{itemize}
    \item How to control bandwidth: Control the bandwidth by delaying the HTTP packets between the YouTube server and the user client. We need to put bandwidth controller and video quality monitor into two separate extensions, because the browser extensions are usually with a single thread so that if we put them together, the video quality report will also be delayed.
\end{itemize}

\section{Evaluation}

\subsection{Experimental settings}
\begin{itemize}
    \item Data collection: A/B testing for all baselines.
    \item Baselines: The baselines in Section 3. Our algorithm: our formulation solution w/ w/o method 2 in save computation cost.
    \item QoE metric: Video session engagement ratio.
\end{itemize}

\subsection{Overall performance}
\begin{itemize}
    \item Compare the QoE gain of our algorithm with those baselines under the average bandwidth. We use real engagement data from the users.
    \item Compare bandwidth saving of our algorithm with those baselines under the same QoE. We use the real user engagement data.
\end{itemize}

\subsection{Understanding the QoE improvement}
\begin{itemize}
    \item User's available bandwidth vs QoE gain: If a user always has large bandwidth, we don't have gain. Because this user can always watch perfect video.
    \item Difference between average QoE model and per-use QoE model vs QoE gain: If a user's preference is very similar to the average user, we will not have performance gain (baselines 1,2,3 will get per-user model very fast).
\end{itemize}

\subsection{Microbenchmarks}

\begin{itemize}
    \item Number of future chunks we look ahead in the future vs QoE gain: Use simulation. Regard a user's QoE model as the user's real QoE.
    \item Player status guess error vs QoE gain: We add a random noise on the player's state, then use simulation to show the impact.
    \item Baselines 1 and 2: Size of the training set vs QoE gain: Use simulation
\end{itemize}

\subsection{Cost}
\begin{itemize}
    \item Computational cost in the client
    \item Computational cost in the server: How many users we can sustain concurrently?
\end{itemize}


==> qoeprofiling-v2.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\section{Design of \name}

So far we have shown that there is substantial user heterogeneity in QoE.
Now, several previous efforts have proposed QoE optimization (ABR logics and bandwidth allocation) that take advantage of {\em known} user preferences.
% and optimize bitrate adaptation based on given per-user QoE models.
However, they are unable to quickly start the per-user QoE optimization for a new user before sufficient measurements are accumulated to model user's unique QoE preferences.
To bridge the gap, we present \name, a new bandwidth-control system that {\em online} builds the per-user QoE model for each new user and optimizes their QoE.
In this section, we describe the problem formulation of \name (\S\ref{?}), then discuss two important baselines that illustrate the key challenge underpinning \name (\S\ref{?}), and present \name's QoE profiling and optimization algorithms in (\S\ref{?}).

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{fake_graphs/method_compare.pdf}
    \caption{.}
    \label{fig:ideal-timeseries}
\end{figure}



% - framework of online qoe modeling: set qoe, get qoe feedback
% - four requirements
% - design space => design point
% - how we set quality
% - how we handle player uncertainty


\subsection{Problem formulation}

\begin{table*}[]
% \footnotesize
\begin{tabular}{ccccc}
\hline
 & \begin{tabular}[c]{@{}c@{}}{\bf Q1:} No control on when \\ \& what users watch\end{tabular} & \begin{tabular}[c]{@{}c@{}}{\bf Q2:} Fast (min \# of \\ profile videos)\end{tabular} & \begin{tabular}[c]{@{}c@{}}{\bf Q3:} High QoE \\ during profiling\end{tabular} & \begin{tabular}[c]{@{}c@{}}{\bf Q4:} Accurate per-user \\ QoE model\end{tabular} \\ \hline
Lab study~\cite{??} &  &  &  & \ding{52} \\ \hline
Offline data analysis~\cite{gao2020personalized} & \ding{52} &  & \ding{52} & \ding{52} \\ \hline
No intervention~\cite{??} & \ding{52} &  & \ding{52} &  \\ \hline
Active learning~\cite{chang2018active} & \ding{52} & \ding{52} &  & \ding{52} \\ \hline
Greedy optimization~\cite{??} & \ding{52} &  & \ding{52} &  \\ \hline
NetVideo (ours) & \ding{52} & \ding{52} & \ding{52} & \ding{52} \\ \hline
\end{tabular}
\vspace{0.4cm}
\caption{}
\label{tab:comparison}
\end{table*}


Given that QoE heterogeneity exists across users and there are ABR algorithms to leverage it once per-user preference is known, our goal is to build QoE model in an {\em online} fashion for any new user as quickly and efficiently as possible. 
We refer to this objective as {\em online per-user QoE modeling and optimization}.


\mypara{Online per-user QoE modeling and optimization}
In modeling the QoE preferences for each user, an ideal solution should meet four properties:
\begin{packeditemize}
\item {\bf Q1:} It should not control when and what users watch, since real network service provider (CDN, ISP) or content providers are unlikely to specify what videos users must watch. 
\item {\bf Q2:} It should finish QoE modeling within a minimum number of profiling video sessions, because service providers want to optimize each of their users as early as possible. 
\item {\bf Q3:} It should provide high QoE during while profiling the per-user QoE models, for the same reason as Q2 that service providers want to maintain high user experience throughout. 
\item {\bf Q4:} Finally, we want the eventual per-user QoE models to be accurate enough for per-user optimization techniques (ABR logics and bandwidth allocation) be best leverage the heterogeneity across users.
\end{packeditemize}

Table~\ref{tab:comparison} puts existing techniques designed for different yet related purposes into the context of these four dimensions. 
First, many previous QoE research based on controlled lab studies or crowdsourcing surveys


minimal negative impact on user QoE  (in terms of the number of sessions and their quality before we start to customize the QoE optimization of a new user).
This enables per-user QoE optimization to start as soon as per-user QoE models are sufficiently accurate. 
% online per-user QoE modeling with minimum negative impact on QoE , and
% 2) initiating per-user QoE optimization based on the latest per-user QoE model.
% the per-user QoE model to start QoE optimization early.
Figure~\ref{fig:ideal-timeserie} shows a desirable behavior of \name (blue line): 
For each user, the quality and QoE measurements of each video session will be used to update the user's QoE model, and over time, the QoE model will become more accurate such that future video sessions can leverage the latest per-user QoE model to improve quality over the baseline (grey) that is agnostic to per-user QoE preferences. 
% increasing a user's QoE with the up-to-date per-user QoE model that is updated after each video session.

Our objective of online QoE modeling and optimization entails two unique aspects.
First, our system should not intervene what and when users watch. 
This is in contrast to the prior work~\cite{??,??} that models QoE in controlled environments (\eg watching videos with same content but a range of different video quality levels). 
It is impractical for real video services or network service providers to model their users by deliberately lowering their video quality.
Second, our system should minimize the number of sessions needed to build accurate per-user QoE models.
This is in contrast to the prior work~\cite{??,??} that models user QoE by first collecting a large dataset of QoE measurements (\eg \fillme samples per user in~\cite{??}) and then offline analyze them to build QoE models.

% Existing solutions are ill-suited for the objective of online per-user QoE modeling and optimization. 


% To put it in context, our objective is different from the prior proposals~\cite{??,??,??} that model QoE by letting users watch {\em curated} videos in controlled setting (lab study).


\begin{figure}[t]
    \includegraphics[width=1.0\linewidth]{fake_graphs/end-to-end.pdf}
    \caption{Deploying \name to a video streaming system: \name collects the player status from the client, including video session time, resolution, buffer length etc., and learn per-user QoE model. The bandwidth capping module uses the per-user QoE model to allocate the bandwidth to the client for either training per-user QoE model or optimizing video QoE.}
    \label{fig:e2eprocedure}
\end{figure}

% Different from prior works~\cite{?}, \name's per-user QoE modeling and optimization purely goes online, where the users can watch the videos with any content any time.
% For the new users, we are not able to let them stay in a highly controlled environment (\eg stay in the same environment, watch a set of videos with fixed content, etc.), so that the lab-based user study~\cite{?} cannot be applied to train per-user QoE model.
% Although some works~\cite{?} can model user QoE by offlinely the data collected in the wild, they usually take long time to collect user data (\eg XXX videos in \cite{?}), and start QoE optimization much late.


\mypara{Setting of \name}
In this paper, we study how to realize online QoE modeling and optimization in a specific setting (depicted in Figure~\ref{??}) that makes two practical assumptions (we will describe how we implement this setting in \S\ref{sec:impl}).
First, to minimize the user annoyance, we use user engagement (\ie the ratio of the video viewing time and the video length) as the QoE metric.
Unlike user quality ratings (used in many prior proposals), the video engagement can be collected passively, while the quality ratings must be given manually by users in an exit-survey (during or after each video session).
Second, we do not control the video content or directly change the behavior of the video player. 
Instead, \name passively monitors the player status (\eg video resolution, buffer length, etc.) to infer the video quality which can be used to train per-user QoE model with video engagement.
It then dynamically controls the available bandwidth to indirectly control the video player's performance. %instead of directly control the module of deciding downloading video bitrate in the video player.
% Finally, we can use the per-user QoE models to optimize the QoE of individual users by controlling bandwidth.

This setting is particularly compatible with the network service providers, such as ISP, CDN, and edge routers, who controls the bottleneck bandwidth of a user. 
The network service providers do not have the access to the video player's logic but can control the users' network connection.
Our evaluation results show potential benefits to theser service providers in practice: \name can improve QoE (user engagement) at the same average bandwidth or save bandwidth to achieve the same QoE (\ie if \name is deployed on the bottleneck link, it might support more concurrent users).
% can be deployed on the bottleneck link to support more users.

That said, there are two natural concerns with this setting. 
First, are user engagement measurements from arbitrary video content reliable enough to model per-user QoE?
Intuitively, video content does impact users' sensitivity to video quality, but if the quality level and video content are independent, then sufficient data at each quality level
The independency between content and quality may not always hold, but we empirically find it has a marginal impact. 
To show it, 
% One immediate question of deploying \name to network providers is how to learn per-user QoE model without knowing the video content?
% Although video content has great impact on engagement (\eg the users might end the video session early if the content is not interesting), we argue that the ranking of sensitivity to two different low-quality issues is consistent across different video content.
% It means that for two types of low-quality issues with different sensitivity, our priority is to avoid the sensitive one even if we have to trade another off.
% To prove this, 
for instance, we can use a Z-test~\cite{?} to calculate the significance of the following statement: 
\jc{write down clearly the z-test statement and the z-test results}
% the distributions of the QoE drop caused by the rebuffering event and the bitrate drop should be different should be significantly different

% a user is more sensitive to a type of low-quality issues than another type.
% For example, for a user who is more sensitive to a 1-second rebuffering event than a 500Kbps bitrate drop, the distributions of the QoE drop caused by the rebuffering event and the bitrate drop should be different should be significantly different, \ie how large the overlap of two distributions is.
% \xu{need revise}
% The Z-score is XXXX which shows that the users have sensitivity to the two low-quality issues across different video content.
% We also examine the users who are more sensitive to low-bitrate or bitrate-switch issues than other low-quality issues, and the conclusion also holds.

Another natural concern is how service providers obtain the video quality.
Fortunately, there are existing techniques to infer video quality by the video streaming traffic \cite{?}.
We can use the session time of the video streaming as the engagement, and can guess the player status with XX\% accuracy. 
We evaluate the impact of the player status inference accuracy and the QoE gain of \name in \S\ref{?}.


\mypara{Components} 
Based on the setting, we envision \name has three modules as shown in Figure~\ref{?}:

\begin{packeditemize}
\item {\em Video quality scheduling:}
For each video session, \name first determines the {\em quality pattern} (\ie the quality of each video chunk) of the session.
Ideally, the QoE measurement from the chosen quality pattern would improve the accuracy of the QoE model, and quality pattern itself should induce decent QoE. 
% For each video session, \name needs to schedule its bandwidth for obtaining the video quality pattern (\ie the quality of each video chunk) to maximize the information contributing to QoE modeling and maintain high QoE.
% This module takes the player status (\eg video resolution, buffer length) and the video engagement as the input to train per-user QoE model.=


\item{\em Dynamic rate limiting:}
Once the video quality pattern is determined, we then need to decide how to dynamically set available bandwidth to realize the quality pattern.
% by limiting the user's video downloading rate.
Ideally, if the video players can rapidly adapt to the downloading rate, we can set the rate as the bitrate of the video quality we want.
% However, in practice, the behavior of video player is more complicated: the video bitrate selection decision can be affected by many factors, such as historical bandwidth, current video resolution, and player buffer length\cite{?}.
% The difficulty is that the player behavior is usually unknown to \name's bandwidth controller, and we might not be able to obtain video quality pattern we have scheduled.
% We deal with this difficulty in Section~\ref{?}.

\item{\em Per-user QoE model:}
Finally, the measurements of engagement and video quality from each user are fed to update the user's QoE model.
% Following the practice in previous works~\cite{?}, we use a random forest to train per-user QoE model.
Since the design of the QoE model itself is not our contribution, we reuse a random-forest-based QoE model from prior work~\cite{?}
and use per-user QoE meausrement data to train the model for each user.\footnote{
In particular, the QoE model works as follows. 
This model takes the video quality as the input variables, and outputs the expected QoE as the output.
The input variables are the video quality of the chunks.
Based on the QoE model we currently have and the video trace, we can decide the video quality pattern to show the users.
We customize feature selection and criteria at the nodes on each decision tree inside the forest.
To train the QoE model faster, the initial QoE model is a one-size-fits all model.
To avoid the explosion of input due to the large number of video chunks, we divide the video into XX parts, and QoE model will take the quality of each part.
The total number of input variables are XX * 3 = XX.
The video quality of each part includes its average video bitrate, total bitrate switch, total rebuffering time.
The output is the user QoE.
The QoE is bucketized the user engagement into XX classes, and the output is the class who gets the most votes from the decision trees inside the random forest.}


\end{packeditemize}

In the remaining of this section, we will explain the challenge facing quality scheduling in \name (\S\ref{??}) and how we address it (\S\ref{??}), before describing the rate limiting module (\S\ref{??}).





\subsection{Why is per-user QoE modeling challenging?}
To highlight the challenge, let us consider two seemingly natural designs (which are inspired by prior work).
For now, we assume that \name has the direct control over the player to set video quality.
Both methods rely on passive QoE (engagement) measurements and update per-user QoE model after each video session.
They differ in how they set the quality patterns to induce QoE feedback.

\mypara{Greedy QoE optimization}
The first natural idea is that as more measurements from a user are used to update the per-user QoE model, the QoE model might get more accurate, so the player can always use the latest per-user QoE model as input to the ABR algorithm, with the assumption that the latest QoE model is accurate.
% The most straightforward method is to passively observe the engagement of users when they naturally watch videos, and then update per-user QoE model after each video session.
% To provide the best possible video quality, we optimize the video quality for each video session with the up-to-date video session.
This seems to be a good idea, because the video quality would gradually improve as the QoE model become more accurate.
% In the whole process, the users are not aware of the QoE modeling, because the video quality is becoming better over time and we do not change any user interface (UI) of the video player.

The drawback, however, is that the QoE model may never be accurate enough to realize the full potential of per-user QoE optimization.
As the ABR algorithm is driven by the lates QoE model, video player might have bias on avoiding certain types of low-quality issues that are assumed to be sensitive in the current (potentially inaccurate) QoE model.
Thus, it becomes difficult to learn the user preferences on those types of low-quality issues, thus missing opportunities to optimize QoE. 
For instance, YouTube players typically assume that rebuffering has a greater impact on QoE than low bitrate, so it strives to minimize rebuffering~\cite{?} by aggressively lowering bitrate whenever bandwidth drops. 
However, as we have seen in \S\ref{??}, some users are actually more sensitive to lower birate than to rebuffering. 

% the training process could take a long time, \ie XXX video sessions for a QoE model~\cite{?}, and thus many video sessions are optimized by a sub-optimal per-user QoE model, which lower the QoE improvement.
% The reason of slow QoE modeling is that the video player might have bias on avoiding certain types of low-quality issues that are assumed to be sensitive in the one-size-fits-all QoE model.
% Thus, it is difficult to learn the user preferences on those types of low-quality issues. \jc{and why this makes qoe worse?}
% For example, YouTube players are trying to minimize the rebuffering event~\cite{?} by trading the video resolution off.
% However, Section~\ref{?} shows that some users are not sensitive to rebuffering events. 
% For those users, we might need many sessions to understand those users' insensitivity to the rebuffering events, and thus for those sessions, we miss the QoE optimization opportunities.
% For the new users who just come to the video streaming service, a XXX QoE drop could lower XXX chance of continuing to use the service, and it might translate to XXX loss in profit.


\mypara{Active learning-based strategy}
Another natural choice is 
% Compared with passively QoE monitoring that does deliberately add low-quality issues, another extreme is 
to actively add low-quality issues to video sessions so that an accurate per-user QoE model can be built with minimum number of sessions.
Previous works~\cite{?} exhibit the effectiveness by active learning: for each update of the per-user QoE model, we use the video quality that can contribute most information to the model convergence, \ie the video with the largest uncertainty.
It only needs XXX videos to get the per-user QoE model from scratch.

This method is not ideal either. 
Although we train per-user QoE model fast and start QoE optimization early, the videos in the training stage might be with severely bad quality, because the video quality patterns with the largest uncertainty in the QoE model are usually with bad video quality.
To accelerate per-user QoE modeling model, the active learning-based methods tend to encapsulate multiple types of low-quality issues into one video, and then deter the new users from using the video service.
For the new users who just come to the video streaming service, a XXX QoE drop could lower XXX chance of continuing to use the service, and it might translate to XXX loss in profit.


\subsection{How \name schedules video quality}
The goal of \name is to do online QoE modeling fast while maintain good video QoE.
The above-mentioned natural ideas cannot achieve this goal: 
greed QoE optimization shows the sub-optimal video by always exploiting QoE model, while active learning-based strategy severely impair the video quality during QoE modeling.

To realize this goal, our insight is to cast the problem into a well-studied frame of regret minimization~\cite{?}.
For each video session, an action is to select a video quality pattern that complies to the user bandwidth limitation.
The regret of an action is the minus sum of QoE and uncertainty of the video pattern selected by this action, \ie the distance to the video with both maximal QoE and uncertainty.

We formulate this problem as minimizing the regret of the actions in current video session and next $T$ sessions:
\begin{align}
    &\min \sum_{i=0}^T -[QoE(v_i)+Uncertainty(v_i)], \label{eq:find_patter}\\
   s.t. \quad & \text{average\_bitrate}(v_i) < \text{Available bandwidth}\label{eq:bt_limit},
\end{align}
where $v_i$ is the action (the selected video quality pattern) in the next $i$-th session ($i=0$ represents the current video session), $QoE(v_i)$ is the predicted QoE of the video quality pattern $v_i$, and $Uncertainty(\cdot)$ is the uncertainty of the given video quality pattern.
The uncertainty of a video quality pattern means how much the QoE model are not sure about classifying this pattern.
The larger uncertainty of a video quality pattern indicates more information that can contribute the per-user QoE model.
In this paper, we use the minimal margin~\ref{?} to quantify the video uncertainty.
In the random forest-based QoE model, the margin is calculated by the vote count difference between the class with the most votes ans the class with the second most votes.
The constraint in~\ref{?} is to make sure we can complete chunk downloading before we watch this chunk, and the constraint~\ref{?} is to limit the user's average bandwidth.
The constraint~\ref{eq:bt_limit} make sure the videoq quality patter is feasible under the user's available bandwidth.
In practice, we consider $T=?$, and for the future sessions, we assume the bitrate of the chunks in the future videos is the same as the current video session.

A feature of such a formulation is that we do not need a clear boundary between the QoE modeling training and optimization stages, regarding that verifying whether the model is converged is also not a trivial problem.
With more video sessions, the per-user QoE model is getting converged, so that the portion of uncertainty is becoming marginal, and minimizing regret will be automatically converted to QoE optimization.



% From the lessons of the previous works, the goal of \name is to fast learn the per-user models and maintain good QoE during QoE model training.
% We want to find a rate-limiting scheme, $B(\cdot)$, that can output a video quality pattern $v$ with the maximal sum of QoE and the amount of information contributing to the QoE model training (\ie uncertainty) by limiting the bandwidth over time.
% % \xu{rate-limiting, bandwidth-capping, bandwidth-control. which one is the better term?}
% Both passive QoE monitoring and active-learning based method cannot achieve our goal, because the former is to maximize user QoE and ignore the uncertainty during the QoE modeling stage, while the other drives in an opposite way.


% Our insight is to cast the problem into a well-studied framework of regret minimization~\cite{?}. 
% The regret is defined as the minus sum of video QoE and uncertainty, and it represents the distance to the video with both maximal QoE and uncertainty.
% The action is the video quality pattern for this video pattern.

% Our formulation is to minimize the regret of the next $T$ video sessions:

\subsection{Dynamic rate limiting}
In our setting, we cannot directly control over the player's choice on quality selection.
Instead, we control the downloading rate (\ie bandwidth) during the course of a session to indirectly control the quality pattern by expecting the player can adapt to the rate we set.
As a result, we might fail to achieve the video quality pattern scheduled by \name's, and the resulted video quality pattern might be with small QoE or uncertainty.
Thus, we should consider the player's behavior in bitrate selection into account.

% The naive solution is that when downloading a chunk, we set the bandwidth to the bitrate we want to obtain in $v$.
% However, if we do so, the user perceived video quality might have much larger regret than we expect!
% For example, if we want to provide the QoE model with the information about video quality dropping from 720p to 480p, in practice there is a chance to get a rebuffering event instead of a 360p chunk.
% If the QoE model already has the information about rebuffering event, such a video quality pattern cannot contribute the uncertainty and good video quality.

First, we prove that the player has the ability to adapt to the video quality scheduled by \name in a short time.
We create the network bandwidth traces that are expected to affect the video player to change the video birate from one to the other.
For example, if we want to have a video bitrate changing from 1Mbps to 500Kbps at the 10-th chunk, in the bandwidth trace we can lower the bandwidth from 1Mbps to 500Kbps when we download the 10-th chunk.
Those network bandwidth traces enumerate all possible video bitrate changes for the video XXXX (\url{www}), and for each kind of bitrate change, we run more 100 times.
In Figure~\ref{?}, we can see that for more than XXX\% cases, the player can adapt to the video quality within in XXX seconds.
\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\linewidth]{fake_graphs/time_to_bounce_back.pdf}
    \caption{The CDF of time that the player needs to adapt its quality to the bandwidth we set. }
    \label{fig:br_adapt}
\end{figure}


Now, we can profile the behavior of the video player.
The prior works~\cite{?} state that the player behavior can be reversed engineering by analyzing the historical data of player choice under different player status.
We profile the probability of a player state changing to another, \ie $D(s_1, s_2, b)$, where $s_1$ and $s_2$ represents the player states, including current bitrate, buffer length, and $b$ is the current bandwidth.
To obtain the transition probability between $s_1, s_2$ under bandwidth $b$, we set the player state to $s_1$ under bandwidth $b_1$ for 100 times, and $D(s_1, s_2, b)$ is the times of the states becoming $s_2$ divided by 100.
Due to the infinite number of all possible player states and bandwidth, we bucketize the bitrate, buffer length and bandwidth for every 200Kbps, 1 second and 200Kbps respectively.
\xu{should specify the video content?}


With the player's behavior profile, our optimization objective is to find a rate-limiting scheme $B$ (bandwidth over time) that can minimize the expected regret for the next $T$ video sessions:
\begin{align}
  \quad&\min -\sum_{i=0}^T\sum_{v_i}p\left(B_i, v_i\right)*[QoE\left(v_i\right)+Uncertainty\left(v_i\right)] \\
  \text{s.t. } & average\_bandwidth(B_i)\leq \text{Available bandwidth} 
\end{align}
where $B_i$ is the rate-limiting scheme for the next $i-th$ session. 
We define $p(B,v)$ as the probability that the video quality pattern $v$ appears under the rate-limiting scheme $B$, and $p(B,v)$ can be calculated by the player profile by going through all possible video quality patterns.
During a video session, the player status is updating over time, and $p(B,v)$ updates accordingly.
Thus, we can update the rate-limiting scheme $B$ by the updated $p(B,v)$.


\subsection{Reducing controller computation overhead}
To calculate the expected regret of a rate-limiting scheme, we might need to enumerate all possible video quality pattern under this scheme.
It is costly prohibitive if we enumerate all the quality patterns due to the large number of the future chunks.
To save the cost, we need to reduce the number of patterns we need to enumerate.
\begin{itemize}
    \item Reducing looking-ahead horizon: When determine the bandwidth of downloading a chunk, we do not need to enumerate all possible quality of the future chunks.
    We can only look ahead for a few number of future chunks and enumerate their quality.
    For the later chunks, we assume the player will perfectly adapt to the bandwidth we set.
    In \name, the looking-ahead horizon is XXX, and we evaluate the choice in Section~\ref{?}
    \item Considering adjacent chunks as a whole: Usually, the length of a chunk in the video streaming services is from XXX to XXX seconds.
    From Figure~\ref{?}, we can see that only XX\% cases can adapt to the desired bitrate within a chunk's time.
    So, we can consider the quality of several adjacent chunks a whole, and it can reduce the time of enumeration.
    For example, for a 60-second long video with 3-second chunk size, we need to enumerate 60/3=20 times, while if we consider 4 adjacent chunks as a whole, we only needs to enumerate 60/(3*4) = 5 time, which saves more than 400\% computation cost.
\end{itemize}

%  illustrate 

==> qoeprofiling-v3.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US



\tightsection{Online QoE modeling and optimization}
\label{sec:framework}

% - framework of online qoe modeling: set qoe, get qoe feedback
% - four requirements
% - design space => design point
% - how we set quality
% - how we handle player uncertainty

We have seen that there is substantial user heterogeneity in QoE.
Now, several previous efforts have proposed QoE optimization (ABR logic~\cite{huo2020meta} and bandwidth allocation~\cite{chen2015qoe}) that take advantage of {\em known} user preferences.
However, they are unable to optimize a new user right after the user joins, as one must first model the user's unique QoE preference.

To bridge the gap, in this section, we first formulate the general problem of {\em online QoE modeling and optimization} and elaborate why existing techniques designed for different-yet-related purposes are not well-suited for this framework. 

% \vspace{-1em}
\tightsubsection{Framework}

%\mypara{Framework}
We envision online QoE modeling and optimization in terms of a simple framework that a service provider can use to profile per-use QoE models and then optimize QoE for new users.
Depicted in Figure~\ref{fig:online-framework}, this framework allows users to watch videos in their natural environments (any content users wish to watch at any time). 
It contains a logical controller (which could be operated by a service provider or by the player) that determines the video quality during each video session.
At the same time, the controller monitors the QoE (defined shortly) of each session and uses the measurements of QoE (subjective) and the video quality (objective) from each session to update the per-user QoE model maintained by the controller. 
%While it may look like other controllers that optimizes ABR or bandwidth allocation decisions, this framework serves a different purpose: it seeks to uncover the 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{fake_graphs/online-framework.pdf}
    \caption{Framework of online QoE modeling and optimization.}
    \label{fig:online-framework}
\end{figure}

\begin{table*}[]
\small
\begin{tabular}{ccccc}
\hline
 & \begin{tabular}[c]{@{}c@{}}{\bf R1:} No control on when \\ \& what users watch\end{tabular} & \begin{tabular}[c]{@{}c@{}}{\bf R2:} Fast (min \# of \\ profile videos)\end{tabular} & \begin{tabular}[c]{@{}c@{}}{\bf R3:} High QoE \\ during profiling\end{tabular} & \begin{tabular}[c]{@{}c@{}}{\bf R4:} Accurate per-user \\ QoE model\end{tabular} \\ \hline
Lab study~\cite{duanmu2019knowledge,duanmu2016sqi} &  &  &  & \ding{52} \\ \hline
Offline data analysis~\cite{gao2020personalized} & \ding{52} &  & \ding{52} & \ding{52} \\ \hline
%No intervention~\cite{??} & \ding{52} &  & \ding{52} &  \\ \hline
Greedy profiling~\cite{chang2018active} & \ding{52} & \ding{52} &  & \ding{52} \\ \hline
Greedy optimization~\cite{menkovski2010online} & \ding{52} &  & \ding{52} &  \\ \hline
\name (ours) & \ding{52} & \ding{52} & \ding{52} & \ding{52} \\ \hline
\end{tabular}
\vspace{0.4cm}
\caption{Requirements of an ideal realization of online QoE modeling and optimization, and in what aspects prior solutions are ill-suited.}
\vspace{-1.7em}
\label{tab:comparison}
\end{table*}

In modeling the QoE preferences for each user, an ideal realization of an online QoE modeling and optimization framework should meet four properties (Table~\ref{tab:comparison}):
\begin{packeditemize}
\item {\bf R1:} It should not control when and what users watch, since real service providers (CDN, ISP) or content providers are unlikely to specify what videos real users must watch first. 
\item {\bf R2:} It should finish QoE modeling within a small number of video sessions, because service providers want to optimize each of their users as early as possible. 
\item {\bf R3:} It should provide high QoE while modeling per-user QoE, \ie one cannot model per-user QoE at the cost of user experience. 
% for the same reason that service providers want to maintain high user experience throughout. 
\item {\bf R4:} Finally, we want the eventual per-user QoE models to be accurate enough for per-user optimization techniques (ABR logic and bandwidth allocation) to best leverage the heterogeneity across users.
\end{packeditemize}

Figure~\ref{fig:ideal-timeseries} shows a desirable behavior of \name (blue line): 
For each user, the quality and QoE measurements of each video session will be used to update the user's QoE model, and over time, the QoE model will become more accurate such that future video sessions can leverage the latest per-user QoE model to improve quality over the baseline (grey) that is agnostic to per-user QoE preferences. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\linewidth]{fake_graphs/method_compare.pdf}
    \caption{QoE over time of an ideal realization of online QoE modeling and optimization (blue) where QoE improves quickly as per-user QoE model becomes more accurate. 
    It outperforms the strawman of active-learning-based aggressive profiling (red) which uses low-quality videos to elicit QoE feedback) and greedily optimizing QoE (green) which relies on the latest though inaccurate per-user QoE model. 
    % \jc{Xu, this figure needs to be improved :)}
    }
    % \vspace{-0.4em}
    \label{fig:ideal-timeseries}
\end{figure}





\tightsubsection{Why is it different?}
\label{subsec:strawmen}

Table~\ref{tab:comparison} puts existing techniques into the context of these four dimensions. 

First, many previous QoE studies, based on controlled lab studies or crowdsourcing surveys~\cite{zhang2021sensei,duanmu2019knowledge,duanmu2016sqi}, are ill-suited, because they require users to watch videos of specific content while varying the video quality to induce QoE samples to build a good QoE model (\ie violating {\bf R1}).
Alternatively, offline data analysis is commonly employed by service providers who are in a position to passively collect massive data on quality and QoE of a large number of sessions from each user~\cite{zhao2019qoe}. 
While analyzing such large datasets might ultimately yield accurate QoE models, the QoE modeling is still done offline (\ie violating {\bf R2}), rather than as an integrated part of the online QoE optimization framework. 

To address these shortcomings, two seemingly natural designs emerge.
Both rely on passive QoE measurements and update the per-user QoE model after each video session.
They differ in whether they set video quality to maximally improve user QoE or maximally help QoE modeling.

%\begin{packeditemize}
\mypara{Greedy optimization using biased QoE models}
As more measurements from a user are collected to update the per-user QoE model, the player can use the latest per-user QoE model as input to the ABR algorithm, under the assumption that the latest QoE model is accurate enough.
This is promising, because the video quality would gradually improve as the QoE model becomes more accurate.
The drawback, however, is that the QoE model may never be accurate enough to realize the full potential of per-user QoE optimization.
This is because 
% As the ABR algorithm is driven by the latest QoE model, 
the latest QoE model may be inaccurate and thus introduces bias in the ABR decisions. 
For instance, 
% player to avoid certain types of low-quality issues that  in the current (potentially inaccurate) QoE
% video player might have bias on avoiding certain types of low-quality issues that are assumed to be sensitive in the current (potentially inaccurate) QoE model.
% Thus, it becomes difficult to learn the user preferences on those types of low-quality issues, thus missing opportunities to optimize QoE. 
% For instance, 
YouTube players typically assume that rebuffering has a greater impact on QoE than low bitrate, so it strives to minimize rebuffering~\cite{anorga2015youtube} by aggressively lowering bitrate whenever bandwidth drops. 
However, as we have seen in \S\ref{sec:moti:hetero}, some users are actually more sensitive to lower birate than to rebuffering. 
So the QoE model may never learn how sensitive each user actually is to rebuffering, thus missing opportunities to optimize QoE (\ie violating {\bf R4}). 


\mypara{Greedy profiling using active learning}
Another natural choice is to add quality issues to video sessions in a way that the user's QoE feedback will maximally reduce the uncertainty of the current QoE model. 
Previous works~\cite{chang2018active} show that active learning (which shows users the video quality whose QoE the current model is most uncertain about) can be used to minimize the number of sessions (QoE samples) needed to build an accurate QoE model;
\eg it only needs $\sim$100 videos to get the per-user QoE model from scratch.
% This will  the  accurate per-user QoE model can be built with minimum number of sessions.
% Previous works~\cite{?} effectiveness by active learning: for each update of the per-user QoE model, we use the video quality that can contribute most information to the model convergence, \ie the video with the largest uncertainty.
This method is not ideal either. 
Although we can train per-user QoE models quickly and start QoE optimization early, the videos in the training stage might require severely bad quality (\ie violating {\bf R3}), because the video quality patterns (\ie a video quality pattern is the quality of each chunk in the video session.) with the largest uncertainty in the QoE model are usually with bad video quality.
To accelerate per-user QoE modeling, the active learning-based methods tend to encapsulate multiple types of quality issues into one video, and the low video quality can cause tens of billions of dollars profit damage according to Conviva~\cite{convivadamage}.

% then deter the new users from using the video service.
% For the new users who just come to the video streaming service, a XXX QoE drop could lower XXX chance of continuing to use the service, and it might translate to XXX loss in profit.
%\end{packeditemize}


\tightsection{Design of \name}
\label{sec:design}

In this section, we describe a specific setting for which we would design a concrete solution, {\em \name}, to realize online QoE modeling and optimization.

\tightsubsection{Overview}

% \mypara{Setting}
%\mypara{Design space}
The design space of online QoE modeling can be characterized along two dimensions:
\begin{packeditemize}
\item {\em What QoE feedback} will be collected from each session?
\item {\em What control knobs} will be used to influence video quality? 
\end{packeditemize}

\mypara{Setting of \name}
\name is a realization of online QoE modeling and optimization in a specific design point.
\name makes \xu{three} practical assumptions (we will describe how we implement this setting in \S\ref{sec:impl}).
First, to minimize the user annoyance, we use user engagement as the QoE metric.
Unlike user ratings (used in many prior proposals), the video engagement can be collected passively, while the quality ratings must be given manually by users in an exit-survey (during or after each video session).
\xu{Although user engagement can be affected other factors (\eg video content, etc.), previous works show a strong relationship between user engagement and the perceived video quality~\cite{?}.}
Second, we do not control the video content or directly change the behavior of the video player.
Instead, \name passively monitors the player status (\eg video resolution, buffer length, etc) to infer the video quality which can be used to train per-user QoE model with user engagement.
It then dynamically changes the available bandwidth to indirectly control the video player's bitrate selection.
\xu{Third, other than the perceived video quality, we do not interfere with the other experience of viewing videos, including user interface (UI), player settings, etc.
It lets the video quality stand out of the factors that can affect user engagement time. 
}
%instead of directly control the module of deciding downloading video bitrate in the video player.
% Finally, we can use the per-user QoE models to optimize the QoE of individual users by controlling bandwidth.

This setting can be suitable for network service providers, such as ISPs, CDNs, and edge routers, who control the bottleneck bandwidth of a user. 
The network service providers do not have the access to the video player's logic but can monitor and control the users' network connection.
To obtain the video quality, service providers can use  existing techniques to infer video quality by the video streaming traffic \cite{bronzino2019inferring}, and use the session time of the video streaming as the user engagement, and can guess the player status with up to 91\% accuracy. 
We evaluate the impact of the player status inference accuracy and the QoE gain of \name in \S\ref{sec:eval}.
Our evaluation results show potential benefits to these service providers in practice: \name can improve QoE (user engagement) without changing the average bandwidth per session, or save bandwidth to achieve the same QoE (\ie if \name is deployed on the bottleneck link, it might support more concurrent users without degrading their QoE).
% can be deployed on the bottleneck link to support more users.

A natural concern regarding this setting is whether user engagement measurements from arbitrary video content are reliable enough to model per-user QoE.
Intuitively, video content does impact users' sensitivity to video quality.
However, in our study, the selection of quality level is totally agnostic to video content.
Thus, averaging over a sufficient amount of data can still reliably build per-user QoE models.
We make this as a pragmatic choice, because our user study cannot record video content.
That said, we hope future studies will take video content and other factors (\eg viewing device) into the modeling of per-user QoE.


\begin{comment}

The independency between content and quality may not always hold, but we empirically find it has a marginal impact. 
For instance, we use a permutation test~\cite{montgomery2010applied} to calculate the significance of the following statement: 
The video content does not affect a user's sensitivity to the same quality issue.
For a quality issue $A$, we select all the video session traces in \name dataset, and other than $A$, those traces also have similar quality in other video parts.
We randomly divide those traces into two group, and test whether the QoE drop of the videos in the two groups is from the same distribution by permutation test.
Since the videos in two groups have different content, if their QoE drop distributions are the same, it means the video content does not have significantly impact on QoE sensitivity.
We test the quality issues (including 0-0.5, 0.5-1.0 second rebuffering, 0-500, 500-1000Kbps bitrate drop, 0-500, 500-1000, 1000-1500Kbps bitrate switch), and the p-values are all larger than 0.05, meaning that we should accept our hypothesis.

\end{comment}

% \jc{write down clearly the z-test statement and the z-test results}


% Another natural concern is how service providers obtain the video quality.
% Fortunately, there are existing techniques to infer video quality by the video streaming traffic \cite{?}.
% We can use the session time of the video streaming as the engagement, and can guess the player status with XX\% accuracy. 
% We evaluate the impact of the player status inference accuracy and the QoE gain of \name in \S\ref{?}.



\mypara{Components} 
Based on the setting, we envision \name has three modules as shown in Figure~\ref{fig:overview}: 
% \jc{xu, please add these modules in the system overview figure}

\begin{packeditemize}
\item {\em Video quality scheduling:}
For each video session, \name first determines the {\em quality pattern} (\ie the quality of each video chunk) of the session.
Ideally, the quality pattern itself should induce decent QoE, while the QoE measurement from the chosen quality pattern would improve the accuracy of the QoE model. 
% For each video session, \name needs to schedule its bandwidth for obtaining the video quality pattern (\ie the quality of each video chunk) to maximize the information contributing to QoE modeling and maintain high QoE.
% This module takes the player status (\eg video resolution, buffer length) and the video engagement as the input to train per-user QoE model.=


\item{\em Dynamic rate limiting:}
Once the video quality pattern is determined, we then need to decide how to dynamically set available bandwidth to realize the quality pattern.
% by limiting the user's video downloading rate.
Ideally, if the video players can rapidly adapt to the downloading rate, we can set the rate as the bitrate of the video quality we want.
% However, in practice, the behavior of video player is more complicated: the video bitrate selection decision can be affected by many factors, such as historical bandwidth, current video resolution, and player buffer length\cite{?}.
% The difficulty is that the player behavior is usually unknown to \name's bandwidth controller, and we might not be able to obtain video quality pattern we have scheduled.
% We deal with this difficulty in Section~\ref{?}.

\item{\em Per-user QoE modeling:}
Finally, the measurements of engagement and video quality from each user are fed to update the user's QoE model.
% Following the practice in previous works~\cite{?}, we use a random forest to train per-user QoE model.
Since the design of the QoE model itself is not our contribution, we reuse a random-forest-based QoE model from prior work~\cite{chang2018active}
and use per-user QoE measurement data to train the model for each user.\footnote{
In particular, the QoE model works as follows. 
This model takes the video quality as the input variables, and outputs the expected QoE as the output.
The input variables are the video quality of the chunks.
Based on the QoE model we currently have and the video trace, we can decide the video quality pattern to show the users.
We customize feature selection and criteria at the nodes on each decision tree inside the forest.
To train the QoE model faster, the initial QoE model is a one-size-fits all model.
To avoid the explosion of input due to the large number of video chunks, we divide the video into 20 parts, and QoE model will take the quality of each part.
The total number of input variables are 20 * 3 = 60.
The video quality of each part includes its average video bitrate, total bitrate switch, total rebuffering time.
The output is the user QoE.
The QoE is bucketized the user engagement into 10 classes, and the output is the class who gets the most votes from the decision trees inside the random forest.}


\end{packeditemize}

Next, we will explain how \name's quality scheduler and rate limiting module achieves meet the four requirements. 


\begin{figure}[t]
    \includegraphics[width=1.0\linewidth]{fake_graphs/end-to-end.pdf}
    \caption{System overview of \name. 
    % \jc{xu, please add these modules in the system overview figure}
    }
    \label{fig:overview}
\end{figure}


\tightsubsection{How \name schedules video quality}
\label{subsec:design:balancing}

The goal of \name is to model QoE online, \ie in real-time, while maintaining good video QoE.
% The above-mentioned natural ideas cannot achieve this goal: 
The two solutions described in \S\ref{subsec:strawmen} are undesirable:
greedy optimization leads to sub-optimal video quality in the long run since it relies on a biased QoE model, while the aggressive modeling approach severely impairs the video quality early on during QoE modeling.

To address this challenge, our insight is to cast the problem into a well-studied frame of regret minimization~\cite{loomes1982regret}.
For each video session $i$, we select a video quality pattern $v_i$ among those that are possible stream under a given average bandwidth limitation.
Mathematically, the picked quality pattern should maximize the sum of the estimated expectation of QoE and the uncertainty of this estimation (explained shortly).
Formally, we solve the following problem to select the quality pattern $v_i$:
\begin{align}
    \max& \quad\quad QoE(v_i)+Uncertainty(v_i), \label{eq:find_patter}\\
   \text{s.t.}&  \quad BandwidthUsage(v_i) < BandwidthLimit\label{eq:bt_limit},
\end{align}
$QoE(v_i)$ is the predicted QoE \xu{(\ie predicted user engagement here)} of the video quality pattern $v_i$, $Uncertainty(v_i)$ is the uncertainty of this prediction, the $BandwidthLimit$ is the pre-determined maximum average bandwidth per session (\eg this can be based on the Internet plan subscribed by the user), and $BandwidthUsage(v_i)$ is calculated by dividing the sum of bitrates of expected watched chunks (the ones within the predicted viewing time $QoE(v_i)*VideoLength$) by the predicted viewing time.

Given the current QoE model (a random forest of decision trees) and a quality pattern $v_i$, each decision tree returns a predicted QoE bucket (a range of user engagement), and we count the number of ``votes'' given by these decision trees to each possible QoE bucket. 
QoE prediction $QoE(v_i)$ is the median of the QoE bucket with the most votes.
The uncertainty $Uncertainty(v_i)$ of this prediction is measured by the difference between the highest vote count and the second highest vote count. 
(This way of measuring uncertainty is also called {\em minimal margin}~\cite{settles2009active}.)
Intuitively, the uncertainty of a video quality pattern indicates how much the current QoE model is unsure about predicting the QoE of this quality. 
The constraint of Eq.~(\ref{eq:bt_limit}) ensures that it is possible to stream the video under the quality pattern $v_i$ within the expected viewing time $QoE(v_i)$ without using more bandwidth than $BandwidthLimit$.

Once a session ends, a pair of its actual session-level quality and user QoE (user engagement) is used to update the current QoE model.
This can be done in various ways.
In our implementation, we train the initial QoE model of each user based on an ``initial dataset'' of 120 sessions which are collected from 10 users\footnote{Those users met the recruiting criteria in~\S\ref{sec:impl} but quit in the middle.} (different from the users whom we eventually test \name on) during the first 2 months of the user study.
And then the measurements (pair of session-level video quality and QoE) from a user will be added to a separate copy of the ``initial dataset''.
That is, each time a new measurement is collected from a user, it is added to the the user's version of  ``initial dataset'' and retrains the model for this user.\footnote{One needs to balance the data size of the ``initial dataset'' and the new samples from each user: if the initial dataset is too large, it will dominate the training of the per-user QoE model. In our implementation, the initial dataset (120 sessions) does not seem to overly dominate the per-user model, but we leave a thorough investigation of this issue to future work.}
\xu{Although the user engagement can be determined by many factors other than the video quality (\eg video content), we minimize the impact from those factors by 1) limiting the user bandwidth within $[XX, XX]Kbps$ (We show that within this range, the engagement time is mostly affected by video quality in Sec XXXX), and 2) the users can watch any videos they are interested in.}


An intuitive interpretation of Eq.~(\ref{eq:find_patter}) is that it minimizes the ``regret'' of choosing a quality pattern.
That is, we minimize 
(1) the suboptimality of the expected QoE (via a high $QoE(v_i)$), and 
(2) the impact on future QoE optimization (via choosing a quality that induces feedback on a highly uncertain QoE prediction $Uncertainty(v_i)$).
This formulation effectively balances the QoE of the current video session and the accuracy of QoE modeling which affects future QoE optimization---this balance is what the two strawmen discussed in \S\ref{subsec:strawmen} do not address.



% we can complete chunk downloading before we watch this chunk, and the constraint~\ref{?} is to limit the user's average bandwidth.


% The uncertainty of a video quality pattern means how much the QoE model are not sure about classifying this pattern.
% The larger uncertainty of a video quality pattern indicates more information that can contribute the per-user QoE model.
% In this paper, we use the minimal margin~\cite{?} to quantify the video uncertainty.
% In the random forest-based QoE model, the margin is calculated by the vote count difference between the class with the most votes and the class with the second most votes.

% The constraint~\ref{eq:bt_limit} make sure the videoq quality patter is feasible under the user's available bandwidth.
% In practice, we consider $T=?$, and for the future sessions, we assume the bitrate of the chunks in the future videos is the same as the current video session.

% Another benefit of the formulation in Eq.~(\ref{eq:find_patter}) is that it adaptively decides when to improve the accuracy of the QoE model and when to optimize the current session's QoE. 

% A feature of such a formulation is that we do not need a clear boundary between the QoE modeling training and optimization stages, regarding that verifying whether the model is converged is also not a trivial problem.
% With more video sessions, the per-user QoE model is getting converged, so that the portion of uncertainty is becoming marginal, and minimizing regret will be automatically converted to QoE optimization.


% The regret of an action is the negative of the sum of expected QoE and uncertainty of the video pattern selected by this action, \ie the distance to the video with both maximal QoE and uncertainty.

% We formulate this problem as minimizing the regret of the actions in current video session and next $T$ sessions:
% \begin{align}
%     &\min \sum_{i=0}^T -[QoE(v_i)+Uncertainty(v_i)], \label{eq:find_patter}\\
%   s.t. \quad & \text{average\_bitrate}(v_i) < \text{Available bandwidth}\label{eq:bt_limit},
% \end{align}
% where $v_i$ is the action (the selected video quality pattern) in the next $i$-th session ($i=0$ represents the current video session), 





% From the lessons of the previous works, the goal of \name is to fast learn the per-user models and maintain good QoE during QoE model training.
% We want to find a rate-limiting scheme, $B(\cdot)$, that can output a video quality pattern $v$ with the maximal sum of QoE and the amount of information contributing to the QoE model training (\ie uncertainty) by limiting the bandwidth over time.
% % \xu{rate-limiting, bandwidth-capping, bandwidth-control. which one is the better term?}
% Both passive QoE monitoring and active-learning based method cannot achieve our goal, because the former is to maximize user QoE and ignore the uncertainty during the QoE modeling stage, while the other drives in an opposite way.


% Our insight is to cast the problem into a well-studied framework of regret minimization~\cite{?}. 
% The regret is defined as the minus sum of video QoE and uncertainty, and it represents the distance to the video with both maximal QoE and uncertainty.
% The action is the video quality pattern for this video pattern.

% Our formulation is to minimize the regret of the next $T$ video sessions:

\tightsubsection{Dynamic rate limiting}
\label{subsec:dynamicratelimiting}
In our setting, a practical concern is that we cannot directly control the player's selection of quality.
Instead, we control the downloading rate (\ie bandwidth) during the course of a session to indirectly control the quality pattern \xu{by inducing the ABR algorithm to adapt to the downloading rate we set}.
As a result, we might fail to achieve the video quality pattern selected by \name's quality pattern scheduler (\S\ref{subsec:design:balancing}).
\xu{Here, we discuss how to take the failure of obtaining the desired video bitrate into account.}
% Thus, we must take the player's behavior in bitrate selection into account.

% The naive solution is that when downloading a chunk, we set the bandwidth to the bitrate we want to obtain in $v$.
% However, if we do so, the user perceived video quality might have much larger regret than we expect!
% For example, if we want to provide the QoE model with the information about video quality dropping from 720p to 480p, in practice there is a chance to get a rebuffering event instead of a 360p chunk.
% If the QoE model already has the information about rebuffering event, such a video quality pattern cannot contribute the uncertainty and good video quality.


\xu{The reason why we can control the video bitrate by the downloading rate is that numerous prior studies have shown that ABR-enabled players can adapt its video quality in response to changes in the available bandwidth.}
(In fact this is used by several papers to reverse-engineer video player logic~\cite{gruner2020reconstructing}).
% largely in the way scheduled by \name within a relatively short delay.
%To show this, we create several network bandwidth traces that are expected to affect the video player to change the video bitrate from one to the other.
% \xu{A naive example is that}, if we want to the player to change its video bitrate from 1Mbps to 500Kbps at the $10^{\textrm{th}}$ chunk, we can lower the bandwidth from 1Mbps to 500Kbps when the player downloads the $10^{\textrm{th}}$ chunk.
\xu{In practice, although the logic of determining the video chunk bitrate inside the ABR logic is a black box, we generally know that it is determined by the player's QoE model, buffer length, and the predicted QoE model.
The selected bitrate for downloading is the one that can maximize the expectation of QoE given the predicted network bandwidth and the buffer length.
A naive example is that, if we want to the player to change its video bitrate from 1Mbps to 500Kbps at the $10^{\textrm{th}}$ chunk, we need to convince the player's ABR algorithm that when it downloads the $10^{\textrm{th}}$ chunk, the available bandwidth is $500Kbps$, and choosing $500Kbps$ bitrate will bring the largest expectation of QoE.
To show this point, we create several network bandwidth traces that are expected to affect the video player to change the video bitrate from one to the other.
Those traces starts with the buffer length, and the current playing video bitrate, and then we change the downloading throughput to another bitrate different from the current one.
We investigate how long the player can adapt its video bitrate to the downloading throughput we set.
Figure~\ref{?} shows that for more than XX\% traces of a participant in our user study, the desired bitrate can be achieved within XX seconds.
We confirm that it also holds for the rest of the users. 
}


An important takeaway from these prior works is that there is usually a non-trivial delay between when the bandwidth changes and when the player responds, and the bitrate which the player switches to is often a distribution, rather a fixed value. 
% the player may even not respond to the change of bandwidth in the way we want (if it changes at all).

\xu{
% Note that there is a rare chance that the player's ABR algorithm cannot adapt to the bandwidth we set.
% It happens when we increase(decrease) the bandwidth but the ABR algorithm cannot increase(decrease) the video bitrate accordingly.
% Actually, this case does not affect us in terms of building per-user QoE model and optimizing the user QoE of video sessions.
% Because we already take the failure of achieving the desired video quality pattern into consideration when we select the bandwidth allocation plan.

Note that there are multiple possible video quality patterns that can be generated by the same bandwidth allocation plan, and we might not get the video quality pattern with the minimal regret.
We admit it could happen, but we can minimize the negative impact, \ie few contribution to the QoE model training and/or bad user QoE.
First, we already consider the possibility of getting the other video quality patterns, since those video patterns' regrets are calculated in the regret expectation of the bandwidth allocation plan.
Second, one might argue that we might calculate the wrong expectation because the profile of the player behavior might not be accurate.
It does happens if the ABR logic changes or the player behavior profile has insufficient data.
Thus, we can either re-profile the player's behavior or add more data points to the existing profile.
}


This observation inspires our solution: 
instead of determining how to induce the player to {\em deterministically} change its bitrate, a more pragmatic approach would be to model {\em distribution} of player's action (when to switch to what bitrate).
In our implementation, we first obtain this distribution on the YouTube player\footnote{YouTube is known to occasionally change the player ABR logic. In this test, we use the YouTube player obtained during Sept 2021 - Dec 2021.} that we test in our user study as follows. 
We run an exhaustive test to build the transition distribution of $D(s_1, s_2, b)$, where $s_1$ and $s_2$ represents the player states, including current bitrate, buffer length, and $b$ is the current bandwidth.
To obtain the transition probability between $s_1, s_2$ under bandwidth $b$ within 12 seconds\footnote{We use 12 seconds because empirically it is the medium delay between when bandwidth changes and when the video player reacts.}, we set the player state to $s_1$ under bandwidth $b_1$ for 100 times, and $D(s_1, s_2, b)$ is the times of the states becoming $s_2$ divided by 100.
Due to the infinite number of all possible player states and bandwidth, we bucketize the bitrate, buffer length and bandwidth for every 200Kbps, 1 second and 200Kbps respectively.
These transition distributions are inherently specific to the video player under study, and we do not claim they are generalizable to other players. 

\begin{comment}

We run a simple test to empirically validate that to what extent we can change bandwidth to induce quality changes on the YouTube player\footnote{YouTube is known to occasionally change the player ABR logic. In this test, we use the YouTube player obtained during \fillme.} that we test in our user study.
Specifically, we pick a video with a set of available bitrates ({0.2, 0,4, 0.6, 0.8, 1.0}Mbps), and for each pair of two different bitrates, $a$ and $b$ from this set, we run start a video session and ensure its bitrate is $a$, and then change the bandwidth from $a$ to $b$ at time $t$, and record when the YouTube player change the bitrate to $b$ at $t'$ (if at all).
We empirically found that the difference between $t$ and $t'$ is between 5 and 30 seconds (with a median around 17 seconds). 
This may seem a non-trivial delay, but it is relatively short compared to the median video lengths of \fillme minutes in our user study (\S\ref{??}).

% Here, we empirically test how long it takes the YouTube video player to change its bitrate from 

% To demonstrate it, we create network bandwidth traces to enumerate all possible video bitrate changes for the video XXXX (\url{www}), and for each kind of bitrate change, we run more 100 times.
% In Figure~\ref{?}, we can see that for more than XXX\% cases, the player can adapt to the video quality within in XXX seconds.
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.6\linewidth]{graphs/motivation/cdf_time_bounce.pdf}
%     \caption{The CDF of time that the player needs to adapt its quality to the bandwidth we set. }
%     \label{fig:br_adapt}
% \end{figure}



Now, we can profile the behavior of the video player.
The prior works~\cite{?} state that the player behavior can be reversed engineering by analyzing the historical data of player choice under different player status.
We profile the probability of a player state changing to another, \ie $D(s_1, s_2, b)$, where $s_1$ and $s_2$ represents the player states, including current bitrate, buffer length, and $b$ is the current bandwidth.
To obtain the transition probability between $s_1, s_2$ under bandwidth $b$, we set the player state to $s_1$ under bandwidth $b_1$ for 100 times, and $D(s_1, s_2, b)$ is the times of the states becoming $s_2$ divided by 100.
Due to the infinite number of all possible player states and bandwidth, we bucketize the bitrate, buffer length and bandwidth for every 200Kbps, 1 second and 200Kbps respectively.
\xu{should specify the video content?}

\end{comment}

The resulting player's transition distributions fit nicely to the formulation of Eq.~(\ref{eq:find_patter}).
% With the player's behavior profile, 
Instead of finding a quality pattern $v_i$ for session $i$, our optimization objective is to find a rate-limiting scheme $b_i$ (bandwidth over time) that can minimize the {\em expected} regret of the video session:
\begin{align}
  \min& -\sum_{v_i}p\left(b_i, v_i\right)*[QoE\left(v_i\right)+Uncertainty\left(v_i\right)], \label{eq:bw_regret}\\
  \text{s.t.}& \quad BandwidthUsage(b_i)\leq BandwidthLimit,
\end{align}
where $p(b,v)$ is the probability that the video quality pattern $v$ appears under the rate-limiting scheme $b$, and $p(b,v)$ can be calculated by the player profile by going through all possible video quality patterns.
During a video session, the player status is updating over time, and $p(b,v)$ updates accordingly.
Thus, we can update the rate-limiting scheme $b$ by the updated $p(b,v)$.

% \begin{align}
%   \quad\min &-\sum_{i=0}^T\sum_{v_i}p\left(B_i, v_i\right)*[QoE\left(v_i\right)+Uncertainty\left(v_i\right)] \\
%   \text{s.t. } & \text{average\_bandwidth}(B_i)\leq \text{Available bandwidth} 
% \end{align}
% where $B_i$ is the rate-limiting scheme for the next $i-th$ session. 
% We define $p(B,v)$ as the probability that the video quality pattern $v$ appears under the rate-limiting scheme $B$, and $p(B,v)$ can be calculated by the player profile by going through all possible video quality patterns.
% During a video session, the player status is updating over time, and $p(B,v)$ updates accordingly.
% Thus, we can update the rate-limiting scheme $B$ by the updated $p(B,v)$.


\tightsubsection{Reducing controller compute overhead}
\label{subsec:costsaving}
To naively calculate the expected regret of a rate-limiting scheme (Eq.~(\ref{eq:bw_regret})), we need to enumerate all possible video quality patterns under this scheme, which can be prohibitively expensive.
% if we enumerate all the quality patterns due to the large number of the future chunks.
We reduce this overhead by two ideas that limit the number of patterns we need to enumerate.
% \begin{itemize}

First, we use a short look-ahead horizon, such that we do not need to enumerate all possible quality of the future chunks.
For the later chunks, we assume the player will perfectly adapt to the bandwidth we set.
In \name, the look-ahead horizon is 2, and in \S\ref{subsec:microbenchmark}, we will evaluate the impact of different look-ahead horizons on QoE improvement and compute overhead.

Second, we coalesce multiple consecutive chunks as longer segments, so that the bandwidth scheme and quality patterns are determined over a handle of segments, rather than many more chunks. 
For example, for a 60-second long video with 3-second chunk size, we need to enumerate 60/3=20 times, while if we consider 4 adjacent chunks as a whole, we only need to enumerate 60/(3*4) = 5 times, which saves more than 400\% computation cost.


% Reducing looking-ahead horizon: When determine the bandwidth of downloading a chunk, we do not need to enumerate all possible quality of the future chunks.
%     We can only look ahead for a few number of future chunks and enumerate their quality.
%     For the later chunks, we assume the player will perfectly adapt to the bandwidth we set.
%     In \name, the looking-ahead horizon is XXX, and we evaluate the choice in Section~\ref{?}

% Considering adjacent chunks as a whole: Usually, the length of a chunk in the video streaming services is from XXX to XXX seconds.
%     From Figure~\ref{?}, we can see that only XX\% cases can adapt to the desired bitrate within a chunk's time.
%     So, we can consider the quality of several adjacent chunks a whole, and it can reduce the time of enumeration.
%     For example, for a 60-second long video with 3-second chunk size, we need to enumerate 60/3=20 times, while if we consider 4 adjacent chunks as a whole, we only needs to enumerate 60/(3*4) = 5 time, which saves more than 400\% computation cost.
% \end{itemize}

% what if rebuffering event / bitrate drop half/half? Does it affect?
% probablisic: what if the profile is not correct? maybe some reasons it is robust.






==> qoeprofiling.tex <==
\section{Design of \name}

So far we have shown that there is substantial user heterogeneity in QoE.
We present \name, a bandwidth-control system that leverage user heterogeneity to optimize QoE.
In this section, we describe the setting and problem formulation of \name (\S\ref{?}), then discuss two important baselines that illustrate the key challenges (\S\ref{?}), and finally present our algorithm of QoE profiling and optimization in (\S\ref{?}).

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{fake_graphs/method_compare.pdf}
    \caption{.}
    \label{fig:my_label}
\end{figure}

\subsection{Problem formulation}

\name's objectives are to 1) minimize the loss on QoE during online per-user QoE modeling, and 2) fast obtain the per-user QoE model to start QoE optimization early.
As shown in Figure~\ref{?}, our expectation of \name is increasing a user's QoE with the up-to-date per-user QoE model that is updated after each video session.

Different from prior works~\cite{?}, \name's per-user QoE modeling and optimization purely goes online, where the users can watch the videos with any content any time.
For the new users, we are not able to let them stay in a highly controlled environment (\eg stay in the same environment, watch a set of videos with fixed content, etc.), so that the lab-based user study~\cite{?} cannot be applied to train per-user QoE model.
Although some works~\cite{?} can model user QoE by offlinely the data collected in the wild, they usually take long time to collect user data (\eg XXX videos in \cite{?}), and start QoE optimization much late.

In this paper, we focus on realizing our objectives under the settings as shown in Figure~\ref{?}
We use the bandwidth knob to indirectly control the video player's performance instead of directly control the module of deciding downloading video bitrate in the video player.
To minimize the user annoyance, we use engagement (\ie the ratio of the video viewing time and the video length) as the metric of QOE instead of the video quality ratings, because the video engagement can be collected without user awareness, while the quality ratings are filled out by the users in an exit-survey after the video session ends.
Since we do not control the video content, \name passively monitor the player status (\eg video resolution, buffer length, etc.) to infer the video quality which can be used to train per-user QoE model with video engagement.
Finally, we can use the per-user QoE models to optimize the QoE of individual users by controlling bandwidth.

This setting is particularly compatible with the network service providers, such as ISP, CDN, and edge routers.
The network service provides do not have the access to the video player's logic but can control the users' network connection.
Also, \name can save bandwidth to achieve the same QoE (See the bandwidth saving \S\ref{?}), and \name can be deployed on the bottleneck link to support more users.

One immediate question of deploying \name to network providers is how to learn per-user QoE model without knowing the video content?
Although video content has great impact on engagement (\eg the users might end the video session early if the content is not interesting), we argue that the ranking of sensitivity to two different low-quality issues is consistent across different video content.
It means that for two types of low-quality issues with different sensitivity, our priority is to avoid the sensitive one even if we have to trade another off.
To prove this, we use the Z-test~\cite{?} to calculate the significance that a user is more sensitive to a type of low-quality issues than another type.
For example, for a user who is more sensitive to a 1-second rebuffering event than a 500Kbps bitrate drop, the distributions of the QoE drop caused by the rebuffering event and the bitrate drop should be different should be significantly different, \ie how large the overlap of two distributions is.
\xu{need revise}
The Z-score is XXXX which shows that the users have sensitivity to the two low-quality issues across different video content.
We also examine the users who are more sensitive to low-bitrate or bitrate-switch issues than other low-quality issues, and the conclusion also holds.

Another question is that how can we obtain the video quality?
There are many works that can infer video quality by the video streaming traffic \cite{?}.
We can use the session time of the video streaming as the engagement, and can guess the player status with XX\% accuracy. 
We evaluate the impact of the player status inference accuracy and the QoE gain of \name in \S\ref{?}.

Based on the setting, we envision \name has two modules as shown in Figure~\ref{?}:

\mypara{Video quality scheduling}
For each video session, \name needs to schedule its bandwidth for obtaining the video quality pattern (\ie the quality of each video chunk) to maximize the information contributing to QoE modeling and maintain high QoE.
This module takes the player status (\eg video resolution, buffer length) and the video engagement as the input to train per-user QoE model.
Following the practice in previous works~\cite{?}, we use a random forest to train per-user QoE model.
This model takes the video quality as the input variables, and outputs the expected QoE as the output.
The input variables are the video quality of the chunks.
We customize feature selection and criteria at the nodes on each decision tree inside the forest.
To train the QoE model faster, the initial QoE model is a one-size-fits all model.
To avoid the explosion of input due to the large number of video chunks, we divide the video into XX parts, and QoE model will take the quality of each part.
The total number of input variables are XX * 3 = XX.
The video quality of each part includes its average video bitrate, total bitrate switch, total rebuffering time.
The output is the user QoE.
The QoE is bucketized the user engagement into XX classes, and the output is the class who gets the most votes from the decision trees inside the random forest.

Based on the QoE model we currently have and the video trace, we can decide the video quality pattern to show the users.


\mypara{Dynamic rate limiting}
Once the video quality pattern the user has been determined, the next step is to schedule the bandwidth scheme (bandwidth over time) to achieve this pattern by limiting the user's video downloading rate.
Ideally, if the video players can rapidly adapt to the downloading rate, we can set the rate as the bitrate of the video quality we want.
However, in practice, the behavior of video player is more complicated: the video bitrate selection decision can be affected by many factors, such as historical bandwidth, current video resolution, and player buffer length\cite{?}.
The difficulty is that the player behavior is usually unknown to \name's bandwidth controller, and we might not be able to obtain video quality pattern we have scheduled.
We deal with this difficulty in Section~\ref{?}.


\subsection{Why is per-user QoE modeling challenging?}
To highlight the challenge, let us consider two seemingly natural designs used in~\cite{?}.
For now, we assume we can have the direct control over the player to set video quality.

\mypara{Passive QoE monitoring}
The most straightforward method is to passively observe the engagement of the videos watched by users in their daily life, and then update per-user QoE model after each video session.
To provide best possible video quality, we optimize the video quality for each video session with the up-to-date video session.
In the whole process, the users are not aware of the QoE modeling, because the video quality is becoming better over time and we do not change any user interface (UI) of the video player.

The main drawback of this method is that the training process could take a long time, \ie XXX video sessions for a QoE model~\cite{?}, and thus many video sessions are optimized by a sub-optimal per-user QoE model, which lower the QoE improvement.
The reason of slow QoE modeling is that the video player might have bias on avoiding certain types of low-quality issues that are assumed to be sensitive in the one-size-fits-all QoE model.
Thus, we are hard to learn the user preferences on those types of low-quality issues.
For example, YouTube players are trying to minimize the rebuffering event~\cite{?} by trading the video resolution off.
However, Section~\ref{?} shows that some users are not sensitive to rebuffering events. 
For those users, we might need many sessions to understand those users' insensitivity to the rebuffering events, and thus for those sessions, we miss the QoE optimization opportunities.
For the new users who just come to the video streaming service, a XXX QoE drop could lower XXX chance of continuing to use the service, and it might translate to XXX loss in profit.


\mypara{Active learning-based quality scheduling}
Compared with passively QoE monitoring that does deliberately add low-quality issues, another extreme is to actively add low-quality issues to the video sessions for learning per-user QoE model faster.
Previous works~\cite{?} exhibit the effectiveness by active learning: for each update of the per-user QoE model, we use the video quality that can contribute most information to the model convergence, \ie the video with the largest uncertainty.
It only needs XXX videos to get the per-user QoE model from scratch.

This method is problematic: although we train per-user QoE model fast and start QoE optimization early, the videos in the training stage might be with severely bad quality.
Because the video quality patterns with the largest uncertainty in the QoE model are usually with bad video quality.
To accelerate per-user QoE modeling model, the active learning-based methods tend to encapsulate multiple types of low-quality issues into one video, and then deter the new users from using the video service.


\subsection{How \name schedules video quality}
From the lessons of the previous works, the goal of \name is to fast learn the per-user models and maintain good QoE during QoE model training.
We want\ie we want to find a rate-limiting scheme, $B(\cdot)$, that can output a video quality pattern $v$ with the maximal sum of QoE and the amount of information contributing to the QoE model training (\ie uncertainty) by limiting the bandwidth over time.
\xu{rate-limiting, bandwidth-capping, bandwidth-control. which one is the better term?}
Both passive QoE monitoring and active-learning based method cannot achieve our goal, because the former is to maximize user QoE and ignore the uncertainty during the QoE modeling stage, while the other drives in an opposite way.

Our insight is to cast the problem into a well-studied framework of regret minimization~\cite{?}. 
The regret is defined as the minus sum of video QoE and uncertainty, and it represents the distance to the video with both maximal QoE and uncertainty.
The action is the video quality pattern for this video pattern.

Our formulation is to minimize the regret of the next $T$ video sessions:
\begin{align}
    &\min \sum_{i=1}^T -\{QoE(v_i)+Uncertainty(v_i)\}, \\
   s.t. \quad & \int_{0}^{t}bitrate_{v_1}(t) < \int_{0}^{t}B(t) \quad \forall \text{time } t\\
   		& average\_bitrate(v_i) < \text{User bandwidth}, 
\end{align}
where $B(t)$ is the rate-limiting scheme and represents downloading rate at time $t$, $Uncertainty(\cdot)$ is the uncertainty of the given video quality pattern, and $QoE(\cdot)$ is the per-user QoE model, and the average bitrate of $v$ must be smaller than the downloading rate limited by \name.
The uncertainty of a video quality pattern means how much the QoE model are not sure about classifying this pattern.
The larger uncertainty of a video sample indicates more information that can contribute the QoE model training.
In this paper, we use the minimal margin~\ref{?} to quantify the video uncertainty.
In the contenxt of random forest, the margin is calculated by the vote count difference between the class with the most votes ans the class with the second most votes.
The constraint in~\ref{?} is to make sure we can complete chunk downloading before we watch this chunk, and the constraint~\ref{?} is to limit the user's average bandwidth.
In practice, we consider $T=?$, and for the future sessions, we assume the bitrate of the chunks if those videos is the same as the current video session.

A feature of such a formulation is that we do not need a clear boundary between the QoE modeling training and optimization stages, regarding that verifying whether the model is converged is also not an easy problem.
With more video sessions, the per-user QoE model is getting converged, so that the portion of uncertainty is becoming marginal, and minimizing regret will be automatically converted to QoE optimization.


\subsection{Dynamic rate limiting}
In our setting, we cannot directly control over the player's choice on quality selection.
Instead, we control the downloading rate (\ie bandwidth) during the course of a session to indirectly control the quality pattern.
Thus, we have to take the player's behavior into account to solve the formulation.

% The naive solution is that when downloading a chunk, we set the bandwidth to the bitrate we want to obtain in $v$.
% However, if we do so, the user perceived video quality might have much larger regret than we expect!
% For example, if we want to provide the QoE model with the information about video quality dropping from 720p to 480p, in practice there is a chance to get a rebuffering event instead of a 360p chunk.
% If the QoE model already has the information about rebuffering event, such a video quality pattern cannot contribute the uncertainty and good video quality.

We first prove that the player can adapt to the video quality we desire in a short time and high probability. 
In our dataset, we find the video sessions which have bandwidth change, and then examine the percentage of the video sessions that the player can eventually adapt to the changed bandwidth, and how long it will take.
In Figure~\ref{?}, we can see that for more than XXX\% cases, the player can adapt to the video quality within in XXX seconds.
\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\linewidth]{fake_graphs/time_to_bounce_back.pdf}
    \caption{The distribution of the player needs to adapt its quality to the bandwidth we set. We set the player status as XX bitrate and XX second buffer length. We enumerate the change of the bandwidth change in [XX, XXX, XX, ...]Kps, and for each change, we run XXX times.}
    \label{fig:my_label}
\end{figure}


Now, we can profile the behavior of the video player.
The prior works~\cite{?} state that the player behavior can be reversed engineering by analyzing the historical data of player choice under different player status.
We profile the probability of a player state changing to another under bandwidth $B$, \ie $D(s_1, s_2, b)$, where $s_1$ and $s_2$ represents the player states, including current bitrate, buffer length, the past bandwidth.
To obtain the transition probability between $s_1, s_2$ under bandwidth $b$, we set the player state to $s_1$ under bandwidth $b$ for 100 times, and $D(s_1, s_2, b)$ is the times of the states becoming $s_2$ divided by 100.
Due to the infinite number of all possible player states and bandwidth, we bucketize the bitrate, buffer length and bandwidth for every 200Kbps, 1 second and 200Kbps respectively.
\xu{be more clear about what traces are using and the setting}


With the player's behavior profile, our optimization objective is to find a rate-limiting $B(t)$ scheme that can minimize the expected regret:
\begin{align}
  \quad&\min -\sum_{i=1}^T\sum_{v_i}p\left(B_i, v_i\right)*\left(QoE\left(v_i\right)+Uncertainty\left(v\right)\right) \\
  \textbf{s.t.  } \quad & \int_{0}^{t}bitrate_{v_i}(t) < \int_{0}^{t}B_i(t) \quad \forall \text{time } t, \\
  &average\_bandwidth(v_i)\leq \text{User bandwidth} ]\forall i
\end{align}
where $B_i(\cdot)$ is the rate-limiting scheme for the session $i$. 
We define $p(B,v)$ as the probability that the video quality pattern $v$ appears under the rate-limiting scheme $B$.


During a video session, we need to dynamically decide the downloading rate for every chunk instead of a fixed bandwidth scheme determined in the beginning the video session.
we need to decide the bandwidth when we download chunk $m$, we can first enumerate all possible bandwidth allocations schemes, and calculate the possible video quality patterns and the corresponding probability regarding the current player status.
We then find the bandwidth scheme that is with the minimal expected regret.
\xu{May be change the formulation to how to decide the quality of chunk i}.


\subsection{Reducing controller computation overhead}
To calculate the expected regret of a rate-limiting scheme, we might need to enumerate all possible video quality pattern under this scheme.
It is costly prohibitive if we enumerate all the quality patterns due to the large number of the future chunks.
To save the cost, we need to reduce the number of patterns we need to enumerate.
\begin{itemize}
    \item Reducing looking-ahead horizon: When determine the bandwidth of downloading a chunk, we do not need to enumerate all possible quality of the future chunks.
    We can only look ahead for a few number of future chunks and enumerate their quality.
    For the later chunks, we assume the player will perfectly adapt to the bandwidth we set.
    In \name, the looking-ahead horizon is XXX, and we evaluate the choice in Section~\ref{?}
    \item Considering adjacent chunks as a whole: Usually, the length of a chunk in the video streaming services is from XXX to XXX seconds.
    From Figure~\ref{?}, we can see that only XX\% cases can adapt to the desired bitrate within a chunk's time.
    So, we can consider the quality of several adjacent chunks a whole, and it can reduce the time of enumeration.
    For example, for a 60-second long video with 3-second chunk size, we need to enumerate 60/3=20 times, while if we consider 4 adjacent chunks as a whole, we only needs to enumerate 60/(3*4) = 5 time, which saves more than 400\% computation cost.
\end{itemize}



==> qoeprofiling_temp.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\section{System design}
\label{sec:qoeprofiling}

\subsection{Problem formulation}

\mypara{System setting}
\begin{itemize}
    \item Illustrate end-to-end procedure of the video streaming systems, where we can put \name
    \item Introduce the settings of \name: why we limit bandwidth?
\end{itemize}

\mypara{Per-user QoE modeling}
\begin{itemize}
    \item this module should output per-user QoE model the quality patterns we want to show the users.
    \item What QoE model we want to build? Why we use engagement instead of explicit user rating?
\end{itemize}

\mypara{Bandwidth capping}
\begin{itemize}
    \item Why we can control video quality pattern by changing bandwidth?
\end{itemize}

\subsection{Baselines of per-user QoE modeling}
\begin{itemize}
    \item passive feedback collection, no harm to the video quality, slow model training. (give a pointer how slow it is)
    \item active learning: aggressively add quality issues for minimizing the number of training videos. Start the optimization phase as soon as possible. (as fast as 100 video sessions from a random QoE model) 
\end{itemize}

\subsection{Balancing training speed and QoE}
\begin{itemize}
    \item our purpose is fast model training and less harm to video quality.
    \item if we assume the player can immediately adapt to the bandwidth change, formulate the math problem.
    \item In practice, the player's behavior is not known. We should take this player uncertainty into account. 
    \item How to profile the player's behavior? Enumerate the player status, log the choice.
    \item An algorithm that shows how do we determine the bandwidth when downloading chunk $i$ given the player status, and the video quality of the previous chunks.
\end{itemize}

\subsection{Reduce computation cost}
\begin{itemize}
    \item The overhead is caused by we need to enumerate the video quality in the future.
    \item Reduce look-ahead horizon: reduce the number of chunks we need to enumerate.
    \item Consider adjacent chunks as a whole: reduce the number of calculation we need to recalculate it bandwidth allocation.
\end{itemize}

\begin{figure}[t]
    \includegraphics[width=1.0\linewidth]{fake_graphs/end-to-end.pdf}
    \caption{Deploying \name to a video streaming system: \name collects the player status from the client, including video session time, resolution, buffer length etc., and learn per-user QoE model. The bandwidth capping module uses the per-user QoE model to allocate the bandwidth to the client for either training per-user QoE model or optimizing video QoE.}
    \label{fig:e2eprocedure}
\end{figure}

So far we have shown that there is substantial user heterogeneity in QoE. %knowing of the user QoE preference heterogeneity will improve user QoE.
To leverage user heterogeneity, we present the design and implementation of \name, a bandwidth-control system that can learn per-user QoE model and optimize user QoE by controling bandwidth.
In this section, we describe the setting and problem formulation of \name (\S\ref{subsec:design:formulation}), then discuss two important baselines that illustrate the key challenges (\S\ref{subsec:design:baselines}), and finally present our algorithm of QoE profiling and optimization in (\S\ref{subsec:design:balancing},\ref{subsec:design:noise}).


\subsection{Problem formulation}
\label{subsec:design:formulation}

\mypara{System setting}
Figure~\ref{fig:e2eprocedure} overviews a typical video streaming service where we can deploy \name to profile the QoE preferences of any new user and use the information to optimize user QoE.
Our setting has three properties that make it potentially applicable to service providers (ISPs, CDNs, edge networks, etc) who control the link of a user.
First, unlike Different from the previous study, \name does not directly control the video quality inside the video player but controls bandwidth to indirectly affect the video quality.
Second, we monitor the user engagement ratio\jc{engagement ratio or engagement? please be consistent} as the metric of user QoE instead of soliciting the user rating in an exit-survey after each video session.
This way, we can get a more natural user feedback, since collecting user engagement data is less annoying than directly asking for user rating and can avoid the user providing random feedback.
Third, unlike most prior QoE studies, we do not control when or what videos users watch.

\jc{two questions: we still need the real-time video quality/player status. how do isps, CDNs know that? some traffic analysis techniques to infer qoe? need some citations here. also i don't know if engagement itself is so easy to infer given video traffic is mostly encrypted..}

\jc{we shouldn't be talking about the user study methodology. the system design and how it's used in our user study should be separate}
In this paper, we deploy \name on the client where we can limit the downloading rate of video chunks to control the video quality to simplify the deployment.
When the user joins our study, we limit its XX\% bandwidth, which will give the ability to increase the downloading rate during the whole evaluation process.




At a high level, \name have two main components:

\mypara{Per-user QoE modeling}
Before optimizing the streaming video, we first need to learn the video quality preference for every user.
To learn each user preference, we need to model the user reactions to different quality issues.
In \name, we limit the downloading rate of video chunks to create different types of quality issues. 
The key questions are 
\begin{itemize}
    \item[1.] What quality issues we need to show the users?
    \item[2.] How to create those quality issues by limiting the user bandwidth?
\end{itemize}


\mypara{Dynamic downloading rate limiting}
Once the video quality pattern needed to show the user has been determined, we need to achieve this quality by limiting the user's downloading speed.
As aforementioned, by default the users in our study only have XX\% of their original bandwidth.
It indicates that we have the ability to increase a user's bandwidth from XX\% to 100\% or lower the bandwidth from XX\% to 0\%.
Ideally, since the video players are supposed to be adaptive to the downloading rate, we can set the rate as the bitrate of the video quality we want.
However, in practice, the behavior of video player is more complicated: the video download decision can be affected by many factors, such as historical bandwidth, current video resolution, and player buffer length\cite{?}.
The difficulty is that the player behavior is usually unknown to the bandwidth controller, and we might not be able to obtain video quality as we desire.
We deal with this difficulty in Section~\ref{?}.


\jc{xu, let's move this to later sections}
% \mypara{Quality sensitivity has the same trend across the video content}
% Although the users have different sensitivity to the video quality of the different video content, we show that the users have the same trend of quality sensitivity across different video content.
% To prove this, we select the users who are more sensitive to 0.3--1.0-second rebuffering than 500Kbps low-quality issue in Figure~\ref{fig:types}.
% We use permutation test~\cite{?} to test the hypothesis that those users have a larger QoE drop if a rebuffering event happens.
% The p-value is 0.046 which shows they are clearly from different distributions and indicates that the users have the same trend of QoE preferences across different video content.
% We also verify this on the users who are more sensitive to low-quality issues.
\xu{we could illustrate QoE model inside the per-user modeling part, explain why we use engagement to model QoE.}

\mypara{Per-user QoE model}
Following the practice in previous works~\cite{?}, we use a random forest to train per-user QoE model.
This model takes the video quality as the input variables, and outputs the expected QoE as the output.
The input variables are the video quality of the chunks.
We customize feature selection and criteria at the nodes on each decision tree inside the forest.
To train the QoE model faster, the initial QoE model is a one-size-fits all model.
To avoid the explosion of input due to the large number of video chunks, we divide the video into XX parts, and QoE model will take the quality of each part.
The total number of input variables are XX * 3 = XX.
The video quality of each part includes its average video bitrate, total bitrate switch, total rebuffering time.
The output is the user QoE.
The QoE is bucketized the user engagement into XX classes, and the output is the class who gets the most votes from the decision trees inside the random forest.


Here, we do not build per-user QoE models under the context of video genre, since the quality sensitivity has the same trend across the video content for the users.
Although the users have different sensitivity to the video quality of the different video content, we show that the users have the same trend of quality sensitivity across different video content.
To prove this, we select the users who are more sensitive to 0.3--1.0-second rebuffering than 500Kbps \xu{it should be a range.} low-quality issue in Figure~\ref{fig:types}.
We use permutation test~\cite{?} to test the hypothesis that those users have a larger QoE drop if a rebuffering event happens.
\xu{Explain what is the permutation test, and why we can use it to test the hypothesis. Also, make this hypothesis in a more clear way}.
The p-value is 0.046 which shows they are clearly from different distributions and indicates that the users have the same trend of QoE preferences across different video content.
We also verify this on the users who are more sensitive to low-bitrate and bitrate-switch issues.



\subsection{Baselines of training per-user QoE models}
\label{subsec:design:baselines}

To train per-user QoE models, we need to determine the quality of the videos we need to show the users, \ie when and where we need to add low-quality issues to the video.
Although the previous works~\cite{?} shows the ability of training per-user QoE models, they are not suitable for our scenarios.
The previous literature falls into two main categories:

\mypara{Passive user feedback collection}
The most straightforward method is to passively observe the user engagement ratio to the videos the users watch in their daily life, and then update per-user QoE model after each video session.
To provide best possible video quality, we optimize the video quality for each video session with the up-to-date video session.
In the whole process, the users are not aware of the QoE model training, because the video quality is becoming better over time.

The main drawback of this method is that the training process might take a long time, and many video sessions are optimized by a sub-optimal per-user QoE model under this process.
The reason is that the video player usually avoids the quality issues from happening, and it is hard to learn certain types of quality issues which the users might be not sensitive to.
For example, YouTube players are trying to minimize the rebuffering event~\cite{?} according to the one-size-fits-all QoE models.
However, Section~\ref{?} shows that some users are not sensitive to rebuffering events. 
For those users, we might need many sessions to understand those users' insensitivity to the rebuffering events, and thus for those sessions, we miss the QoE optimization opportunities.
For the new users who just come to the video streaming service, a XXX QoE drop could lower XXX chance of continuing to use the service, and it might translate to XXX loss in profit.


\mypara{Active user feedback collection}
Compared with silently collecting user feedback, another extreme is that \emph{can we actively customize video quality for fast learning per-user QoE model}.
Previous works show this idea by active learning: for each update of the per-user QoE model, we use the video quality that can contribute most to the convergence of the model, \ie the video with the largest uncertainty.

This method is problematic: the video quality patterns with the largest uncertainty are usually with bad video quality.
To accelerate the convergence of model training, the past active learning-based methods usually encapsulate multiple types into one video.
Thus, it will severely impair the video quality and deter the new users from using the video service.

\xu{We might need a name for those baselines instead of just naive AL, natural ABR, etc...}

\subsection{Balancing training speed and video quality}
\label{subsec:design:balancing}

From the lessons of the previous works, fast training speed usually brings unsatisfied video quality.
Thus, our objective is to fast learn the per-user models without impairing the user QoE too much, \ie we want to find a rate-limiting scheme $B(t)$ that can output a video quality pattern $v$ with the maximal sum of QoE and the amount of information contributing to the QoE model training (\ie uncertainty).
\xu{rate-limiting, bandwidth-capping, bandwidth-control. which one is the better term?}
\begin{align}
    &\argmax_B \{QoE(v)+Uncertainty(v)\}, \\
   s.t. \quad & bitrate_v(t) < B(t) \quad \forall \text{time } t, \\
   		& average\_bandwidth(B) < \text{Rate limitation}, 
\end{align}
where $B(t)$ represents the downloading rate at time $t$, $Uncertainty(\cdot)$ is the uncertainty of the given video quality pattern, and $QoE(\cdot)$ is the per-user QoE model, and the average bitrate of $v$ must be smaller than the downloading rate limited by \name.
In this paper, we are training per-user QoE model by customizing the existing QoE model instead of inventing a new QoE model.
% Following the practice in previous works~\cite{?}, we use a random forest to train per-user QoE model.
% This model takes the video quality as the input variables, and outputs the expected QoE as the output.
% The input variables are the video quality of the chunks.
% We customize feature selection and criteria at the nodes on each decision tree inside the forest.
% To train the QoE model faster, the initial QoE model is a one-size-fits all model.
% To avoid the explosion of input due to the large number of video chunks, we divide the video into XX parts, and QoE model will take the quality of each part.
% The total number of input variables are XX * 3 = XX.
% The video quality of each part includes its average video bitrate, total bitrate switch, total rebuffering time.
% The output is the user QoE.
% The QoE is bucketized the user engagement into XX classes, and the output is the class who gets the most votes from the decision trees inside the random forest.
The uncertainty of a video quality pattern means how much the QoE model are not sure about classifying this pattern.
The larger uncertainty of a video sample indicates more information that can contribute the QoE model training.
In this paper, we use the minimal margin~\ref{?} to quantify the video uncertainty, \ie the vote difference between the class with the most votes ans the class with the second most votes.
\xu{we should also introduce the definition of regret here.}


The naive solution is that when downloading a chunk, we set the bandwidth to the bitrate we want to obtain in $v$.
However, if we do so, the user perceived video quality might have much larger regret than we expect!
For example, if we want to provide the QoE model with the information about video quality dropping from 720p to 480p, in practice there is a chance to get a rebuffering event instead of a 360p chunk.
If the QoE model already has the information about rebuffering event, such a video quality pattern cannot contribute the uncertainty and good video quality.

To address this issue, we need to consider the behavior of the player into account.
We formulate the problem in Eq.~\ref{?}, \ie \emph{find a rate-limiting $B(t)$ scheme that can minimize the expected regret}:
\begin{align}
  \quad&\argmax_{B} \sum_{v}p\left(B, v\right)*\left(QoE\left(v\right)+Uncertainty\left(v\right)\right) \\
  \textbf{s.t.  } \quad & bitrate_v(t) < B(t) \quad \forall \text{time } t, \\
  &average\_bandwidth(B)\leq \text{Rate limitation}
\end{align}
where $B$ is the rate-limiting scheme (\ie the downloading over time). 
We define $p(B,v)$ as the probability that the video quality pattern $v$ appears under the rate-limiting scheme $B$.

Other than taking player's behavior into account, another benefit of such formulation is that we do not need a clear boundary between the model training and the QoE optimization stages, regarding that verifying whether the model is converged is also not an easy problem.
With more video sessions, the per-user QoE model is getting converged, so that the portion of uncertainty is becoming marginal, and minimizing regret will be automatically converted to QoE optimization.


\subsection{Predict player's behavior}
\label{subsec:design:noise}

Although we do not know the exact decisions of the video players, we can still the desired video quality get to some extent.
There are two questions:
\begin{itemize}
    \item Can we finally get the desired video quality by changing bandwidth?
    \item How long the player need to adapt to the video quality we desire? 
\end{itemize}
To answer this two questions, we check the traces in our dataset.
In our dataset, we find the video sessions which have bandwidth change, and then examine the percentage of the video sessions that the player can eventually adapt to the changed bandwidth, and how long it will take.
In Figure~\ref{?}, we can see that for more than XXX\% cases, the player can adapt to the video quality within in XXX seconds.
\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\linewidth]{fake_graphs/time_to_bounce_back.pdf}
    \caption{The distribution of the player needs to adapt its quality to the bandwidth we set. We set the player status as XX bitrate and XX second buffer length. We enumerate the change of the bandwidth change in [XX, XXX, XX, ...]Kps, and for each change, we run XXX times.}
    \label{fig:my_label}
\end{figure}


\mypara{Profiling player behavior}: 
To solve the formulation in Eq.~\ref{?}, we need to calculate the probability of a video quality pattern $v$ under a given rate-limiting scheme $B$.
\xu{where we define the term ``video quality pattern" first? Maybe we should say it some places in section 2.}
When the bandwidth is constant, the video quality is usually the closest bitrate that is no larger than the bandwidth.
When the bandwidth varies overtime, it is not trivial to predict the quality of next chunks as shown in Figure~\ref{?}.
At high level, we have two ways to solve this problem: 
\begin{itemize}
    \item[(1)] We can directly ask the player developers for the decision making details.
    \item[(2)] We can profile the player's behavior, \ie given the player status, the probability of the quality of the next downloaded chunk.
\end{itemize}

In this paper, we use method (2).
We profile the probability of a player state changing to another under bandwidth $B$, \ie $D(s_1, s_2, b)$, where $s_1$ and $s_2$ represents the player states, including current bitrate, buffer length, the past bandwidth.
To obtain the transition probability between $s_1, s_2$ under bandwidth $b$, we set the player state to $s_1$ under bandwidth $b$ for 100 times, and $D(s_1, s_2, b)$ is the times of the states becoming $s_2$ divided by 100.
Due to the infinite number of all possible player states and bandwidth, we bucketize the bitrate, buffer length and bandwidth for every 200Kbps, 1 second and 200Kbps respectively.
\xu{be more clear about what traces are using and the setting}

When we need to decide the bandwidth when we download chunk $m$, we can first enumerate all possible bandwidth allocations schemes, and calculate the possible video quality patterns and the corresponding probability regarding the current player status.
We then find the bandwidth scheme that is with the minimal expected regret.

\subsection{Saving computation cost}
To calculate the expected regret of a rate-limiting scheme, we might need to enumerate all possible video quality pattern under this scheme.
It is costly prohibitive if we enumerate all the quality patterns due to the large number of the future chunks.
To save the cost, we need to reduce the number of patterns we need to enumerate.
\begin{itemize}
    \item Reducing looking-ahead horizon: When determine the bandwidth of downloading a chunk, we do not need to enumerate all possible quality of the future chunks.
    We can only look ahead for a few number of future chunks and enumerate their quality.
    For the later chunks, we assume the player will perfectly adapt to the bandwidth we set.
    In \name, the looking-ahead horizon is XXX, and we evaluate the choice in Section~\ref{?}
    \item Considering adjacent chunks as a whole: Usually, the length of a chunk in the video streaming services is from XXX to XXX seconds.
    From Figure~\ref{?}, we can see that only XX\% cases can adapt to the desired bitrate within a chunk's time.
    So, we can consider the quality of several adjacent chunks a whole, and it can reduce the time of enumeration.
    For example, for a 60-second long video with 3-second chunk size, we need to enumerate 60/3=20 times, while if we consider 4 adjacent chunks as a whole, we only needs to enumerate 60/(3*4) = 5 time, which saves more than 400\% computation cost.
\end{itemize}



% \begin{algorithm}[t]
%  \KwData{QoE model $Q$}
%  \KwData{Uncertainty calculator $U$}
%  \KwData{the quality of $m$ downloaded chunks $q_1, q_2, \dots, q_{m-1}$}
%  \KwData{Player behavior profile $D$}
%  \KwResult{Downloading bandwidth of the next chunk}
%  $\mathcal{B}\leftarrow$ the set of all possible combinations of downloading throughput for the future chunks\;
%  minimal regret, bw plan $\leftarrow 0, Null $\;
%  \For{ $B$ in $\mathcal{B}$} {
%     Possible video quality patterns and probability $\leftarrow$ $P(B)$\;
%     expected QoE $\leftarrow 0$\;
%     \For{$v$ in Possible video quality patterns}{
%          expected QoE $+= v_{prob}*(Q(\{q-1, \dots, q_{m-1}, v_{quality}\}) + U(v_{quality}))$\;
%     }
%     \uIf{expected QoE > minimal regret}{
%          minimal regret $\leftarrow$ expected QoE\;
%     }
%  }
%  \textbf{return} The downloading rating for chunk $m$ in bw plan\;
%  \caption{Determine the downloading bandwidth for the chunks}
% \end{algorithm}


% \begin{algorithm} 
% 	\caption{Bandwidth of downloading $m$-th chunk} 
% 	\label{alg3} 
% 	\begin{algorithmic}
% 	    \REQUIRE QoE model $Q$, Uncertainty calculator $U$, the quality of $m$ downloaded chunks $q_1, q_2, \dots, q_{m-1}$, Player behavior profile $D$, current player status $S$
% 	    \ENSURE bandwidth of downloading the $m$-th chunk.
% 	    \STATE fidn thelk
% 	    \FORALL{rate-limiting scheme $B$}
% 	    \STATE haha
% 	    \ENDFOR
% 		\STATE $y \gets 1$ 
% 		\IF{$n < 0$} 
% 		\STATE $X \gets 1 / x$ 
% 		\STATE $N \gets -n$ 
% 		\ELSE 
% 		\STATE $X \gets x$ 
% 		\STATE $N \gets n$ 
% 		\ENDIF 
% 		\WHILE{$N \neq 0$} 
% 		\IF{$N$ is even} 
% 		\STATE $X \gets X \times X$ 
% 		\STATE $N \gets N / 2$ 
% 		\ELSE[$N$ is odd] \STATE $y \gets y \times X$ 
% 		\STATE $N \gets N - 1$ 
% 		\ENDIF 
% 		\ENDWHILE
% 		\STATE\quad
% 		\STATE \textbf{function} expected$\_$regret($B, \{q_1, \dots, q_m\}, D, S$):
% 		\FORALL{bandwidth }
% 		\ENDFOR
% 		\STATE \textbf{return} fee
% 	\end{algorithmic} 
% \end{algorithm}

%  fig 1: change to three rows of subfigs. each row is a dataset.

%  fig 2/3: arrows in the corner. Put ours and waterloo datasets in different subfigures.
%  fig 2/3: information of arrows could also be in the axis labels.
%  subsection about why we can model QoE for different video content. put to 3.1 problem setting. 
%  fig 4/5: maybe we can restrict it to the video sessions with a single quality issue.
%  fig 4/5: maybe an ABR algorithm for a case study.

%  eval: mem effect simulation. 

% justify why we use user engagement as the QoE feedback in QoE model. how to justify it can not be affected by video content too much. 

% distribution of average bandwidth for different sessions.
% imperically it is a corner case, and even if that happens, it has a small impact.

==> short_abstract.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


% \begin{abstract}
% Users have significant heterogeneity in perceiving the same video quality, and such heterogeneity provides a new opportunity to optimize user expereice of quality (QoE).
% To exploit such heterogeneity, a missing part is how to automatically model the QoE preference on video quality for every new user.
% To find out an effective QoE modeling scheme, we need a platform to faithfully compare their performance.
% The conventional evaluation approaches use lab-based user study or analysis based on historical data.
% However, their evaluations are biased, because they do not use the data collected from the new user's naturalistic environment of viewing videos.
% In this paper, we propose an evaluation platform, \name, based on in-situ (a.k.a in-the-wild) study, to collect data in users' everyday lives.
% We made many designed choices to guarantee an unbiased comparison between the schemes, like randomized A/B test etc.
% We also validate \name by evaluating three QoE modeling schemes.
% \end{abstract}

% \begin{abstract}
% Conventional approaches to optimize user quality of experience (QoE) for online video streams typically consider certain aspects of heterogeneity, including the content of the video and the devices being used to watch the video.  
% Yet, existing video delivery systems have ignored one of the biggest sources of heterogeneity in video QoE: the quality preferences of \emph{individual} users.
% Previous work has suggested the schemes of modeling per-user QoE preferences, and yet the challenge of unbiasedly evaluating the effectiveness of those schemes deployed in a new user's everyday life remained as an open problem.
% To address this problem, this paper presents \name, a platform that can unbiasedly evaluate the QoE modeling schemes {\em in situ} instead of costly and biased lab-based study.
% We validate \name by evaluating two conventional as well as one proposed QoE modeling schemes.
% The results show by exploiting QoE heterogeneity we can improve QoE (measured in engagement) by XXX\% with the same bandwidth or save XXX\% bandwidth while maintaining the same QoE.
% \end{abstract}

\begin{abstract}
% Conventional approaches to optimize user quality of experience (QoE) for online video streams typically consider certain aspects of heterogeneity, including the content of the video and the devices being used to watch the video.  
% Yet, existing video delivery systems have ignored one of the biggest sources of heterogeneity in video QoE: the quality preferences of \emph{individual} users.
% Previous work has suggested the schemes of modeling per-user QoE preferences, and yet the challenge of unbiasedly evaluating the effectiveness of those schemes deployed in a new user's everyday life remained as an open problem.
% To address this problem, this paper presents \name, a platform that can unbiasedly evaluate the QoE modeling schemes {\em in situ} instead of costly and biased lab-based study.
% We validate \name by evaluating two conventional as well as one proposed QoE modeling schemes.
% The results show by exploiting QoE heterogeneity we can improve QoE (measured in engagement) by XXX\% with the same bandwidth or save XXX\% bandwidth while maintaining the same QoE.

% Recent work has suggested that leveraging the heterogeneity across the quality preferences of individual users can significantly improve the quality of experience (QoE).
% Although a number of QoE modeling schemes for individual users have been proposed, evaluating the effectiveness of those schemes under the real-world settings for new users remains as an open problem.
% The conventional evaluation methods like lab-based user study and historical data analysis might lead to biased results due to the great difference of the viewing context between the lab or the existing users in the historical data and the new user's real-world setting.
% To address this issue, we propose \name that uses {\em in-situ} user study to unbiasedly evaluate QoE modeling schemes in new users' every lives.
% We use \name to evaluate the effectiveness of two conventional as well as one proposed QoE modeling schemes under the real-world settings. 
% The results show that by exploiting QoE heterogeneity we can improve QoE (measured in engagement) by XXX-21.6\% with the same bandwidth or save XXX-21.2\% bandwidth while maintaining the same QoE.

% Recent work has suggested the great potential of leveraging the video quality preference heterogeneity across users in improving the quality of experience (QoE).
% To unleash this potential, we need to model each user's quality preferences by  the user QoE feedback to the videos with different quality issues, and then deploy the per-user QoE models to the video streaming systems as the optimization objective. 
% We argue that an unbiased effectiveness evaluation of QoE modeling schemes for new users still remains as an open problem.
% Conventional methods that usually rely on lab-based study or offline data analysis cannot directly measure a new user's QoE under the real-world setting, making the evaluation results not valid.
% Until recently, a number of tools are proposed for monitoring the video quality during a video session, but they are not able to add the quality issues curated by QoE modeling schemes.
% In this paper, we propose \name that provides a tool for adjusting video quality in situ without any control over when \& what users watch.
% To avoid the bias caused by the viewing environment and video content, \name randomly determines which QoE scheme to use before each video session.
% Enabled by \name, we evaluate the effectiveness of two conventional as well as one proposed QoE modeling schemes under the real-world settings. 
% The results show that by exploiting QoE heterogeneity we can improve QoE (measured in engagement) by XXX-21.6\% with the same bandwidth or save XXX-21.2\% bandwidth while maintaining the same QoE.

% A recent trend of optimizing the quality of experience (QoE) for online video streams is to leverage the heterogeneity of video quality preferences across the users.
% The success of such an optimization highly depends on the effectiveness of the schemes which learn each user's quality preference (\ie QoE modeling schemes).
% A general procedure of those schemes is to analyze the user QoE feedback to the videos with quality issues (\eg bitrate drop, rebuffering).
% To accelerate the procedure, the schemes usually deliberately add quality issues to the online videos.
% We argue that evaluating those schemes' effectiveness for new users still remains as an open problem.
% Conventional evaluation methods that rely on the existing users' data collected from lab-based user studies or historical viewing experiences might result in bias due to the quality preference mismatch between a new user and the existing users.
% Although some data collection tools can fit new users, they cannot adjust the video quality, which might slow down the modeling procedure.
% In this paper, we propose \name that provides a tool for adjusting video quality in situ without any control over when \& what users watch.
% To avoid the bias caused by the viewing environment and video content, \name randomly determines which QoE scheme to use before each video session.
% Enabled by \name, we evaluate the effectiveness of two conventional as well as one proposed QoE modeling schemes under real-world settings. 
% The results show that by exploiting QoE heterogeneity we can improve QoE (measured in engagement) by XXX-21.6\% with the same bandwidth or save XXX-21.2\% bandwidth while maintaining the same QoE.


% A recent trend of optimizing the quality of experience (QoE) for online video streams is to leverage the heterogeneity of video quality preferences across the users.
% The success of such an optimization highly depends on the effectiveness of the schemes which learn each user's quality preference (\ie QoE modeling schemes).
% To evaluate effectiveness, conventional evaluation methods rely on analyzing existing users' data collected from lab-based user studies or historical viewing history.
% However, those methods' evaluation could be biased on new users due to the quality preference mismatch between a new user and the existing users. 
% Although some tools can collect and analyze data for new users, they cannot adjust the video quality for QoE modeling schemes to elicit user preferences.
% In this paper, we propose \name that provides a tool to adjust video quality in situ without any control over when \& what users watch.
% To avoid the bias caused by the viewing environment and video content, \name randomly determines which scheme to evaluate before each video session.
% Enabled by \name, we evaluate the effectiveness of two conventional as well as one proposed QoE modeling schemes under real-world settings. 
% The results show that by exploiting QoE heterogeneity we can improve QoE (measured in engagement) by XXX-21.6\% with the same bandwidth or save XXX-21.2\% bandwidth while maintaining the same QoE.

% A recent trend of optimizing the quality of experience (QoE) for video streaming services is to leverage the heterogeneity of video quality preferences at the granularity of {\em individual} users.
% Despite prior work has studied QoE customization schemes for learning and exploiting per-user quality preferences, the effectiveness of those schemes is still not clear.
% The missing piece is a platform that allows service operators to test the QoE customization schemes for new users.
% It is challenging because the QoE customization schemes need to have online interactions with each new user's video sessions for adjusting video quality and collecting the corresponding user QoE feedback, while all existing work falls short.
% In this paper, we present the design, implementation and early deployment of \name, a platform that enables the operators to test QoE customization schemes in an unbiased manner.
% As a case study, we test three QoE customization schemes on \name, which offers the insights that we can improve QoE (measured in engagement) by XXX-21.6\% with the same bandwidth or save XXX-21.2\% bandwidth while maintaining the same QoE by exploiting the user preference heterogeneity.

% A recent trend of optimizing quality of experience (QoE) of videos is to leverage the heterogeneity of video quality preferences across {\em individual} users.

A recent trend of online video optimization in quality of experience (QoE) is to leverage the heterogeneity of quality preferences across {\em individual} users.
Although these efforts have suggested the great potential of online QoE customization by individual users' quality preferences, network operators still have not deployed them to realize the promised QoE improvement.
The missing piece is a platform that allows operators to test the effectiveness of these QoE customization schemes on new users.
Such a platform is challenging because those QoE customization schemes need to interact online with new users to collect QoE feedback and adjust video quality to learn a new user's quality preferences or optimize the video QoE.
Unfortunately, existing work like lab-based user studies usually do such testing offline and thus extending to new users is a challenge.
In this paper, we present the design, implementation, and early deployment of \name, a platform that enables network operators to test QoE customization schemes online while minimizing bias.
As a case study, we test two strawman QoE customization schemes --- one is to maximally optimize QoE by inaccurate user preference, and the other is to aggressively lower video QoE for fast preference learning --- on \name under real-world settings and then propose a preliminary solution to address the shortcomings of the two strawmen. 
Our insight is that compared to the strawman schemes, we can further improve QoE (measured in engagement) by 13.9\% with the same bandwidth or conversely save 17.3\% bandwidth while maintaining the same QoE.




\end{abstract}

% \begin{abstract}
% Conventional approaches to optimize user quality of experience (QoE) for
%     online video streams typically consider certain aspects of heterogeneity,
%     including the content of the video and the device being used to watch the
%     video.  Yet, existing video delivery systems have ignored one of the biggest
%     sources of heterogeneity in video QoE: the quality preferences of
%     \emph{individual} users.  We demonstrate, using three independent
%     datasets, that users exhibit considerable heterogeneity in QoE, even when
%     watching the same video, on the same device, with the same video quality.
%     Previous work has suggested that such heterogeneity can be exploited to
%     improve QoE, and yet the challenge of automatically learning user QoE
%     preferences without imposing undue burden on the user has remained an open
%     problem.  To address this problem, this paper presents \name, a
%     bandwidth-control system which, for each new user, automatically adjusts
%     throughput during each video session to (1)~learn the user's unique QoE
%     model and (2)~optimize resource allocation in accordance with these
%     preferences.  One significant challenge involves quickly reducing model
%     uncertainty (which requires subjecting the user to sub-optimal video
%     quality) without unacceptably degrading the user's overall experience.
%     To address this challenge, \name frames this problem in terms of
%      the well-studied framework of regret minimization: for each video
%     session, \name selects video quality that minimizes the
%     ``regret'' on the current session's QoE (\ie gap to the best possible
%     quality) and on future video sessions' QoE (\ie inaccuracy of QoE model).
%     To evaluate \name in a real-world setting, we implemented a browser-based
%     user-study platform, deployed it to 15 users, and tested \name against
%     baseline resource allocation strategies
%     for four months.  The results show that \name can
%     improve QoE (measured in engagement) by 13.9\% with the same bandwidth or
%     save 17.3\% bandwidth while maintaining the same QoE.
% \end{abstract}


==> short_eval.tex <==
\tightsection{Evaluation}
\label{sec:eval}

We use \name to test two natural QoE customization schemes (GreedyOpt and GreedyPF) and our proposed ``Balance" described in \S~\ref{sec:short_modeling}.
The key result is that compared to the two natural schemes, we can further improve QoE by 13.9\% with the same bandwidth or save 17.3\% bandwidth while maintaining the same QoE.

\tightsubsection{Setup}

% As described in \S\ref{sec:design_choices}, for a fair comparison, when a video session begins, we randomly determine which scheme is going to be used for this session.
% After each session, we record video engagement (\ie the ratio of video session time and video length) as the user QoE.
% We compare three QoE modeling baselines with the default ABR without any intervention (NoOpt, \ie no per-user QoE optimization) in terms of the average QoE across the users under a fixed average bandwidth throttling rate of 60\% (\S\ref{sec:impl}). 

\begin{table}[t]
\begin{tabular}{|ll||ll||ll|}
\hline
Age      & \# & Gender & \# & Internet plan & \# \\
\hline
21 to 29 & 4  & Female & 7  & 25Mbps                                                                      & 12 \\
% \hline
30 to 39 & 8  & Male   & 8  & 50Mbps                                                                      & 3  \\
% \hline
40+      & 3  &        &    &                                                                             &   \\
\hline
\end{tabular}
\vspace{1em}
\caption{User Demographics in user study}
\vspace{-2em}
\label{tab:userstats}
\end{table}

\begin{figure*}[t]
\begin{minipage}{\linewidth}
      \centering
      \begin{minipage}[t]{0.28\linewidth}
          \vspace{0pt}
        \begin{figure}[H]
            \includegraphics[width=1.0\linewidth]{graphs/evaluation/qoe_overtime.pdf}
            \caption{Average QoE over time across users of the QoE customization schemes and the default ABR with no intervention.}
            \label{fig:qoe_gain}
        \end{figure}
      \end{minipage}
      \hspace{0.005\linewidth}
      \begin{minipage}[t]{0.28\linewidth}
         \vspace{0pt}
        \begin{figure}[H]
            \includegraphics[width=1.0\linewidth]{graphs/evaluation/bw_saving.pdf}
            \caption{Average QoE across users vs. Average throughput buckets during the first 60 sessions of each user.}
            \label{fig:bw_saving}
        \end{figure}
      \end{minipage}
      \hspace{0.005\linewidth}
      \begin{minipage}[t]{0.2\linewidth}
          \vspace{0pt}
        \begin{figure}[H]
            \includegraphics[width=1.0\linewidth]{graphs/evaluation/al_paramenter.pdf}
            \caption{GreedyPF's QoE vs. \# videos for training.}
            \label{fig:al_parameter}
        \end{figure}
      \end{minipage}
    \hspace{0.005\linewidth}
      \begin{minipage}[t]{0.18\linewidth}
         \vspace{0pt}
        \begin{figure}[H]
            \includegraphics[width=1.0\linewidth]{graphs/evaluation/cdf_time_bounce.pdf}
            \caption{CDF of player's adaption time to bandwidth change}
            \label{fig:time_to_change}
        \end{figure}
      \end{minipage}
\end{minipage}
\end{figure*}

We conduct user study on the participants recruited from Prolific~\cite{prolificlink} and Amazon MTurk~\cite{mturklink}.
The demographics is in Table~\ref{tab:userstats}.
In the pre-screening stage, we paid participants $\$10$ for completing the filtering survey and installing the browser extension in accordance with the minimum wage. 
Participants also received an additional $\$2$ a week for each week they remained in the study with our browser extension running. 

We compare three QoE customization schemes in~\S\ref{sec:short_modeling} with the baseline (NoOpt) that we do not have any intervention on the video quality.
This baseline represents the default ABR performance without leveraging the user QoE heterogeneity.




% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.8\linewidth]{graphs/evaluation/qoe_overtime.pdf}
%     \caption{Improvement of average QoE over time across users of the baselines of QoE modeling scheme and the default ABR with no intervention.}
%     \label{fig:qoe_gain}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.8\linewidth]{graphs/evaluation/bw_saving.pdf}
%     \caption{Average QoE across users vs. average throughput buckets during the first 60 sessions of each user.}
%     \label{fig:bw_saving}
% \end{figure}

\tightsubsection{Overall performance}

\mypara{QoE improvement}
Figure~\ref{fig:qoe_gain} shows how average QoE of different schemes improves as a user watches more videos.
Balance can quickly build a reliable per-user QoE model with a marginal QoE degradation in the first few sessions after a new user joins the service.
For the first 60 sessions, Balance achieves on average $9.2-21.6\%$ higher QoE than the others under the same average bandwidth limit.
GreedyPF has much worse QoE than other methods during first 30 sessions when it builds the QoE model, but after that, it has the similar QoE as Balance.
The video QoE of GreedyOpt is not as high as Balance, since it uses sub-optimital QoE model to optimize user QoE.
Note that no matter what scheme we use, both of them can improve user QoE than NoOpt.
% Maybe we need to refer to the appendix for the details.


\mypara{Bandwidth saving}
Next, we run the same real-world test in Figure~\ref{fig:qoe_gain} but with different limits on average bandwidth usage.
Figure~\ref{fig:bw_saving} shows the average bandwidths and the corresponding average QoE of different schemes during the first 60 video sessions after these schemes take effect. 
We can see that Balance can save $17.3-21.2\%$ bandwidth while achieving similar QoE compared to other baselines.
At the same time, we notice that under low the available bandwidth (\eg $250 Kbps$), GreedyPF achieves similar QoE as Balance and GreedyOpt, because such low bandwidth would naturally create various types of quality issues in the video quality patterns, so GreedyPF does not pay extra QoE penalty to build per-user QoE models.



\tightsubsection{Microbenchmarks}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.7\linewidth]{graphs/evaluation/al_paramenter.pdf}
%     \caption{GreedyPF's QoE vs. \# videos for training.}
%     \label{fig:al_parameter}
% \end{figure}


\mypara{GreedyPF's training set size}
If we can use fewer video sessions to train the per-user QoE model by GreedyPF, we might mitigate GreedyPF's severe QoE degradation.
Figure~\ref{fig:al_parameter} shows the QoE in the optimization stage when we vary the number of videos for QoE modeling by deploying GreedyPF to real users.
We can use 30 videos to do QoE modeling for obtaining high QoE in the optimization stage while degrade less QoE during QoE modeling.

\mypara{Player's adaption time to bandwidth change}
Figure~\ref{fig:time_to_change} shows how much time the player can adapt its bitrate to the changed bandwidth.
The data in this figure are collected from the video sessions in Figures~\ref{fig:qoe_gain}, \ref{fig:al_parameter}, and \ref{fig:qoe_gain} when the QoE customization schemes need to change the video quality in the middle of those sessions, and thus it covers a wide range of video quality change.
We can see that the median time of bandwidth adaptation for the player is 16.7 seconds.
It confirms the predictability of proposed by prior ABR logic reverse engineering work~\cite{licciardello2020understanding}.

==> short_framework.tex <==

\tightsection{Evaluating QoE Modeling Schemes}
\label{sec:impl}

In this section, we present a platform that enables the evaluation between different online QoE modeling schemes.

\subsection{Design requirement}

% Three points: Fair, agnostic to user specific factors, reusable

We argue that an platform that can automatically evaluate different QoE modeling schemes on new users should be 1) fair to different schemes; 2) no bias on user-related factors; and 3) easy to deploy.

A fair comparison needs each individual user needs to be under the same context (\eg video viewing devices) when watching the videos generated by different schemes.
Lab-based study is an extreme example that strictly ensures the fairness: For difference schemes, their curated videos shown to the users are with the same content and watched in the same physical place~\cite{duanmu2019sqoe4,?}.

The evaluation should not be biased by other QoE-related factors except video quality, such as video content interestingness~\cite{zhang2021sensei}, context factors~\cite{?}, etc.
Lab-based study is biased by video interestingness: If a user is not interested in the content of the curated videos, it unlikely tells the video QoE difference between different schemes~\cite{zhang2021sensei}.
Offline-analysis in which we can simulate the video quality patterns generated from different schemes by searching the similar ones in a user's historical data is still biased.
We cannot simply extend the results to new users, because it is based on an implicit assumption: we can always find an exiting user who has very similar QoE preference to the new user, which is not always true.

Deployability is also important, because we need to run the evaluation when new users or schemes come.
Apparently, lab-based study is costly, since it has to repeatedly gather every new users in the same place.



% The framework of per-user QoE modeling is in Figure~\ref{?}.
% This framework contains a logical controller (which could be operated by a service provider or by the player) that decides the video quality in each video session.
% Different from other online QoE monitoring platforms~\cite{?} that collect video quality data for offline analysis, our platform can dynamically change the video quality within a video session based on the video quality of downloaded chunks.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.9\linewidth]{fake_graphs/online-framework.pdf}
%     \caption{Framework of online QoE modeling and optimization.}
%     \label{fig:online-framework}
% \end{figure}


\subsection{Design choice}
Generally, to meet the requirements we evaluate the schemes {\em in the wild}, \ie we embed the evaluation into the users' everyday lives: they can watch any videos they like on their own devices, and we do interfere with any QoE factors other than video quality (\eg use user engagement as the QoE metric).

\mypara{Fairness and Bias-avoiding}
There is a trade-off between fairness and bias-avoiding: To avoid any possible bias, we need to conduct the user study in the wild, but it is hard to guarantee every scheme is running under the exact same environment.
We choose the following settings to balance fairness and bias.

{\em No control and data collection on when \& what users watch}:
To avoid the QoE preference bias due to the interestingness of video content, we do not have any control and data collection on when and what users watch, given that we might have no prior knowledge of a new user's interest.
It is still fair for different schemes, because for any video, it has an equal chance to be customized by anyone of the the schemes (See randomized A/B test below).



{\em User engagement as QoE metric}:
We use user engagement, \ie the percentage of a video watched by the user~\cite{?}, as the QoE metric to avoid the bias caused by user annoyance~\cite{fotrousi2018effect}.
We can collect user engagement without the user's awareness, unlike user rating that requires the user fills out an exit-survey after a video session ends.
User engagement is widely-used in the industry, not only because of its less annoyance, but also the direct relation to the revenue.
A natural concern regarding this setting is whether user engagement from arbitrary video content are reliable enough to model per-user QoE. 
Intuitively, video content does impact users’ sensitivity to video quality. 
However, in our study, the selection of quality level is totally agnostic to video content. Thus, averaging over a sufficient amount of data can still reliably build per-user QoE models.

{\em Randomized A/B test}:
We borrow the idea from A/B test, \ie randomly determining which strategy to optimize QoE when each video session begins.
It makes our evaluation be agnostic to those schemes, video content and context factors, \ie for every video content and viewing context, each scheme has an equal chance to be chosen.
Thus, it is a fair comparison if the results of each scheme is averaged by a sufficient amount of data.


{\em Recording the context factors}:
We need to minimize the QoE affect form the context factors, although we cannot directly control over the context factors.
For each video session, we can record the following context factors: the player display size (\ie the width and the length of the player in pixel), viewing device, and active status (\ie the player is the active application in the operating system, indicating whether the user was watching the video.). 
To make a fair comparison, those schemes are with the same above-mentioned context factors.
The implementation of context factor monitoring is in Appendix~\ref{?}

% The recordable context factors of platform 
% Throughout the study, for each individual participant, the video sessions generated by different schemes have the same player display size (\ie the width and the length of the player in pixel), viewing device, and active status (\ie the player is the active application in the operating system, indicating whether the user was watching the video.).


% An ideal comparison needs the users to watch the videos under the same context, including viewing device, player display size, or even psychological status.
% However, it is unrealistic even for an in-lab evaluation where the researchers are supposed to more control over those factors.
% In the in-the-wild evaluation, since we are not able to directly control over or even monitor all of those factors, we try our best to keep the monitorable factors the same for different schemes.
% Throughout the study, for each individual participant, the video sessions generated by different schemes have the same player display size (\ie the width and the length of the player in pixel), viewing device, and active status (\ie the player is the active application in the operating system, indicating whether the user was watching the video.).


\mypara{Deployability}
Deployability requires the users can easily participate in the evaluation.
In our design shown in Figure~\ref{?}, the participants only need to install a browser extension on their video viewing devices.
Thus, other than video quality, we do not interfere with the user experience other than video quality, which make its deployment much easier than the lab-based studies.
\xu{add a figure to show the architecture}



% \subsection{How to compare different schemes}

% The main challenge for our in-the-wild comparison is ensuring the fairness between those schemes, since we cannot directly control over the QoE factors (\eg viewing devices, video content, etc.) other than the video quality.


% \mypara{Monitoring the context factors}
% An ideal comparison needs the users to watch the videos under the same context, including viewing device, player display size, or even psychological status.
% However, it is unrealistic even for an in-lab evaluation where the researchers are supposed to more control over those factors.
% In the in-the-wild evaluation, since we are not able to directly control over or even monitor all of those factors, we try our best to keep the monitorable factors the same for different schemes.
% Throughout the study, for each individual participant, the video sessions generated by different schemes have the same player display size (\ie the width and the length of the player in pixel), viewing device, and active status (\ie the player is the active application in the operating system, indicating whether the user was watching the video.).


% \mypara{Randomized A/B test} 
% To mitigate the influence from video content, we borrow the idea from A/B test: we randomly determine which strategy we use to optimize QoE when each video session begins.
% Thus, the evaluation results of each individual scheme are averaged over a sufficient amount of video content that a user like. 
% We make this as a pragmatic choice, because our in-the-wild study cannot control over the video content. 


\subsection{Implementation}

Our design choice is implemented in a specific setting: we control the video quality by bandwidth and conduct the evaluate the schemes by a crowdsourcing-based user study.

% We implement the framework of our in-the-wild evaluation under the following settings.
% \begin{packeditemize}
%     \item No control over the video content: Unlike the in-lab studies that specify the videos to show the users, we do not control and record the video content, which make the users watch any content they like for providing the in-the-wild user feedback.
%     \item User engagement as QoE metric: It is widely-used in the industry, not only because of its less annoyance compared to collecting soliciting user rating, but also the direct relation to the revenue.
%     \item Indirect video quality control by throughput: The commercial video players, such as YouTube and Netflix, do not have open APIs for replacing their default ABR logic. To evaluate different schemes in the wild, we change the video downloading throughput to induce the video player to obtain the desired quality of different schemes.
% \end{packeditemize}

Controlling video quality by the player's ABR logic is an ideal solution, but the commercial video players, such as YouTube and Netflix, do not have open APIs for replacing their default ABR logic, which prevents us doing in-the-wild evaluation.
It is doable, because although the ABR logic is a black box, it is predictable to some extent.
Video player is designed to adapt to the network bandwidth for maximizing user QoE, though the players differ in the adaption speed~\cite{?}, which is agreed by those works that do reverse engineering for ABR logic.
Thus, a video player highly likely adapts to the network bandwidth it has.

This setting can be suitable for network service providers, such as ISPs, CDNs, and edge routers, who control the bottleneck bandwidth of a user. 
The network service providers do not have the access to the video player’s logic but can monitor and control the users’ network connection. 
To obtain the video quality, service providers can use existing techniques to infer video quality by the video streaming traffic~\cite{?}, and use the session time of the video streaming as the user engagement, and can guess the player status with up to 91\% accuracy. 
% need to mention we why we can control the bandwidth.
% In this paper, we focus on modeling and optimizing per-user QoE on YouTube by dynamically changing the user bandwidth.


\begin{table}[t]
\begin{tabular}{|ll||ll||ll|}
\hline
Age      & \# & Gender & \# & Internet plan & \# \\
\hline
21 to 29 & 4  & Female & 7  & 25Mbps                                                                      & 12 \\
% \hline
30 to 39 & 8  & Male   & 8  & 50Mbps                                                                      & 3  \\
% \hline
40+      & 3  &        &    &                                                                             &   \\
\hline
\end{tabular}
\vspace{1em}
\caption{User Demographics}
% \vspace{-2em}
\label{tab:userstats}
\end{table}

\mypara{User study}
We evaluate the schemes on real human users recruited from the crowdsourcing platforms (\ie Prolific~\cite{} and Amazon MTurk~\cite{}) where can provide the users with large diversity.
The demographics of the participants is in Table~\ref{tab:userstats}.

% We recruit the user study participants from Prolific~\cite{?} and Amazon MTurk~\cite{?}.
% They are all from US, and have diversity in terms of age and gender shown in Table~\ref{tab:userstats}. 

In the user study, we first published a filtering survey for pre-screening the users.
The eligible users should suffer video quality issues frequently, indicating that video quality is a significant factor of user QoE.
To avoid the random feedback in the survey, we write a video quality monitor (Implementation details in Appendix~\ref{?}) installed on the participants' browsers to confirm their feedback.
The selected participants should use video streaming services $\geq 10$ hours per week and suffer from quality issues $\geq$20 times per week.

% Then, we modeled and optimized those participants' QoE through the browser extension that changes the downloading throughput according to the schemes we evaluate.
% The detail of controlling the downloading and the implementation of the browser extension are in \S\ref{?} and Appendix~\ref{?} respectively.

% The users should watch YouTube and suffer from quality issues frequently, since the video quality has a little impact on the QoE of a user who does not have video quality issues.
% To avoid the random feedback in the survey, we write a video quality monitor installed on the participants' browsers to confirm their feedback.
% The eligible participants should use video streaming services $\geq 10$ hours per week and suffer from quality issues $\geq$20 times per week.
% Then, we modeled and optimized those participants' QoE through the browser extension that changes the downloading throughput according to the schemes we evaluate.
% The detail of controlling the downloading and the implementation of the browser extension are in \S\ref{?} and Appendix~\ref{?} respectively.

We conducted this user study from September to December 2021 on 6 users from MTurk and 9 from Prolific. 
In the pre-screening stage, we paid participants $\$$10 for completing the filtering survey and installing the browser extension in accordance with the minimum wage in our area. 
Participants were also paid an additional $\$$2 a week for each week they remained in the study with our browser extension running. 

\mypara{Limitations} In this in-the-wild study, we have limited control over the user's network bandwidth and context factors, so we comprise in the following implementation details.

{\em Throughput capping} One implementation limitation is that we cannot freely increase the physical bandwidth as the network providers do.
Although we need to maintain the average throughput of a video session to be complied to the user's internet plan, the schemes might need the flexibility to increase and/or decrease the downloading throughput within a session for affecting the video quality.
Thus, to enable this flexibility, we cannot guarantee the users to use their full bandwidth.
We make a comprise that we use a 60\% throughput capping, \ie to maintain the average bandwidth of each session as 60\% of the full bandwidth.
Although the video sessions might have different full bandwidth, the above-mentioned randomized A/B test ensures that different schemes have a similar distributions of the session bandwidth.

{\em Long user study period}: The other limitation is that a user's QoE preference might change within the month-long period of user study.
Although it is true, it has marginal affects on our evaluation.
First, our evaluation still fairly compares different schemes, since the schemes have the same problem because of the randomized A/B test.
Second, within the user study period, the difference of QoE preference across the users is much larger than that of an individual user in different time periods of the user study.
We evaluate such the difference in \S\ref{?}.

==> short_framework_v2.tex <==
\tightsection{Framework of QoE modeling evaluation}

In this section, we present a framework to evaluate different online QoE modeling schemes on any new users in an accurate, fair and reusable way.
The evaluation framework should enable the users to watch the videos generated from different QoE modeling schemes, and meanwhile, collect the user feedback to help QoE modeling in terms of training or testing of the per-user QoE models.


\tightsubsection{Design requirement}

We argue that an platform framework should satisfy the following three requirements.

\mypara{Collecting everyday experience}
Our framework should directly compare different QoE modeling schemes in a user's everyday life, since a user's QoE preference could vary significantly in different viewing environment.
For example, a user perceive the video bitrate in different ways: a higher sensitivity to bitrate would happen when the user is watching videos on a high-resolution TV~\cite{?}.
\xu{does it only affect researchers? lab-study might not be reusable.}

\mypara{Fair comparison}
Since many factors can affect user QoE preference (\eg video content, viewing environment), our framework needs to align with the QoE factors other than video quality for different schemes.


\mypara{Reusability}
The previous study~\cite{?} has shown that the QoE preferences are significantly different across users and viewing environment.
There is a need of modeling the QoE preferences regularly for any new combination of user and viewing environment.
We need to minimize QoE modeling's cost for scaling it out.


However, the traditional evaluation frameworks cannot achieve the three requirements simultaneously.

\mypara{Lab-based study}
In lab-based study, the users are gathered in the lab and required to watch the same set of curated videos in the same physical place~\cite{?}, and it is suitable to the case where we need to find out the common points of a user's QoE preferences under different environment.
Lab-based study strictly ensures the fairness between different schemes, but its results are biased due to its inexplicit assumption: a user has the same preferences under different environment, which is apparently not true.
Also, the cost is prohibitive if we do the study on every new user.

\xu{if we only care about comparing different schemes under a given environment. Can this conclusion easily extend to a user's everyday life?}


\mypara{Offline analysis}
In offline analysis, we can simulate the video quality patterns generated from different schemes by searching the similar ones in a user’s historical data.
It is reusable and fair, but cannot obtain the user's everyday life experience when we apply those QoE modeling schemes.
However, the analysis could be biased, since we might not always find out an exiting user who
has very similar QoE preference and viewing environment to the new user in the historical data.

\xu{Add a baseline. if a video player/isp naively implement such a platform.}

\tightsubsection{Design choice}

To collect a user's everyday life experience, we need to evaluate those schemes {\em in the wild}, \ie we embed the evaluation into the users' everyday lives.
We choose the following settings: 

{\em No control and data collection on when \& what users watch}:
To avoid the QoE preference bias due to the interestingness of video content, we do not have any control and data collection on when and what users watch, given that we might have no prior knowledge of a new user's interest.
It is still fair for different schemes, because for any video, it has an equal chance to be customized by anyone of the the schemes (See randomized A/B test below).

{\em User engagement as QoE metric}:
We use user engagement, \ie the percentage of a video watched by the user~\cite{?}, as the QoE metric.
Although it is a more noisy metric than user rating collected by an exit-survey after every video session ends, it is still practical.
First, in in-the-wild study, the users might not provide the ratings after a session ends, so that we might not able to collect enough data points to compare different schemes.
\xu{Give an example that the percentage of users would not provide ratings}.
We can collect user engagement without the user's awareness, and thus we can get data after every video session ends.
Second, although it is noisy, user engagement is still highly correlated with user perception~\cite{?}.
Also, it is already widely-used in the industry, not only because of its less annoyance during user feedback collection, but also the direct relation to the revenue.
A natural concern regarding this setting is whether user engagement from arbitrary video content are reliable enough to model per-user QoE. 
Intuitively, video content does impact users’ sensitivity to video quality. 
However, in our study, the selection of quality level is totally agnostic to video content. Thus, averaging over a sufficient amount of data can still reliably build per-user QoE models.


We also use {\em Randomized A/B test} to ensure the fairness.
We borrow the idea from A/B test, \ie randomly determining which strategy to optimize QoE when each video session begins.
It makes our evaluation be agnostic to those schemes, video content and context factors, \ie for every video content and viewing context, each scheme has an equal chance to be chosen.
Thus, it is a fair comparison if the results of each scheme is averaged by a sufficient amount of data.

Note that such design choices also ensure the reusability, since the users do not need to put much effort in the evaluation, which minimizes thew cost: the users neither need to go to the lab nor fill out the exit-survey.

It can benefit various users of this evaluation framework.

\begin{packeditemize}
\item Researchers: They usually uses a small scale lab-study test different schemes on a set of users~\cite{?}, which cannot be able to tell a user's everday life experience. Our framework offers a much cheaper and more scalable way to test researchers' ideas.
\item Network providers: Network providers have collected a large amount of user data about user engagement and video quality (both can be accurately inferred~\cite{?}), although those data could be biased by the deployed schemes.
(For example, ???)
Our framework offer a control knob (\ie user bandwidth, will describe later) to control the video quality generated from different schemes, and does not need the collaboration from other system parts.
\item Video player providers: For video player providers, ?
\end{packeditemize}


\tightsubsection{An instance of implementation}
\xu{
\begin{itemize}
    \item We target the researchers who do not have the access to the ABR logic and have limited ability to control the user bandwidth.
    \item How to implement? We design a browser extension, which can {\em passively} monitor video quality and user feedback. It can minimize the user effort: the users only need to install the browser extension in the beginning. And it uses bandwidth to affect the video quality.
    Can further ensure the fairness by aligning the viewing environment other than randomized A/B test.
    \item Why bandwidth-controlling work? The video players are designed to be adpative to bandwidth change, although their adaptation speed differs~\cite{licciardello2020understanding}. This assumption is also shared by other work about player reverse engineering.
\end{itemize}
}

% In this paper, we focus on modeling the user preference by controlling user bandwidth, which is suitable for researchers and network providers who do not have the access to the video player's logic.

% Controlling video quality by the player's ABR logic is an ideal solution, but the commercial video players, such as YouTube and Netflix, do not have open APIs for replacing their default ABR logic, which prevents us doing in-the-wild evaluation.
% It is doable, because although the ABR logic is a black box, it is predictable to some extent.
% Video player is designed to adapt to the network bandwidth for maximizing user QoE, though the players differ in the adaption speed~\cite{?}, which is agreed by those works that do reverse engineering for ABR logic.
% Thus, a video player highly likely adapts to the network bandwidth it has.


% We need to minimize the QoE affect form the context factors, although we cannot directly control over the context factors.
% For each video session, we can record the following context factors: the player display size (\ie the width and the length of the player in pixel), viewing device, and active status (\ie the player is the active application in the operating system, indicating whether the user was watching the video.). 
% To make a fair comparison, those schemes are with the same above-mentioned context factors.
% The implementation of context factor monitoring is in Appendix~\ref{?}

\tightsubsection{Deployment}

\xu{
\begin{itemize}
    \item 
\end{itemize}
}

\begin{table}[t]
\begin{tabular}{|ll||ll||ll|}
\hline
Age      & \# & Gender & \# & Internet plan & \# \\
\hline
21 to 29 & 4  & Female & 7  & 25Mbps                                                                      & 12 \\
% \hline
30 to 39 & 8  & Male   & 8  & 50Mbps                                                                      & 3  \\
% \hline
40+      & 3  &        &    &                                                                             &   \\
\hline
\end{tabular}
\vspace{1em}
\caption{User Demographics}
% \vspace{-2em}
\label{tab:userstats}
\end{table}

\mypara{User study}
We evaluate the schemes on real human users recruited from the crowdsourcing platforms (\ie Prolific~\cite{} and Amazon MTurk~\cite{}) where can provide the users with large diversity.
The demographics of the participants is in Table~\ref{tab:userstats}.

% We recruit the user study participants from Prolific~\cite{?} and Amazon MTurk~\cite{?}.
% They are all from US, and have diversity in terms of age and gender shown in Table~\ref{tab:userstats}. 

In the user study, we first published a filtering survey for pre-screening the users.
The eligible users should suffer video quality issues frequently, indicating that video quality is a significant factor of user QoE.
To avoid the random feedback in the survey, we write a video quality monitor (Implementation details in Appendix~\ref{?}) installed on the participants' browsers to confirm their feedback.
The selected participants should use video streaming services $\geq 10$ hours per week and suffer from quality issues $\geq$20 times per week.


\mypara{Throughput capping}: To control the user throughput, we ask the users to install a browser extension that can also monitor the video viewing status. One implementation limitation is that we cannot freely increase the physical bandwidth as the network providers do.
Although we need to maintain the average throughput of a video session to be complied to the user's internet plan, the schemes might need the flexibility to increase and/or decrease the downloading throughput within a session for affecting the video quality.
Thus, to enable this flexibility, we cannot guarantee the users to use their full bandwidth.
We make a comprise that we use a 60\% throughput capping, \ie to maintain the average bandwidth of each session as 60\% of the full bandwidth.
Although the video sessions might have different full bandwidth, the above-mentioned randomized A/B test ensures that different schemes have a similar distributions of the session bandwidth.


==> short_framework_v2_temp.tex <==
\tightsection{Framework of QoE modeling evaluation}

In this section, we present a platform that enables the evaluation between different online QoE modeling schemes in terms of how fast and accurate we can obtain an per-user QoE model.

\tightsubsection{Design requirement}

We argue that an platform that can automatically evaluate different QoE modeling schemes on new users should be 1) an {\em unbiased comparison}; 2) with {\em minimal intervention} in user perception.


\begin{packeditemize}
\item Unbiased comparison: Those schemes' evaluation results should reflect the users' real experience in their daily life.
The reasons are two fold.
First, such a comparison is fair, because all the schemes are evaluated in the same environment.
Second, a user's QoE preference could vary significantly in different environment.
For example, users have different quality requirement in their interested and uninterested content \cite{zhang2021sensei,?}, and users perceive the videos in different ways for different devices (\eg the users might be more sensitive to video bitrate when watching on a high-resolution TV~\cite{?}).
Although lab-based study can make sure a fair environment by forcing the users to watch the same video and sit in the same environment, but it cannot reflect the user experience in real life.

\item +fair comparison

\item Minimal intervention : To make sure the evaluation results reflect their everyday experience, the users should be less aware of our experience. It usually means the cost (in terms of money and user QoE damage) of evaluation is cheap, since we need to model per-user QoE preference for any new user and any new environment.
Although offline-analysis in which we can simulate the video quality patterns generated from different schemes by searching the similar ones in a user’s historical data is with the minimal intervention (we do not need any user effort), it cannot extend to new users and new environment, because it is based on an implicit assumption: we can always find an exiting user who has very similar QoE preference to the new user, which is not always true. 
\end{packeditemize}

\begin{packeditemize}
\item user natural experience 
\item fair experience
\item reusable
\end{packeditemize}

% different compare QoE rating and engagement.

% why the people value control experiment?

\tightsubsection{Design choice}

Generally, to meet the requirements we evaluate the schemes {\em in the wild}, \ie we embed the evaluation into the users' everyday lives: they can watch any videos they like on their own devices, and we do interfere with any QoE factors other than video quality (\eg use user engagement as the QoE metric).

There is a trade-off between fairness and bias-avoiding: To avoid any possible bias, we need to conduct the user study in the wild, but it is hard to guarantee every scheme is running under the exact same environment.

We also do not want to involve too much user effort by constantly watching uninterested videos and providing feedback.

{\em No control and data collection on when \& what users watch}:
To avoid the QoE preference bias due to the interestingness of video content, we do not have any control and data collection on when and what users watch, given that we might have no prior knowledge of a new user's interest.
It is still fair for different schemes, because for any video, it has an equal chance to be customized by anyone of the the schemes (See randomized A/B test below).

{\em User engagement as QoE metric}:
We use user engagement, \ie the percentage of a video watched by the user~\cite{?}, as the QoE metric to avoid the bias caused by user annoyance~\cite{fotrousi2018effect}.
We can collect user engagement without the user's awareness, unlike user rating that requires the user fills out an exit-survey after a video session ends.
User engagement is widely-used in the industry, not only because of its less annoyance, but also the direct relation to the revenue.
A natural concern regarding this setting is whether user engagement from arbitrary video content are reliable enough to model per-user QoE. 
Intuitively, video content does impact users’ sensitivity to video quality. 
However, in our study, the selection of quality level is totally agnostic to video content. Thus, averaging over a sufficient amount of data can still reliably build per-user QoE models.

{\em Randomized A/B test}:
We borrow the idea from A/B test, \ie randomly determining which strategy to optimize QoE when each video session begins.
It makes our evaluation be agnostic to those schemes, video content and context factors, \ie for every video content and viewing context, each scheme has an equal chance to be chosen.
Thus, it is a fair comparison if the results of each scheme is averaged by a sufficient amount of data.

It can benefit various users of this evaluation framework.

\begin{packeditemize}
\item Researchers: Researchers usually want to test a new scheme's performance in various users' everyday life. Our framework provides a cheap and scalable way to test researchers' ideas. Offline traces are hard to obtain, while lab-based study is costly.  sampling bias and cannotextend.
\item Network providers: The network providers can infer the user's engagement and video quality (up to 91\% accuracy~\cite{?}), and it does not need more extra cost to directly control the video player (which they are not able to do either) but can improve the user's QoE by exploiting the per-user QoE model.
\item Player providers:
\end{packeditemize}
% how to use? how to answer some new questions that cannot be answered by the previous alternatives? 
\tightsubsection{An instance of implementation}

In this paper, we focus on modeling the user preference by controlling user bandwidth, which is suitable for researchers and network providers.

Controlling video quality by the player's ABR logic is an ideal solution, but the commercial video players, such as YouTube and Netflix, do not have open APIs for replacing their default ABR logic, which prevents us doing in-the-wild evaluation.
It is doable, because although the ABR logic is a black box, it is predictable to some extent.
Video player is designed to adapt to the network bandwidth for maximizing user QoE, though the players differ in the adaption speed~\cite{?}, which is agreed by those works that do reverse engineering for ABR logic.
Thus, a video player highly likely adapts to the network bandwidth it has.


We need to minimize the QoE affect form the context factors, although we cannot directly control over the context factors.
For each video session, we can record the following context factors: the player display size (\ie the width and the length of the player in pixel), viewing device, and active status (\ie the player is the active application in the operating system, indicating whether the user was watching the video.). 
To make a fair comparison, those schemes are with the same above-mentioned context factors.
The implementation of context factor monitoring is in Appendix~\ref{?}

\tightsubsection{Deployment}

\begin{table}[t]
\begin{tabular}{|ll||ll||ll|}
\hline
Age      & \# & Gender & \# & Internet plan & \# \\
\hline
21 to 29 & 4  & Female & 7  & 25Mbps                                                                      & 12 \\
% \hline
30 to 39 & 8  & Male   & 8  & 50Mbps                                                                      & 3  \\
% \hline
40+      & 3  &        &    &                                                                             &   \\
\hline
\end{tabular}
\vspace{1em}
\caption{User Demographics}
% \vspace{-2em}
\label{tab:userstats}
\end{table}

\mypara{User study}
We evaluate the schemes on real human users recruited from the crowdsourcing platforms (\ie Prolific~\cite{} and Amazon MTurk~\cite{}) where can provide the users with large diversity.
The demographics of the participants is in Table~\ref{tab:userstats}.

% We recruit the user study participants from Prolific~\cite{?} and Amazon MTurk~\cite{?}.
% They are all from US, and have diversity in terms of age and gender shown in Table~\ref{tab:userstats}. 

In the user study, we first published a filtering survey for pre-screening the users.
The eligible users should suffer video quality issues frequently, indicating that video quality is a significant factor of user QoE.
To avoid the random feedback in the survey, we write a video quality monitor (Implementation details in Appendix~\ref{?}) installed on the participants' browsers to confirm their feedback.
The selected participants should use video streaming services $\geq 10$ hours per week and suffer from quality issues $\geq$20 times per week.


\mypara{Throughput capping}: To control the user throughput, we ask the users to install a browser extension that can also monitor the video viewing status. One implementation limitation is that we cannot freely increase the physical bandwidth as the network providers do.
Although we need to maintain the average throughput of a video session to be complied to the user's internet plan, the schemes might need the flexibility to increase and/or decrease the downloading throughput within a session for affecting the video quality.
Thus, to enable this flexibility, we cannot guarantee the users to use their full bandwidth.
We make a comprise that we use a 60\% throughput capping, \ie to maintain the average bandwidth of each session as 60\% of the full bandwidth.
Although the video sessions might have different full bandwidth, the above-mentioned randomized A/B test ensures that different schemes have a similar distributions of the session bandwidth.


==> short_framework_v3.tex <==
\tightsection{Framework of QoE modeling evaluation}
In this section, we present a framework to evaluate online QoE modeling schemes that aims to any new users.
This framework should enable different schemes to show the videos with customized quality as well as collect user feedback to help the schemes in training and testing per-user QoE models.
Our framework should be able to tell how fast we can obtain the per-user QoE models, how accurate those models are and how satisfied with the video quality during the evaluation the users are.

\tightsubsection{Design requirement}

The design of such a framework should satisfy two requirements: fairness and reusability.

\mypara{Fairness}
To ensure a fair comparison, the framework should align the non-video-quality QoE factors for different schemes, since those factors can significantly affect the a user's QoE preference, \eg video content~\cite{?}, viewing context~\cite{?}.
For example, a user could perceive the video bitrate in different ways: a higher sensitivity to bitrate would happen when the user is watching videos on a high-resolution TV~\cite{?}.
For such users, if we force them to watch videos on a low-resolution TV, the evaluation will favor the QoE modeling schemes that aggressively lower the video's bitrate, because those schemes would not lower user's QoE during too much during the evaluation and thus misleads to a conclusion that the users might satisfy with those schemes' video quality.

\mypara{Reusability}
Since the QoE preferences are significantly different across users, we cannot simply assume this user's QoE preferences can match the existing QoE models.
Thus, we need to regularly model QoE preference as long as new users start to use the video streaming service.
It means the framework could be reused for many times to test which scheme is suitable to the new user.
To test schemes on more users, we need to minimize the cost of using this framework.


\tightsubsection{Design choice}

\begin{table*}[t]
\begin{tabular}{|l|l|l|l|}
\hline
 & Non-quality factors & QoE metrics & How to collect QoE feedback \\ \hline
Researchers~\cite{?} & Fully controlled &  Mostly user rating & Lab-based user study\\ \hline
Network providers~\cite{?} & Not controlled & Mostly user engagement &  Offline data analysis\\ \hline
Player providers~\cite{?}  & Not controlled & User engagement\& User rating &  Offline data analysis \\ \hline
\end{tabular}
\vspace{1em}
\caption{Potential users of our evaluation framework and their common-used evaluation settings}
\label{tab:potential_users}
\end{table*}

We then discuss the choices of design this evaluation framework.

\mypara{With or Without control over non-quality factors}
Ideally, we want to compare different schemes under the same settings of non-quality factor ensure fairness.
A straightforward way is to fully control over those factors when the users watch the videos with the quality generated from different schemes, include but not limited to video content, viewing devices, etc.
However, such a full control has prohibitive cost if we want to fix those factors for a large number of users.
To mitigate this problem, during the evaluation, we can have no control over those non-quality factors, \eg when \& what users watch, viewing environment, but keep monitoring those factors.
Then, we can compare the schemes those are run under the same setting of those factors.
Here, we use {\em randomized A/B test} to ensure that for any non-quality factor setting, each scheme has equal chance to execute.
We borrow the idea from A/B test, \ie, randomly determining which scheme to do QoE modeling when each video session begins, which makes our evaluation framework be agnostic to those schemes.

% In-situ study rather than lab-based study, historical data-based analysis
\mypara{User study, or Historical data-based analysis}
For modeling a new user's QoE, we can always have a cost-efficient way --- simulating the video quality patterns generated from different schemes by searching the similar ones in the historical data.
However, the comparison results might not be convincible, since we might not always find out an exiting user who has very similar QoE preference and viewing environment to the new user in the
data we have.
To avoid this case, we need to do user study to obtain the new user's QoE model.
Lab-based user study is widely used in the research community, which the users are gathered in the lab and required to watch the same set of curated videos in the same physical place~\cite{?}.
It is suitable to the case where we need to find out the common points of QoE preferences under the same setting of non-quality QoE factors across the users.
Lab-based study strictly ensures the fairness between different schemes, but its cost is prohibitive if we do the study on every new user.
Also, lab-based study often fails to simulate the real-lie environment, and thus hampers the ecological validity of the results.
In-situ study, {\em a.k.a.,} in-the-wild study, is to embed the evaluation into the users’ everyday lives, and likely to reveal the user experience in naturalistic environments.
Thus, we need to minimize the intervention to the user's everyday life, indicating that we cannot control the non-video-quality QoE factors.

\mypara{User engagement or User rating}
QoE modeling schemes need to train per-user QoE models by the user feedback to the videos with different quality.
Two popular metrics are user rating and user engagement.
User rating is collected by an exit survey after each video session ends.
It is usually used in the lab-based study, where the users are required to provide the ratings, while in in-situ study, the users are likely to skip the survey after a video session, which might cause the insufficiency of user feedback collection.
User engagement, \ie  the percentage of a video viewed by a user~\cite{?}, does not involve the user effort of providing us feedback, which allows us to collect user feedback for every video session.
This metric is widely-used in the industry, not only because of its minimal intervention to user viewing experience, but also the direct relation to the revenue.
A natural concern regarding this setting is whether user engagement from arbitrary video content are reliable enough to model per-user QoE. 
In our study, the selection of quality level is totally agnostic to video content.
Thus, averaging over a sufficient amount of data can still reliably build per-user QoE models.

% in-situ or lab or data analysis
% video session-level randomization
% + control bw rather than bitrate or abr.
% user engagement vs rating.

There are three types of potential users who need to evaluate the QoE modeling schemes, and their traditional design choices are listed in Table~\ref{tab:potential_users}.
\xu{
why the three potential users select the settings (what's their goals?)? and what they miss from the settings?
\begin{packeditemize}
\item Researchers: Researchers usually aim to compare different scheme under different environment, and they choose lab-based study that can control environment. However, the settings 
\item Network providers
\item Video player providers
\end{packeditemize}
}
% \begin{packeditemize}
% \item Researchers: Their . 
% They usually use a lab-based study where test different schemes on a set of users~\cite{?}, which cannot be able to tell a user's everyday life experience. Our framework offers a much cheaper and more scalable way to test researchers' ideas.

% \item Network providers: Network providers have collected a large amount of user data about user engagement and video quality (both can be accurately inferred~\cite{?}), although those data could be biased by the deployed schemes.
% (For example, ???)
% Our framework offer a control knob (\ie user bandwidth, will describe later) to control the video quality generated from different schemes, and does not need the collaboration from other system parts.

% \item Video player providers: For video player providers, the video quality patterns is.
% \end{packeditemize}



\tightsubsection{An instance of framework implementation}

In this paper, we implement the framework for network service providers, such as ISPs, CDNs, and edge routers, who control the bottleneck bandwidth of a user. 
The network service providers do not have the access to the video player’s logic but can monitor and control the users’ network connection.

To obtain the video quality, service providers can use existing techniques to infer video quality by the video streaming traffic~\cite{?}, and use the session time of the video streaming as the
user engagement, and can guess the player status with up to 91\% accuracy.

Although we cannot control or even obtain video content, we can control the video quality by changing users' video downloading bandwidth.
It is doable, because although the ABR logic is a black box, it is predictable to some extent.
Video player is designed to adapt to the network bandwidth for maximizing user QoE, though the players differ in the adaption speed~\cite{?}, which is agreed by those works that do reverse engineering for ABR logics~\cite{?}.


We design a browser extension that can monitor buffer size, video quality, user engagement as well as non-quality QoE factors, including player display size (\ie the width and the length of the player in pixel), viewing device, and active status  (\ie the player is the active application in the operating system, indicating whether the user was watching the video.).
To make a fair comparison, the data collected from those schemes for evaluation are with the same above-mentioned non-quality factors.
The implementation details of the browser extension is in Appendix~\ref{?}

This browser extension can also affect video quality by throttling video downloading throughput.
Because we cannot freely increase the physical bandwidth as the network providers do. 
Although we need to maintain the average throughput of a video session to be complied to the
user’s internet plan, the schemes might need the flexibility to increase and/or decrease the downloading throughput within a session for affecting the video quality. 
Thus, to enable this flexibility, we cannot guarantee the users to use their full bandwidth. We make a comprise that we use a 60\% throughput capping, \ie to maintain the average band-
width of each session as 60\% of the full bandwidth. Although the video sessions might have different full bandwidth, the randomized A/B test ensures that different
schemes have a similar distributions of the session bandwidth.

\begin{table}[t]
\begin{tabular}{|ll||ll||ll|}
\hline
Age      & \# & Gender & \# & Internet plan & \# \\
\hline
21 to 29 & 4  & Female & 7  & 25Mbps                                                                      & 12 \\
% \hline
30 to 39 & 8  & Male   & 8  & 50Mbps                                                                      & 3  \\
% \hline
40+      & 3  &        &    &                                                                             &   \\
\hline
\end{tabular}
\vspace{1em}
\caption{User Demographics}
% \vspace{-2em}
\label{tab:userstats}
\end{table}

Different from the traditional way, we conduct a user study for evaluating the schemes to show the reusability of our framework for the new users.
The participants were recruited from the crowdsourcing platforms (\ie Prolific~\cite{?} and Amazon MTurk~\cite{?}) where can provide the users with large diversity.
The demographics of the participants is in Table~\ref{tab:userstats}.


In the user study, we first published a filtering survey for pre-screening the users.
The eligible users should suffer video quality issues frequently, indicating that video quality is a significant factor of user QoE.
To avoid the random feedback in the survey, we write a video quality monitor (Implementation details in Appendix~\ref{?}) installed on the participants' browsers to confirm their feedback.
The selected participants should use video streaming services $\geq 10$ hours per week and suffer from quality issues $\geq$20 times per week.



==> short_framework_v4.tex <==
\tightsection{QoE modeling evaluation}

In this section, we present a framework, \name, to evaluate online QoE modeling schemes.
By \name, the real human beings can watch the videos that the quality is customized by the schemes for evaluation, and then provide their QoE feedback to help us understand how fast we can obtain the per-user QoE models, how accurate those models are and how satisfied with the video quality during the evaluation the users are.

\tightsubsection{Design Requirement}

To effectively evaluate the QoE modeling schemes, \name should satisfy the following requirements.

\mypara{Unbiased comparison}
An unbiased comparison requires \name to evaluate the schemes under the same context (including video content, viewing device, player display size, etc.~\cite{?}), and this context should be closed to the users' everyday lives.
Since previous study~\cite{?} already shows the context factor can greatly impact the user's QoE preferences, the performance of a scheme would greatly vary under different contexts.
For example, a higher sensitivity to bitrate would happen to some users is when the videos are played on a high-resolution TV rather than a low-resolution one~\cite{?}.
For such users, if we force them to watch videos on a low-
resolution TV, the evaluation will favor those QoE modeling
schemes that aggressively lower the video’s bitrate.

\mypara{Minimal intervention in viewing experience}
Minimizing the intervention indicates that we can loop less efforts of the real human users, and thus minimize the cost of conducting the evaluation.
The cost is important to \name, because we cannot simply assume a new user’s QoE preferences can match some existing QoE models, and we have to regularly model a new user's QoE preference when the user starts to use the video streaming service.


\tightsubsection{Design Choices}
% all important choices here, including bw as QoE metric

% in-situ or lab or data analysis
% video session-level randomization
% + control bw rather than bitrate or abr.
% user engagement vs rating.


We then discuss \name's design choices for for meeting the above-mentioned requirements.

\mypara{In-situ study rather than lab-based study and historical data analysis}
\name uses in-situ study ({\em a.k.a,} in-the-wild study) to minimize the viewing context difference between our evaluation and the users' everyday lives.
It does not control when \& what users watch and the viewing context, and thus it is likely to reveal the user experience in naturalistic environments compared with a lab-based study where the users are gathered in the lab and required to watch the same set of curated videos in the same physical place~\cite{?}.
Lab-based study is suitable to the case where we need to find out the common points of QoE preferences under the same setting of non-quality QoE factors across the users.
Although it strictly ensures the fairness between different schemes, it often fails to simulate the naturalistic environment, which hampers the ecological validity of the results.
Also its cost is prohibitive if we do the study on every new user.
One might argue that user study might not necessary, since we can do offline analysis --- for a video quality pattern generated by a scheme, we can search the similar pattern and the corresponding QoE feedback in the historical data.
However, we might not always find out such a pattern, because we cannot assume there is an exiting user who has very similar QoE preference and viewing environment to the new user.



\mypara{Video session-level randomization}
Video session-level randomization can make sure every scheme has a similar distribution of video content and video viewing context.
In in-situ study, the main problem is that we cannot directly control over the viewing context, so that the evaluation might be biased.
To mitigate this problem, we borrowed from A/B test, \ie, randomly determining which scheme to do QoE modeling when each video session begins, which makes our evaluation framework be agnostic to those schemes.


\mypara{User engagement vs. User rating}
There are two popular QoE metrics: user rating and user engagement.
\name chooses user engagement, \ie  the percentage of a video viewed by a user~\cite{?}.
This metric is widely-used in the industry, not only because of its minimal intervention to user viewing experience, but also the direct relation to the revenue.
A natural concern regarding this setting is whether user engagement from arbitrary video content are reliable enough to model per-user QoE. 
In our study, the selection of quality level is totally agnostic to video content.
Thus, averaging over a sufficient amount of data can still reliably build per-user QoE models.
User rating is collected by an exit survey after each video session ends.
It is usually used in the lab-based study, where the users are required to provide the ratings, while in in-situ study, the users are likely to skip the survey after a video session, which might cause the insufficiency of user feedback collection.
It also involves the user effort of providing us feedback, which significantly increases the cost of conducting user study.


\mypara{Using bandwidth to video quality}
\name uses bandwidth as a knob to indirectly control video quality.
Its benefit is that we do not need to understand the commercial player's ABR logic that is usually not open sourced like YouTube and Netflix. 
Although we still need to predict the ABR logic reaction to different bandwidth, it is doable, because the ABR logic itself is designed to adapt to the network bandwidth for maximizing user QoE, though the players differ in the adaption speed~\cite{?}, which is agreed by those works that do reverse engineering for ABR logic~\cite{?}.


The potential users of \name are network providers, researchers and video player providers.
\begin{packeditemize}
\item {\bf Network service providers} control the bottleneck link of the video streaming system, and thus they concern how to use limited bandwidth resource to more users without degrading user QoE.
They usually optimize the user QoE by the insights found from the historical data~\cite{?} which might be biased for new users.

\item {\bf Researchers} need to compare the performance of different schemes, so that they usually choose a lab-based user study in a fully-controlled environment (including video content and viewing context).
The results might not reflect the condition in real life, and the cost is expensive.

\item {\bf Video player providers} design ABR logic to optimize iser QoE under the restriction of bandwidth. 
They usually conduct lab-based user study or historical data analysis to create QoE models~\cite{?}, and it is hard to extend to new users.

\end{packeditemize}

\name is suitable for network service providers, such as ISPs, CDNs, and edge routers.
The network service providers do not have the access to the video player’s logic but can monitor and control the users’ network connection. 
To obtain the video quality, service providers can use existing techniques to infer video quality by the video streaming traffic~\cite{?}, and use the session time of the video streaming as the user engagement, and can guess the player status with up to 91\% accuracy. 

\tightsubsection{Implementation}

We introduce how to implement our design choices.

\begin{table}[t]
\begin{tabular}{|ll||ll||ll|}
\hline
Age      & \# & Gender & \# & Internet plan & \# \\
\hline
21 to 29 & 4  & Female & 7  & 25Mbps                                                                      & 12 \\
% \hline
30 to 39 & 8  & Male   & 8  & 50Mbps                                                                      & 3  \\
% \hline
40+      & 3  &        &    &                                                                             &   \\
\hline
\end{tabular}
\vspace{1em}
\caption{User Demographics}
% \vspace{-2em}
\label{tab:userstats}
\end{table}

\mypara{Recruiting participants}
The participants were recruited from the crowdsourcing platforms (\ie Prolific~\cite{?} and Amazon MTurk~\cite{?}) where can provide the users with large diversity.
The demographics of the participants is in Table~\ref{tab:userstats}.

In the user study, we first published a filtering survey for pre-screening the users.
The eligible users should suffer video quality issues frequently, indicating that video quality is a significant factor of user QoE.
To avoid the random feedback in the survey, we write a video quality monitor (will introduce soon) installed on the participants' browsers to confirm their feedback.
The selected participants should use video streaming services $\geq 10$ hours per week and suffer from quality issues $\geq$20 times per week.


\mypara{Monitoring video quality}
We design a browser extension that can monitor buffer size, video quality, user engagement.
It also monitors the context factors, including player display size (\ie the width and the length of the player in pixel), viewing device, and active status  (\ie the player is the active application in the operating system, indicating whether the user was watching the video.), to ensure every scheme is evaluated under the same context.
The implementation details of the browser extension is in Appendix~\ref{?}

\mypara{Controlling video quality}
We wrote an browser extension to affect video quality by throttling video downloading throughput.
Because we cannot freely increase the physical bandwidth as the network providers do. 
Although we need to maintain the average throughput of a video session to be complied to the
user’s internet plan, the schemes might need the flexibility to increase and/or decrease the downloading throughput within a session for affecting the video quality. 
Thus, to enable this flexibility, we cannot guarantee the users to use their full bandwidth. We make a comprise that we use a 60\% throughput capping, \ie to maintain the average bandwidth of each session as 60\% of the full bandwidth. 
Although the video sessions might have different full bandwidth, the randomized A/B test ensures that different schemes have a similar distributions of the session bandwidth.

\mypara{Player profile}
Although we do not know the exact logic the player, like previous ABR reverse engineering work~\cite{?}, we can still profile the player's behavior $p(b,v)$ that is the probability that the video quality pattern $v$ appears under a bandwidth allocation plan $b$, \ie the bandwidth allocated to the video session over time.
To obtain $p(b, v)$, we run an exhaustive test to build the transition distribution of $D(s_1, s_2, b)$, where $s_1$ and $s_2$ represents the player states, including current bitrate, buffer length, and $b$ is the current bandwidth.
To obtain the transition probability between $s_1, s_2$ under bandwidth $b$ within 12 seconds\footnote{We use 12 seconds because empirically it is the medium delay between when bandwidth changes and when the video player reacts.}, we set the player state to $s_1$ under bandwidth $b_1$ for 100 times, and $D(s_1, s_2, b)$ is the times of the states becoming $s_2$ divided by 100.
To reduce the search space, we bucketize the bitrate, buffer length and bandwidth for every 200Kbps, 1 second and 200Kbps respectively.



\xu{add limitations to our methods.}

\xu{interface, how to deploy algorithm by the interface we provide,
what do we need to provide for the
}

==> short_framework_v5.tex <==

\tightsection{\name}

\label{sec:framework}

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{graphs/graph/vidhoc_framework.pdf}
    \caption{System overview of \name}
    \vspace{-0.5em}
    \label{fig:framework}
\end{figure}

% To utilize significant QoE heterogeneity across the users (shown in \S~\ref{sec:short_moti}), we propose \name (as shown in Figure~\ref{fig:framework}) to regularly evaluate the effectiveness of the existing and the newly proposed QoE modeling schemes that model the QoE preferences for the new users.
% The real human users can watch any video content at any time and provide their feedback towards the video quality scheduled by \name.
% \name schedules a video's quality pattern (\ie the video quality overtime) in a way of maximizing the pattern's ``importance" (will describe in \S~\ref{sec:short_modeling}) calculated by the QoE modeling scheme.
% In each video session,  \name randomly determines which QoE modeling schemes need to evaluate in the beginning, and then interacts with the scheme by inquiring the importance of the possible quality patterns given the bandwidth limitation of this session.
% After the session ends, \name reports the video quality pattern and user QoE feedback to the scheme which updates the user's QoE model accordingly.

% In this section, we will discuss \name's design and implementation.
    
\name is a platform that enables online tests of QoE customization schemes' effectiveness on new users; the goal of \name is to compare those schemes in an unbiased fashion.

As shown in Figure~\ref{fig:framework}, in a video session \name randomly selects a QoE customization scheme to evaluate and uses the bandwidth knob to schedule a quality setting (\ie, video quality pattern that includes the bitrate, rebuffering time of the video segments over time) determined by the scheme for either per-user QoE modeling or optimization.
Within the session, \name keeps monitoring the player status (\eg buffer length, video bitrate, rebuffering, etc.) and sends reports to the QoE customization scheme, which allows the scheme to change its quality setting.
After the session, the QoE customization scheme can update the user's QoE model according to the video session's quality and the corresponding QoE feedback.
We can repeat this procedure multiple times to compare the QoE of the video sessions customized by other schemes.

% The experimenters can use \name to answer the questions like ``How fast a scheme can model a new user's QoE?", ``How much QoE improvement we can have if we apply the QoE model trained by a particular scheme in the real world?".
% \name provides tools to automatically deploy those schemes on the users with minimal interventions on the viewing experience.

In this section, we will discuss the design and the rationale behind \name by answering the three questions:
\begin{packeditemize}
\item What are the requirements of an unbiased evaluation of QoE customization schemes' effectiveness?~(\S\ref{subsec:requirement})

\item What are the design choices to fulfill the requirements?~(\S\ref{sec:design_choices})

\item How do we implement those design choices and deploy them to the users?(\S\ref{sec:impl})
\end{packeditemize}

\tightsubsection{Design Requirement}
\label{subsec:requirement}
We need \name to conduct an unbiased comparison between the schemes and make it easily scale to new users.

\mypara{Unbiased comparison}
An unbiased comparison requires \name to test different QoE customization schemes under the same video content and viewing context (\eg viewing device, player display size, etc.~\cite{zhu2018measuring}) that should be as similar as possible to that of the users' everyday lives.
Previous studies~\cite{zhu2015understanding, gao2020personalized,kara2015your} show that the context factors can greatly impact the user's QoE preferences, and thus a QoE customization scheme's effectiveness could vary significantly under different contexts.
For example, a lower QoE sensitivity to bitrate would happen to some users when the videos are played on a low-resolution TV rather than a high-resolution one~\cite{zhu2015understanding}.
For such users, if the test is conducted on a high-
resolution TV, it will favor those QoE customization
schemes that focus on modeling the preferences on high-resolution devices, which causes a bias if the users usually watch videos on low-resolution devices.

\mypara{Minimal intervention in viewing experience}
Minimizing the intervention indicates that real human users need minimal amount of time to complete our test, and thus minimizing the monetary cost for the test.
The cost is important to \name, because we cannot simply assume a new user’s QoE preference can match those of some existing users, so we have to regularly model a new user's QoE preference when the user starts to use the video streaming service.


\tightsubsection{Design Choices}
\label{sec:design_choices}

Although there is no standardized methodology to satisfy the above-mentioned requirements, we carefully select a set of design choices in \name to make sure each scheme to be tested under the similar contexts with minimal user efforts.

\mypara{In-situ study rather than lab-based study and historical data analysis}
\name uses an in-situ ({\em a.k.a.,} in-the-wild) user study~\cite{rogers2017research} to minimize the viewing context difference between our test and the users' everyday lives.
\name does not control when \& what users watch, and thus it is more likely to reveal the user experience in natural environments compared with a lab-based study where the users are gathered in the lab and required to watch the same set of curated videos in the same physical place~\cite{duanmu2016sqi, duanmu2017qoe,duanmu2018quality,duanmu2019sqoe4,bampis2018towards}.
Lab-based user study is suitable for the case where we need to find out the common points of QoE preferences across the users under the same setting of context factors.
Although lab-based study strictly ensures the comparison fairness between different schemes, it fails to simulate the real-world environment, which hampers the ecological validity of the results, because the users have different preferences across context factors (\eg bitrate sensitivity on low- and high-resolution viewing devices).
Also, its cost is prohibitive if we deploy the study on every new user who might have different quality preferences from the existing users.
One might argue that user study might not be necessary, since we can do offline data analysis --- for a video quality pattern curated by a scheme, we can search existing users' viewing history for similar patterns with similar QoE feedback to the new user's.
However, we might not always find out such a pattern, because we cannot assume there is an existing user who has a very similar QoE preference and viewing environment to the new user.


\mypara{Video session-level randomization}
Video session-level randomization can make sure every scheme is tested under a similar distribution of video content and viewing context.
In an in-situ study, the main problem is that we cannot directly control the viewing context so the results might be biased by testing the schemes under different contexts.
To mitigate this problem, we use a randomized A/B test, \ie randomly determining which scheme to use when each video session begins, making \name agnostic to those schemes.


\mypara{User engagement vs. User rating}
There are two popular QoE metrics: user rating~\cite{itu1999subjective} and user engagement~\cite{balachandran2012quest, dobrian2011understanding}.
\name chooses user engagement, \ie the percentage of a video viewed by a user~\cite{dobrian2011understanding}.
This metric is widely used in the industry, not only because of its minimal intervention in user viewing experience (\ie users do not need to take time to feedback on their QoE by an exit survey), but also the direct relation to the revenue.
A natural concern regarding this setting is whether user engagement from arbitrary video content is reliable enough to model per-user QoE. 
In our study, the selection of video quality levels is totally agnostic to video content.
Thus, averaging over a sufficient amount of data can still reliably build per-user QoE models.
User rating is collected by an exit survey after each video session ends.
It is widely used in the lab-based study where the users are paid for providing ratings, while in the in-situ study, the users are likely to skip the survey, which might cause the insufficiency of user QoE feedback collection.
It also involves a lot of user efforts of providing their feedback, which significantly increases the cost of conducting the user study.


\mypara{Using bandwidth to control video quality}
\name uses bandwidth as a knob to indirectly control video quality.
Its benefit is that we do not need to directly modify the commercial player's ABR logic which is usually not open-sourced like YouTube and Netflix. 
Although we still need to predict the ABR logic's reaction to different bandwidth settings, it is doable. 
Because the ABR logic itself is designed to adapt to the network bandwidth for maximizing user QoE, though the players differ in the adaptation speed~\cite{licciardello2020understanding}.
This assumption is agreed by the reverse engineering work for ABR logic~\cite{gruner2020reconstructing, mondal2017candid}.

One concern is that we cannot {\em accurately} control when and what the video quality changes in a video session because the video player usually needs an uncertain amount of time to adapt to the changed bandwidth.
In~\S\ref{sec:eval}, we show that 16.7 seconds is the medium delay between when bandwidth changes and when the video player reacts.
If you use a QoE model taking the quality of long video segments as input (\eg usually >1 minute in \name), it causes minor affects on QoE model training.
However, there is still a chance that the player fails to adapt to the bandwidth we set.
To mitigate the problem, we need to consider the probability of getting the undesired quality when scheduling the video quality pattern.
We will describe it later in \S\ref{sec:impl}

% There are three types of experimenters that want to evaluate the QoE modeling schemes:
% \begin{packeditemize}
% \item {\bf Network service providers} control the bottleneck link of the video streaming system, and thus they concern how to use limited bandwidth resource to support more users without degrading user QoE.
% They usually optimize the user QoE by the insights found from the historical data~\cite{?} which might be biased for new users.

% \item {\bf Researchers} need to find out the difference between different schemes, so that they usually choose a lab-based user study in a fully-controlled environment (including video content and viewing context).
% The results might not reflect the condition in real life, and the cost is expensive.

% \item {\bf Video player providers} design ABR logic to optimize iser QoE under restricted bandwidth. 
% They usually conduct lab-based user study or historical data analysis to create QoE models~\cite{?}, and it is hard to extend to new users.
% \end{packeditemize}

\mypara{Potential experimenters}
\name is suitable for network service providers who control the bottleneck links, such as ISPs, CDNs, and edge routers.
The network service providers do not have the access to the video player’s logic but can monitor and control the users’ network connection. 
Network providers can use existing techniques to infer video quality by the video streaming traffic~\cite{bronzino2019inferring} with up to 91\% accuracy, and use the session time of the video stream as the user engagement. 

\tightsubsection{Implementation}
\label{sec:impl}

Although \name is suitable for the network service providers, we have the following limitations that hinder us to deploy \name as the network service providers do:
\begin{packeditemize}
\item We cannot find new users to test the QoE customization schemes as easily as the network providers.

\item We cannot freely control (\ie increase or decrease) the physical network bandwidth of the users.
\end{packeditemize}
To mitigate those limitations, we will discuss \name's implementation details to make \name's results equivalent to those at network service providers.


\mypara{Crowdsourcing user study}
We recruit the participants as ``new users" for \name's in-situ user study from crowdsourcing platforms (\eg Prolific~\cite{prolificlink} and Amazon MTurk~\cite{mturklink}) which can provide large demographic diversity~\cite{varvello2016eyeorg} across the participants. 
We first published a filtering survey for pre-screening the users.
The eligible users should experience video quality issues frequently, indicating that video quality is a significant factor in user QoE.
To avoid the random feedback in the survey, we write a video quality monitor (will describe soon) installed on the participants' browsers to confirm their feedback.
In~\S\ref{sec:eval}, we selected participants who used video streaming services $\geq 10$ hours per week and suffered from quality issues $\geq$20 times per week on YouTube for QoE customization scheme testing.

\mypara{Monitoring video quality}
We wrote a browser extension that can monitor buffer size, video quality, user engagement.
It also monitors the context factors, including player display size (\ie the width and the length of the player in pixel), viewing device, and active status  (\ie the player is the active application in the operating system, indicating whether the user is watching the video.), to ensure every scheme is evaluated under the same context.
More implementation details of the browser extension are in Appendix~\ref{sec:impl:plugin:monitor}

\mypara{Bandwidth throttling}
We wrote a browser extension to affect video quality by throttling video downloading throughput, since we cannot freely increase the physical bandwidth as network providers do. 
Although we need to maintain the average throughput of a video session to have complied with to the user’s internet plan, the QoE customization schemes might need the flexibility to increase and/or decrease the downloading throughput within a session for affecting the video quality. 
Particularly, to enable this flexibility, we make a comprise of using a $\alpha$\% throughput capping, \ie to maintain the average bandwidth of each session as $\alpha$\% of the full bandwidth (we use $\alpha=60$ in our study). 
Although the video sessions might have different full bandwidths, the video session-level randomization ensures that different schemes have a similar distribution of their session bandwidths.
The detailed implementation is described in Appendix~\ref{sec:impl:plugin:bw}.

\mypara{Realizing the video quality desired by QoE customization schemes}
Since the bandwidth knob cannot accurately control the video quality, \name needs to consider the probability of getting the undesired video quality.
Instead of a concrete quality pattern $v_i$, we can target a bandwidth allocation schedule $b_i$ (\ie bandwidth for users over time) that can maximize the {\em expected} importance ($IMPT$, will describe in \S\ref{sec:short_modeling}) of the perceived video quality pattern:
\begin{align}
  \max &\  \sum_{v_i}p\left(b_i, v_i\right)*IMPT(v_i), \label{eq:bw_regret}\\
  \text{s.t.}& \quad BWUsage(b_i)\leq BWLimit,
\end{align}
where $p(b,v)$ is the probability that the video quality pattern $v$ appears under the rate-limiting schedule $b$, and $BWLimit$ is the pre-determined maximum average bandwidth per session (\eg this can be based on the Internet plan subscribed by the user), and $BWUsage(v_i)$ is calculated by dividing the sum of bitrates of expected watched chunks by the predicted viewing time (\ie user engagement).

Although we might not understand every detail of a commercial player's ABR algorithm, a number of previous ABR reverse engineering works~\cite{gruner2020reconstructing, mondal2017candid} proves that the feasibility of profiling the player's behavior $p(b,v)$ which is the probability that the video quality pattern $v$ appears under a bandwidth allocation schedule $b$, \ie the bandwidth allocated to the video session over time.
To obtain $p(b, v)$, we run an exhaustive test to build the transition distribution of $D(s_1, s_2, b)$, where $s_1$ and $s_2$ represents the player states, including current bitrate, buffer length, and $b$ is the current bandwidth.
To obtain the transition probability between $s_1, s_2$ under bandwidth $b$ within 16.7 seconds (\ie the empirically medium delay between when bandwidth changes and when the video player reacts), we set the player state to $s_1$ under bandwidth $b_1$ for 100 times, and $D(s_1, s_2, b)$ is the times of the states becoming $s_2$ divided by 100.
To reduce the search space, we bucketize the bitrate, buffer length and bandwidth for every 200Kbps, 1 second and 200Kbps respectively.


==> short_intro.tex <==
\tightsection{Introduction}
\label{sec:intro}

% Video streaming system and QoE modeling background

Video streaming systems strive to maximize user-perceived quality of experience (QoE) within the constraints imposed by limited network resources.
Prior QoE optimization work are based on {\em QoE models} that characterize relationships between QoE and common video quality metrics (\eg video bitrate, rebuffering time).
Given these relationships, existing systems seek to optimize QoE by improving the underlying quality metrics.
Traditionally, the QoE models leverage general features, such as  viewing context factors (\eg devices, room brightness) and video content (\eg sports, news).
For each combination of these generic features, a QoE model is usually developed {\em offline} (via user study~\cite{zhang2021sensei, duanmu2019knowledge} or analysis of historical data~\cite{gao2020personalized}) and then applied to users.

% Personalizing user video experience can greatly benefit video streaming

However, these traditional QoE models fail to capture the differences among {\em individual} users.
Indeed, the literature has shown that in terms of how quality affects QoE, there is substantial heterogeneity across users.
As~\cite{duanmu2020assessing} shows, the users could have >20\% tolerance to the same video quality drop (\eg rebuffering) on average.
Moreover, different users are more sensitive to different aspects of video quality.

% Missing parts in previous work. Previous works show the QoE improvement given per-user QoE model, and build per-user QoE models.

Although recent efforts have studied the schemes of building per-user QoE models~\cite{?}, the missing part is {\em how to evaluate the effectiveness of those schemes in the real world of a new user}.
In prior work~\cite{??}, offline lab-based user study and historical data analysis are usually used for QoE model evaluation, but their results might be biased.
In lab-based study, the users are asked to watch the videos with manually content and quality issues determined by the modeling schemes, and then provide their QoE feedback in a highly-controlled environment.
The bias can be caused by the significant difference in the context factors between the real-world and the controlled environments.
For example, if a lab-based study uses high-resolution TVs to play videos, it would favor a scheme that emphasizes on modeling the user preference on video resolution, and thus the results are biased if the new user only views video on low-resolution devices.
In data analysis, a common approach is to simulate the case where a modeling scheme is supposed to be applied to new users by searching historical data.
The bias of the simulation comes from an inexplicit assumption: \ie the data from existing users contains the QoE preference of a new user, which is apparently not true~\cite{bartulovic2017biases}.


In this paper, we propose \name, a platform to evaluate QoE modeling schemes by in-situ ({\em a.k.a.}, in-the-wild) user study, where the users can watch any video content at any time on their own devices in their every-life environment.
To ensure an unbiased evaluation, before a video session \name randomly determines which QoE modeling scheme to use, making sure every scheme has a similar distribution of viewing context and video content.
\name controls bandwidth, and thus flow throughput, during a video session, to dynamically adjust the video quality according to the evaluated QoE modeling scheme.
This design spares us from modifying the bitrate adaptation algorithms (ABR) on the video player, considering that the ABR algorithms on most commercial players (\eg YouTube, Netflix) are not open-sourced.

A practical challenge facing \name is that, due to the proprietary nature of the video player, changing bandwidth at the bottleneck link may induce different player actions and user-perceived quality, when \name realizes a video quality pattern desired by the QoE modeling scheme. 
For instance, if \name needs to measure a user’s QoE when the resolution drops from 1080p to 360p, it will lower the available bandwidth, but as a result, player may either drop the resolution from 1080p to 360p, or continue playing at 1080p but experience a rebuffering event instead. 
To address this issue, we change our goal from determining a specific video quality pattern that maximizes its ``importance" (\eg how much information this pattern can contribute to QoE modeling), to dynamically creating a bandwidth schedule that can minimize the expected importance over a distribution of possible video quality resulting from the chosen bandwidth schedule.

Next, we use \name to evaluate the effectiveness of two conventional and one proposed QoE modeling schemes on real human users to show the potential of leveraging the across-user heterogeneity in real world. 
The first scheme~\cite{?} is to passively measure user QoE under their natural video quality, \ie show the videos without deliberately adding quality issues. 
This scheme might take a long time to accumulate enough samples to learn an accurate per-user QoE model. 
The second scheme~\cite{?} is to select the quality for a small number of videos such that their QoE feedback will maximally increase the accuracy of the per-user QoE model after a small number of sessions. 
This approach does reduce the number of QoE samples, but users might experience low QoE during the process; after all, the QoE samples that are more informative to QoE modeling tend to have lower quality.
To address the above disadvantages, we propose the third solution that can balance the training videos’ QoE and user feedback to contribute to its individualized QoE model training, \ie maximizing the sum of a video session's QoE and QoE modeling contribution (\eg uncertainty~\cite{settles2009active,lewis1994} in active learning). 

This paper presents two main contributions:
\begin{packeditemize}
\item We articulate the need of an evaluation platform that evaluates the effectiveness of per-user QoE modeling schemes in an unbiased manner, and then implement \name for realizing this idea.

\item We evaluate two conventional and one proposed QoE modeling schemes on \name. In an evaluation of 15 users on \name, we show that if considering the QoE preference heterogeneity, we can improve the QoE by XXX-21.6\% while maintaining the same bandwidth usage, or maintain the same QoE while using XXX-21.2\% less bandwidth.
\end{packeditemize}


==> short_intro_v2.tex <==
\tightsection{Introduction}
\label{sec:intro}

% Video streaming system and QoE modeling background
Video streaming systems strive to maximize user-perceived quality of experience (QoE) within the constraints imposed by limited network resources.
Prior QoE optimization work are based on {\em QoE models} that characterize relationships between QoE and common video quality metrics (\eg video bitrate, rebuffering time).
Given these relationships, existing systems seek to optimize QoE by improving the underlying quality metrics.
Traditionally, the QoE models leverage general features, such as viewing context factors (\eg devices, room brightness) and video content (\eg sports, news).
For each combination of these generic features, a QoE model is usually developed {\em offline} (via user study~\cite{zhang2021sensei, duanmu2019knowledge} or analysis of historical data~\cite{gao2020personalized}) and then applied to all users.

% Personalizing user video experience can greatly benefit video streaming
Recently, a new dimension of heterogeneity --- the differences among individual users --- has been used for video QoE optimization~\cite{huo2020meta}.
In terms of how quality affects QoE, there is substantial heterogeneity across users.
As~\cite{duanmu2020assessing} shows, the bottom 20\% of users have >20\% tolerance than the top 10\% of users to the same video quality drop (\eg rebuffering) on average.
Moreover, different users are more sensitive to different aspects of video quality.

% Missing parts in previous work. Previous works show the QoE improvement given per-user QoE model, and build per-user QoE models.

Although previous efforts~\cite{gao2020personalized,chang2018active,menkovski2010online} have explored the schemes of modeling the quality preferences for individual users, they do not address {\em how to evaluate the effectiveness of those modeling schemes on new users}.
Conventional methods conduct lab-based user studies or analyze the viewing history to collect the videos' QoE feedback.
The quality of those videos is curated for either eliciting user preference by a modeling scheme or QoE optimization by exploiting the learned preference.
The conventional methods are problematic if we extend them to new users.
Lab-based study is expensive and thus cannot apply to all new users, while viewing history analysis cannot apply to a new user without any historical data.
If we use existing users' QoE feedback to evaluate those schemes, the results are biased due to an inexplicit assumption: \ie the data from existing users contains the QoE preference of a new user, which is apparently not true~\cite{bartulovic2017biases}.
One may argue that some tools~\cite{casas2013youqmon, staehle2010yomo, nam2014youslow} can collect and then analyze new users' QoE feedback, but they cannot adjust the video quality for either preference modeling or QoE optimization.


To address this problem, we propose \name, a platform to evaluate per-user QoE modeling schemes in an unbiased fashion.
\name controls the available bandwidth, during a video session, to dynamically adjust the video quality according to the evaluated QoE modeling scheme.
Particularly, \name evaluates the modeling schemes under users' naturalistic environment, \ie no control over when \& what user watch.
Before a video session \name randomly determines which QoE modeling scheme to evaluate, making sure every scheme has a similar distribution of viewing context and video content to avoid bias.


Next, we use \name to evaluate the effectiveness of two conventional and one proposed QoE modeling schemes on real human users.
An effective QoE modeling scheme should 1) fast learn per-user QoE model with minimal negative impact on user QoE, and 2) be accurate enough for QoE optimization.
The first scheme~\cite{menkovski2010online} is to passively measure user QoE under their natural video quality, \ie show the videos without deliberately adding quality issues to elicit user preferences. 
This scheme might take a long time to accumulate enough samples to learn an accurate per-user QoE model. 
The second scheme~\cite{chang2018active} is to select the quality for a small number of videos such that their QoE feedback will maximally increase the accuracy of the per-user QoE model after a small number of sessions. 
This approach does reduce the number of QoE samples, but users might experience low QoE during the process; after all, the QoE samples that are more informative to QoE modeling tend to have lower quality.
To address the above disadvantages, we propose the third solution that can balance the training videos’ QoE and user feedback to contribute to its individualized QoE model training, \ie maximizing the sum of a video session's QoE and QoE modeling contribution (\eg uncertainty~\cite{settles2009active,lewis1994} in active learning). 

This paper presents two main contributions:
\begin{packeditemize}
\item We articulate the need of an evaluation platform that evaluates the effectiveness of per-user QoE modeling schemes in an unbiased manner, and then implement \name for realizing this idea.

\item We evaluate two conventional and one proposed QoE modeling schemes on \name. In an evaluation of 15 users on \name, we show that if considering the QoE preference heterogeneity, we can improve the QoE by XXX-21.6\% while maintaining the same bandwidth usage, or maintain the same QoE while using XXX-21.2\% less bandwidth.
\end{packeditemize}


==> short_intro_v3.tex <==
\tightsection{Introduction}
\label{sec:intro}

% Video streaming system and QoE modeling background
Video streaming systems strive to maximize user-perceived quality of experience (QoE) within the constraints imposed by limited network resources.
Prior QoE optimization work are based on {\em QoE models} that characterize relationships between QoE and common video quality metrics (\eg video bitrate, rebuffering time).
Given these relationships, existing systems seek to optimize QoE by improving the underlying quality metrics.
Traditionally, the QoE models group user's QoE preferences based on coarse-grained features, such as viewing context factors (\eg devices, room brightness) and video content (\eg sports, news).
For each combination of these generic features, a QoE model is usually developed {\em offline} (via user study~\cite{zhang2021sensei, duanmu2019knowledge} or analysis of historical data~\cite{gao2020personalized}) and then applied to all users.

% Personalizing user video experience can greatly benefit video streaming

Recently, a new dimension of heterogeneity --- the differences among {\em individual} users' quality preferences --- has been studied for video QoE optimization~\cite{huo2020meta, duanmu2020assessing}.
In terms of how quality affects QoE, there is substantial heterogeneity across users.
As~\cite{duanmu2020assessing} shows, the bottom 20\% of users have >20\% tolerance than the top 10\% of users to the same video quality drop (\eg rebuffering) on average.
Moreover, different users are more sensitive to different aspects of video quality.

To exploit this user heterogeneity, previous efforts of QoE customization schemes have tackled two questions.
(1) How to efficiently build QoE models using {\em offline} user studies and data analysis. 
A common approach is to let recruited participants first watch videos (often identical content) with manually selected quality issues by the schemes and then collects user feedback to learn the per-user QoE models~\cite{zhang2021sensei,duanmu2016sqi,duanmu2019knowledge}. 
(2) How to leverage {\em known} heterogeneity among different users' video quality preferences to optimize QoE on an individual basis.
For example, client-side ABR logic~\cite{mao2017neural, yan2020learning, yin2015control,huo2020meta} can customize the video quality based on per-user QoE models, and bandwidth can be better allocated across users with heterogeneous QoE models~\cite{nathan2019end}.


% Missing parts in previous work. Previous works show the QoE improvement given per-user QoE model, and build per-user QoE models.

However, prior work does not address {\em how to test the effectiveness of QoE customization schemes on new users}.
The effectiveness of QoE customization scheme includes three aspects: (1) how fast the schemes can learn a per-user QoE model for a new user; (2) how much negative impact on video QoE the schemes have during model learning; and (3) how much QoE improvement we can get after leveraging the per-user QoE model.
Thus, to test those schemes, we need to interact with the video sessions to adjust video quality for either per-user QoE model training or QoE optimization, which the previous video QoE and quality monitors~\cite{staehle2010yomo, nam2014youslow} cannot achieve.
Conventional testing methods~\cite{duanmu2016sqi,duanmu2017qoe, duanmu2018quality,chang2018active} conduct lab-based user studies or analyze the viewing history, which cannot extend to the new users.
Lab-based study is expensive and thus cannot apply to all new users, while viewing history analysis cannot apply to a new user without any historical data.
For the above reasons, video streaming providers have not customized QoE optimization online based on each user's QoE preference, and the potential benefits of these academic efforts~\cite{gao2020personalized,mao2017neural, yan2020learning, yin2015control,nathan2019end,huo2020meta} are not realized. 

To address this problem, we present the design, implementation and early deployment of \name, a platform that enables network operators to test QoE customization schemes online.
After a new user joins, \name controls the available bandwidth, during every video session, to dynamically adjust the video quality according to the tested QoE customization scheme, since video player ABR algorithms are influenced by throughput history and thus predictable~\cite{licciardello2020understanding} (more discussions in~\S\ref{sec:framework}).
Particularly, \name tests the QoE customization schemes under users' naturalistic environment, \ie no control over when \& what user watch.
Before a video session \name randomly determines which scheme to test, making sure every scheme has a similar distribution of viewing context and video content to avoid bias.
In our early deployment, the users need to install a browser extension that monitors the YouTube player status (\eg video quality, user engagement) and dynamically controls a user’s video downloading rate. 


To showcase its practical value, we use \name to evaluate the effectiveness of three QoE customization schemes on real human users.
The first scheme~\cite{menkovski2010online} is to passively measure user QoE under their natural video quality, \ie show the videos without deliberately adding quality issues to elicit user preferences. 
This scheme might take a long time to accumulate enough samples to learn an accurate per-user QoE model. 
The second scheme~\cite{chang2018active} is to select the quality for a small number of videos such that their QoE feedback will maximally increase the accuracy of the per-user QoE model after a small number of sessions. 
This approach does reduce the number of QoE samples, but users might experience low QoE during the process; after all, the QoE samples that are more informative to QoE modeling tend to have lower quality.
To address the above disadvantages, we propose the third solution that can balance the training videos’ QoE and user feedback to contribute to its individualized QoE model training, \ie maximizing the sum of a video session's QoE and QoE modeling contribution (\eg measured by uncertainty~\cite{settles2009active,lewis1994} in active learning). 


From the results of case study, our insight is that QoE customization by individual user's quality preference is promising: In an evaluation of 15 users on \name, we show that if considering the QoE preference heterogeneity, we can improve the QoE by XXX-21.6\% while maintaining the same bandwidth usage, or maintain the same QoE while using XXX-21.2\% less bandwidth.



==> short_intro_v4.tex <==
\tightsection{Introduction}
\label{sec:intro}

% Video streaming system and QoE modeling background
Video streaming systems strive to maximize user-perceived quality of experience (QoE) under limited network resources.
Prior QoE optimization work is based on {\em QoE models} that characterize relationships between QoE and video quality metrics (\eg video bitrate, rebuffering time).
Traditional QoE models leverage the heterogeneity in the factors affecting QoE, such as viewing context factors (\eg devices, room brightness) and video content (\eg sports, news).
For each combination of these factors, a QoE model is usually developed {\em offline} (via user study~\cite{zhang2021sensei, duanmu2019knowledge} or analysis of video viewing history~\cite{gao2020personalized}) and then applied to new users.

% Personalizing user video experience can greatly benefit video streaming

Recent studies~\cite{huo2020meta, duanmu2020assessing} have shown a new source of heterogeneity: the differences among {\em individual} users' quality preferences.
Prior work~\cite{duanmu2020assessing} showed in a lab-based user study, the bottom 20\% of users have >20\% more tolerance than the top 10\% of users to the same video quality issue (\eg rebuffering) on average.
Moreover, different users are more sensitive to different aspects of video quality.

Previous efforts focus on video QoE customization to leverage this user heterogeneity in two aspects:
(1) How to build per-user QoE models using offline user studies.
A common approach solicits the recruited participants' QoE feedback on the same set of videos with a wide range of quality issues.
These quality issues are added by the QoE customization schemes to elicit the user preferences~\cite{zhang2021sensei,duanmu2016sqi,duanmu2019knowledge}. 
(2) How to leverage known per-user QoE models for video QoE optimization.
For instance, client-side ABR logic~\cite{gao2020personalized, mao2017neural, yan2020learning, yin2015control,huo2020meta} can customize the video quality based on per-user QoE models, and bandwidth can be better allocated across users with heterogeneous QoE models~\cite{nathan2019end}.

% Missing parts in previous work. Previous works show the QoE improvement given per-user QoE model, and build per-user QoE models.

However, network operators still have not realized those academic efforts because prior work does not address {\em how to test  the effectiveness of those QoE customization schemes online on 
new users}.
The QoE customization schemes need to adjust video quality and collect QoE feedback online, by which an effective scheme can quickly learn a new user's QoE preference as well as optimize video QoE as much as possible.
Unfortunately, conventional testing methods that conduct lab-based user studies~\cite{duanmu2016sqi,duanmu2017qoe, duanmu2018quality} or viewing history analysis ~\cite{chang2018active,staehle2010yomo, nam2014youslow} cannot do online tests on new users.
Further, lab-based studies are too expensive to deploy on all new users, while a new user may not have video viewing history or preferences that match previous study participants. 


To address this problem, we present the design, implementation, and early deployment of \name, a platform that enables online tests of QoE customization schemes on new users for network operators.
Usually, the operators need to compare different schemes on new users with different preferences.
The natural questions of conducting such a comparison in \name  includes (1) how to adjust online video quality curated by the QoE customization schemes; (2) how to make the comparison easily extended to new users; and (3) how to ensure an unbiased comparison.
We elaborate the answers in~\S\ref{sec:framework}.

To showcase its practical value, we use \name to test two natural strawman QoE customization schemes and one preliminary solution to the two schemes' shortcomings.
The first strawman scheme~\cite{menkovski2010online} is constantly leveraging the current per-user QoE model to optimize QoE, although it will update the QoE model after each video session.
This scheme might take a long time to accumulate enough samples to elicit the user preference, thus resulting in suboptimal QoE before obtaining an accurate QoE model. 
The second scheme~\cite{chang2018active} is to aggressively add quality issues to videos by active learning, accelerating per-user QoE model training.
This scheme tends to result in poor QoE during model training, but it is directly at odds with the operators’ goal to maximize QoE in each video session.
To address the above disadvantages, we propose a preliminary solution that can balance the training videos’ QoE and the per-user model training speed, \ie maximizing the sum of a video session's QoE and its contribution to QoE modeling (\eg measured by uncertainty~\cite{settles2009active,lewis1994} in the literature of active learning). 

A new insight comes from \name's test on these three QoE customization schemes: In an evaluation of 15 users under real-world settings, compared to two natural schemes we can further improve the QoE by 13.9\% while maintaining the same bandwidth usage, or maintain the same QoE while using 17.3\% less bandwidth.



==> short_motivation.tex <==
\tightsection{Motivation}
\label{sec:short_moti}

We motivate our work by showing great user heterogeneity how various video quality metrics affect user QoE on an opensource dataset~\cite{?}\footnote{This dataset includes the video quality ratings from $\sim 30$ users for 1,350 video sessions on difference devices (\eg HDTV, UHDTV) and video content (\eg sports, game). We also analyze more datasets, and the results are in Appendix~\ref{sec:extend_moti}.}.
Those findings inform the needs of per-user QoE modeling schemes.
\begin{figure}[t]
      \begin{subfigure}[t]{1.0\linewidth}
      \captionsetup{justification=centering}
         \includegraphics[width=1.0\linewidth]{graphs/motivation/sep_hetero_rebuf.pdf}
         \vspace{-1.7em}
        \caption{Sensitivity to rebuffering}
        \label{subfig:rebuf}
      \end{subfigure}
          \vfill
          \vspace{0.8em}
          \begin{subfigure}[t]{1.0\linewidth}
      \captionsetup{justification=centering}
         \includegraphics[width=1.0\linewidth]{graphs/motivation/sep_hetero_bitrate.pdf}
         \vspace{-1.7em}
        \caption{Sensitivity to low bitrate}
        \label{subfig:rebuf}
      \end{subfigure}
          \vfill
          \vspace{0.8em}
          \begin{subfigure}[t]{1.0\linewidth}
      \captionsetup{justification=centering}
         \includegraphics[width=1.0\linewidth]{graphs/motivation/sep_hetero_btsw.pdf}
         \vspace{-1.7em}
        \caption{Sensitivity to bitrate switch}
        \label{subfig:rebuf}
      \end{subfigure}
    \vfill
   \vspace{1em}
    \caption{There is a significant heterogeneity across users in terms of their sensitivity to a fixed low quality of 
    (a) a short rebuffering event of 0.3-0.5 seconds (in Waterloo and \name datasets) or 1.0 second (in Sensei videos), 
    (b) a fixed low average bitrate (200--500~Kbps lower than highest bitrate), and 
    (c) a bitrate switch (with a magnitude of 1--1.5~Mbps). 
    CDFs of QoE rating differences of different users in response to each quality issue in the Waterloo, Sensei, and \name datase. \xu{fix the figures: only keeps the results from waterloo dataset. throw others to the appendix}
}
\vspace{-0.2em}
    \label{fig:diff_react}
\end{figure}

We first show the user heterogeneity is consistently significant in terms of how sensitive QoE is to the quality metrics of video quality.
We calculate the average QoE difference $\Delta Q_{Buf}(i)$ due to a short rebuffering event $Buf$ (0.3--0.5 seconds) on user $i$ by the difference in average QoE between the two group:
\begin{align}
   \Delta Q_{Buf}(i) = \text{ }&AvgQoE(\text{user } i\text{'s videos} \text{ with }Buf) - \nonumber \\
   &AvgQoE(\text{user } i\text{'s videos} \text{ without }Buf).
    \label{eq:qoedrop}
\end{align}
Similarly, we define $\Delta Q_{lowbitrate}(i)$ and $\Delta Q_{bitrateswitch}(i)$ to be the impact of low bitrate of $200-500 Kbps$ and a bitrate switch of magnitude $1-1.5 Mbps$ on QoE of user $i$, respectively.
Figure~\ref{fig:diff_react} shows the distribution of $\Delta Q_{Buf}$, $\Delta Q_{lowbitrate}$, and $\Delta Q_{bitrateswitch}$ over the users in each dataset.
We see that top 33\% users on average are 67\% more sensitive to the same quality difference than the the bottom 33\% of users.

We also show that the magnitude of heterogeneity in video quality preferences across individual users is on par with other well-known factors such as video content and viewing devices.
We calculate the average QoE drops (Eq.~(\ref{eq:qoedrop})) due to the same short rebuffering event used in Figure~\ref{fig:diff_react} in each video content or each device (HDTV, UHDTV, smartphone), and then calculate the variance of these QoE drops across different videos or different devices. 
The standard deviations (normalized by mean) for the rebuffering event across individual users, across videos, and across devices are $0.33\pm 0.03$, $0.41\pm 0.03$, $0.34\pm 0.01$.
Similar results are for other quality issues, such as low bitrate and bitrate switch (See Appendix~\ref{sec:extend_moti} for more details).

\mypara{Summary}
The key takeaways from our analysis are:
\begin{packeditemize}
    \item There is always significant user heterogeneity, in terms of how each quality aspect (rebuffering, low bitrate, and bitrate switch) affect user QoE.

    \item The magnitude of heterogeneity in video quality preferences across individual users is on par with other well-known factors such as video content and viewing devices.
\end{packeditemize}


==> short_qoeprofiling.tex <==
\tightsection{Online QoE modeling schemes}

In this section, we first formulate the general problem of online QoE modeling and elaborate why existing techniques designed for different-yet-related purposes are not well-suited.
Then, we propose a concrete solution, \name, to realize online QoE modeling and optimization.

\tightsubsection{Performance requirement}
\label{sec:modeling:requirement}

We envision that per-user QoE modeling can be applied to all video streaming users for QoE optimization.
To enable this scalability, the schemes need to meet the four properties.
\begin{packeditemize}
    \item \textbf{P1}: It should finish QoE modeling within a small number of video sessions for optimizing each individual's QoE as early as possible.
    \item \textbf{P2}: It should provide high QoE while modeling per-user QoE, \ie one cannot model per-user QoE at the cost of user experience.
    \item \textbf{P3}: It should obtain per-user QoE models to be accurate enough for per-user optimization techniques to best leverage the heterogeneity across users.
\end{packeditemize}


\tightsubsection{Strawmen online modeling schemes}
\label{sec:modeling:baselines}

To address the shortcomings of offline QoE modeling, two seemingly natural designs emerge. 
Both rely on passive QoE measurements and update the per-user QoE model after each video session. 
They differ in whether they set video quality to maximally improve user QoE or maximally help QoE modeling.


\mypara{Greedy optimization using biased QoE models}
As more measurements from a user are collected to update the per-user QoE model, we can always optimize QoE by the latest per-user QoE model, under the assumption that the latest QoE model is accurate enough.
This is promising, because the QoE would gradually improve with a QoE model becoming more accurate.
The drawback, however, is that the QoE model may never be accurate enough to realize the full potential of per-user QoE optimization due to the quality bias of the sessions for training QoE model.
For instance,  rebuffering is less common than lower bitrate in YouTube, because YouTube player typically assumes that rebuffering has a greater impact on QoE than low bitrate, so it strives to minimize rebuffering~\cite{anorga2015youtube} by aggressively lowering bitrate whenever bandwidth drops.
This scheme might miss the opportunity to learn the QoE preference of the users who are not sensitive to rebuffering, and thus, it violates {\bf P4}. 


\mypara{Greedy profiling using active learning}
Another natural choice is to add quality issues to video sessions in a way that the user's QoE feedback will maximally reduce the uncertainty of the current QoE model.
Previous works~\cite{chang2018active} show that active learning (which shows users the video quality whose QoE the current model is most uncertain about) can be used to minimize the number of sessions (QoE samples) needed to build an accurate QoE model;
\eg it only needs $\sim$100 videos to get the per-user QoE model from scratch.
This method is not ideal either. 
Although we can train per-user QoE models quickly and start QoE optimization early, the videos in the training stage might require severely bad quality (\ie violating {\bf P3}), because the video quality patterns (\ie a video quality pattern is the quality of each chunk in the video session.) with the largest uncertainty in the QoE model are usually with bad video quality.
To accelerate per-user QoE modeling, the active learning-based methods tend to encapsulate multiple types of quality issues into one video, and the low video quality can cause tens of billions of dollars profit damage according to Conviva~\cite{convivadamage}.


\tightsubsection{Balancing Modeling Speed and QoE}

We propose \name that can maintain good QoE while fast training per-user QoE model to address the shortcomings of the baselines in~\S\ref{sec:modeling:baseline}:
\begin{align}
    \max& \quad\quad QoE(v_i)+Uncertainty(v_i), \label{eq:find_patter}\\
   \text{s.t.}&  \quad BandwidthUsage(v_i) < BandwidthLimit\label{eq:bt_limit},
\end{align}
$QoE(v_i)$ is the predicted QoE of the video quality pattern $v_i$ (will describe shortly), $Uncertainty(v_i)$ is the uncertainty contributed by $v_i$ under the context of active learning~\cite{?}, which indicate the training speed, the larger uncertainty per training video pattern, the faster speed of model training, the $BandwidthLimit$ is the pre-determined maximum average bandwidth per session (\eg this can be based on the Internet plan subscribed by the user), and $BandwidthUsage(v_i)$ is calculated by dividing the sum of bitrates of expected watched chunks (the ones within the predicted viewing time $QoE(v_i)*VideoLength$) by the predicted viewing time.


\mypara{Practical challenge}
We use the bandwidth knob to induce the video player to generate our desired $v_i$ by setting the bandwidth as the desired bitrate of the chunk we need to download.
However, we might not get the desired video quality for every chunk in $v_i$ due to this indirect control over video player.

To mitigate the problem, we need to consider the probability of getting the undesired quality.
Thus, instead of a specific quality pattern $v_i$, we target a bandwidth allocation scheme $b_i$ (bandwidth over time) that can maximize the {\em expected} QoE and uncertainty:
\begin{align}
  \max& \sum_{v_i}p\left(b_i, v_i\right)*[QoE\left(v_i\right)+Uncertainty\left(v_i\right)], \label{eq:bw_regret}\\
  \text{s.t.}& \quad BandwidthUsage(b_i)\leq BandwidthLimit,
\end{align}
where $p(b,v)$ is the probability that the video quality pattern $v$ appears under the rate-limiting scheme $b$, and $p(b,v)$ can be calculated by the player profile by going through all possible video quality patterns (will describe shortly).
We re-calculate $b_i$ multiple times within a video session for better QoE and uncertainty. 

Moreover, even if we get the undesired quality of a chunk, the negative affect is not significant.
There are two cases of a chunk not getting the expected quality.
The first case is that the chunk gets lower bitrate than the expected.
In this case, the actual bandwidth consumption is also smaller than the expected, resulting in worse QoE.
To mitigate this problem, \name would allocate more bandwidth for the following chunks to mitigate the QoE loss.
The second case is that the chunk has higher bitrate than expected.
Since the chunk consumes more bandwidth than its quota, the next chunks should pay for that, which creates more bandwidth fluctuations that can add uncertainty to $v_i$.


\tightsubsection{Implementation}
\mypara{QoE model and uncertainty}
We borrow the random-forest-based QoE model from~\cite{?}, which takes the video quality of the chunks as the input, and outputs the expected QoE.
To train faster, the initial QoE model is a one-size-fits-all model.
\name customizes feature selection and criteria at the nodes on each decision tree inside the forest.
To avoid the explosion of input due to the large number of video chunks, we divide the video into 20 parts whose quality is the QoE model input.
The output QoE is bucketized into 10 classes, and it is the class who gets the most votes from the decision trees inside the random forest.
We use smallest margin to calculate the uncertainty given an input.


\mypara{Player profile}
We can build this profile by the assumption shared with the works of ABR logic reverse engineering~\cite{?}: a player behavior is predictable to some extent, since it is designed to adapt to the network bandwidth for maximizing user QoE, though the players differ in the adaption speed~\cite{licciardello2020understanding}.
To obtain the player profile $p(b, v)$, we run an exhaustive test to build the transition distribution of $D(s_1, s_2, b)$, where $s_1$ and $s_2$ represents the player states, including current bitrate, buffer length, and $b$ is the current bandwidth.
To obtain the transition probability between $s_1, s_2$ under bandwidth $b$ within 12 seconds\footnote{We use 12 seconds because empirically it is the medium delay between when bandwidth changes and when the video player reacts.}, we set the player state to $s_1$ under bandwidth $b_1$ for 100 times, and $D(s_1, s_2, b)$ is the times of the states becoming $s_2$ divided by 100.
To reduce the search space, we bucketize the bitrate, buffer length and bandwidth for every 200Kbps, 1 second and 200Kbps respectively.


% \tightsubsection{Reducing controller compute overhead}
% \label{subsec:costsaving}
% To naively calculate the expected regret of a rate-limiting scheme (Eq.~(\ref{eq:bw_regret})), we need to enumerate all possible video quality patterns under this scheme, which can be prohibitively expensive.
% We reduce this overhead by two ideas that limit the number of patterns we need to enumerate.
% % \begin{itemize}

% First, we use a short look-ahead horizon, such that we do not need to enumerate all possible quality of the future chunks.
% For the later chunks, we assume the player will perfectly adapt to the bandwidth we set.
% In \name, the look-ahead horizon is 2, and in \S\ref{subsec:microbenchmark}, we will evaluate the impact of different look-ahead horizons on QoE improvement and compute overhead.

% Second, we coalesce multiple consecutive chunks as longer segments, so that the bandwidth scheme and quality patterns are determined over a handle of segments, rather than many more chunks. 
% For example, for a 60-second long video with 3-second chunk size, we need to enumerate 60/3=20 times, while if we consider 4 adjacent chunks as a whole, we only need to enumerate 60/(3*4) = 5 times, which saves more than 400\% computation cost.

==> short_qoeprofiling_v2.tex <==
\tightsection{Online QoE modeling schemes}

In this section, we first formulate the general problem of online QoE modeling, and then list three concrete solutions as the benchmarks.

\tightsubsection{Performance requirement}
\label{sec:modeling:requirement}

We envision that per-user QoE modeling can be applied to all video streaming users for QoE optimization.
To enable this scalability, the schemes need to meet the four properties.
\begin{packeditemize}
    \item \textbf{P1}: It should finish QoE modeling within a small number of video sessions for optimizing each individual's QoE as early as possible.
    \item \textbf{P2}: It should provide high QoE while modeling per-user QoE, \ie one cannot model per-user QoE at the cost of user experience.
    \item \textbf{P3}: It should obtain per-user QoE models to be accurate enough for per-user optimization techniques to best leverage the heterogeneity across users.
\end{packeditemize}

\tightsubsection{Online modeling schemes}
\label{sec:modeling:baselines}

We list three online QoE modeling schemes which differs in whether they set video quality to maximally improve user QoE or maximally help QoE modeling.


\mypara{Greedy optimization using biased QoE models (GreedyOPT)}
As more measurements from a user are collected to update the per-user QoE model, we can always optimize QoE by the latest per-user QoE model, under the assumption that the latest QoE model is accurate enough.
Mathematically, if we denote $QoE(v_i)$ as the predicted QoE\footnote{We also use a random-forest-based QoE model from~\cite{?}, which takes the video quality of the chunks as the input, and outputs the expected QoE.
To train faster, the initial QoE model is a one-size-fits-all model. We customizes feature selection and criteria at the nodes on each decision tree inside the forest.
To avoid the explosion of input due to the large number of video chunks, we divide the video into 20 parts whose quality is the QoE model input.
The output QoE is bucketized into 10 classes, and it is the class who gets the most votes from the decision trees inside the random forest.} (user engagement) of  video quality pattern $v_i$, for video session $i$ this scheme is to
\begin{align}
    \max& \quad GOAL_{GreedyOPT}(v_i)=QoE(v_i), \\
   \text{s.t.}&  \quad BandwidthUsage(v_i) < BandwidthLimit\label{eq:bt_limit},
\end{align}
where $BandwidthLimit$ is the pre-determined maximum average bandwidth per session (\eg this can be based on the Internet plan subscribed by the user), and $BandwidthUsage(v_i)$ is calculated by dividing the sum of bitrates of expected watched chunks (the ones within the predicted viewing time $QoE(v_i)*VideoLength$) by the predicted viewing time.

This is promising, because the QoE would gradually improve with a QoE model becoming more accurate. The drawback, however, is that the QoE model may never be (violating {\bf P1}) accurate enough to realize the full potential of per-user QoE optimization due to the quality bias of the sessions for training QoE model.
For instance,  rebuffering is less common than lower bitrate in YouTube, because YouTube player typically assumes that rebuffering has a greater impact on QoE than low bitrate, so it strives to minimize rebuffering~\cite{anorga2015youtube} by aggressively lowering bitrate whenever bandwidth drops.
This scheme might miss the opportunity to learn the QoE preference of the users who are not sensitive to rebuffering, and thus, it violates {\bf P3}. 


\mypara{Greedy profiling using active learning (GreedyPF)}
Another natural choice is to add quality issues to video sessions in a way that the user's QoE feedback will maximally accelerate QoE modeling, \ie for video session $i$, we want
\begin{align}
    \max& \quad GOAL_{GreedyPF}(v_i)=Uncertaity(v_i), \\
   \text{s.t.}&  \quad BandwidthUsage(v_i) < BandwidthLimit\label{eq:bt_limit},
\end{align}
where $Uncertainty(v_i)$ quantifies how much a data sample contributes to model training in the context of active learning~\cite{?}.
Previous works~\cite{chang2018active} show that such a scheme can be used to minimize the number of sessions (QoE samples) needed to build an accurate QoE model;
\eg it only needs $\sim$100 videos to get the per-user QoE model from scratch.

This method is not ideal either. 
Although we can train per-user QoE models quickly and start QoE optimization early, the videos in the training stage might require severely bad quality (\ie violating {\bf P2}), because the video quality patterns (\ie a video quality pattern is the quality of each chunk in the video session.) with the largest uncertainty in the QoE model are usually with bad video quality.
To accelerate per-user QoE modeling, the active learning-based methods tend to encapsulate multiple types of quality issues into one video, and the low video quality can cause tens of billions of dollars profit damage according to Conviva~\cite{convivadamage}.


\mypara{Balancing modeling speed and QoE (Balance)}
We propose a scheme that can maintain good QoE while fast training per-user QoE model to address the shortcomings of the above-mentioned schemes, \ie for every session $v_i$
\begin{align}
    \max& \quad GOAL_{Balance}(v_i) QoE(v_i)+Uncertainty(v_i), \label{eq:find_patter}\\
   \text{s.t.}&  \quad BandwidthUsage(v_i) < BandwidthLimit\label{eq:bt_limit}.
\end{align}

Another benefit of this scheme is that we do not need to explicit divide the QoE modeling and QoE optimizaition phases.
Because with more video sessions, the weight of uncertainty diminishes as we can focus more on optimizing user QoE.



\tightsubsection{Practical challenge}
We might not get the desired video quality for every chunk in $v_i$ due to the bandwidth knob's indirect control over video player.

To mitigate the problem, we need to consider the probability of getting the undesired quality.
Thus, instead of a specific quality pattern $v_i$, we target a bandwidth allocation scheme $b_i$ (bandwidth over time) that can maximize the {\em expected} optimization goal:
\begin{align}
  \max& \quad \sum_{v_i}p\left(b_i, v_i\right)*GOAL(v_i), \label{eq:bw_regret}\\
  \text{s.t.}& \quad BandwidthUsage(b_i)\leq BandwidthLimit,
\end{align}
where $p(b,v)$ is the probability that the video quality pattern $v$ appears under the rate-limiting scheme $b$ (introduced in \S~?).
We re-calculate $b_i$ multiple times within a video session if we fail to get the target quality in the middle of the video session. 

Moreover, even if we get the undesired quality of a chunk, the negative affect is not significant.
There are two cases of a chunk not getting the expected quality.
The first case is that the chunk gets lower bitrate than the expected.
In this case, the actual bandwidth consumption is also smaller than the expected, resulting in worse QoE.
To mitigate this problem, \name would allocate more bandwidth for the following chunks to mitigate the QoE loss.
The second case is that the chunk has higher bitrate than expected.
Since the chunk consumes more bandwidth than its quota, the next chunks should pay for that, which creates more bandwidth fluctuations that can add uncertainty to $v_i$.






==> short_qoeprofiling_v3.tex <==
\tightsection{Online QoE customization}
\label{sec:short_modeling}

% In this section, we first formulate the general problem of online QoE modeling, and then list two conventional and one proposed modeling algorithms.

% \tightsubsection{Performance requirement}
% \label{sec:modeling:requirement}

% We envision that per-user QoE modeling can be applied to all video streaming users for QoE optimization.
% To enable this scalability, the schemes need to meet the three properties.
% \begin{packeditemize}
%     \item \textbf{P1}: It should finish QoE modeling within a small number of video sessions for optimizing each individual's QoE as early as possible.
%     \item \textbf{P2}: It should provide high QoE while modeling per-user QoE, \ie one cannot model per-user QoE at the cost of user experience.
%     \item \textbf{P3}: It should obtain per-user QoE models to be accurate enough for per-user optimization techniques to best leverage the heterogeneity across users.
% \end{packeditemize}

% \tightsubsection{Online modeling schemes}
% \label{sec:modeling:baselines}

We first discuss two natural online QoE customization schemes which differ in whether they set the video quality to maximally improve user QoE or maximally help QoE modeling, and then propose our scheme that can balance the user QoE during modeling and the modeling speed.

\mypara{Greedy optimization using biased QoE models (GreedyOpt)}
As more QoE measurements from a user are collected to update the per-user QoE model, we can always optimize QoE by the latest per-user QoE model, under the assumption that the latest QoE model is accurate enough.
Mathematically, if we denote $QoE(v_i)$ as the predicted QoE\footnote{We use a random-forest-based QoE model from~\cite{chang2018active}, which takes the video quality of the chunks as the input, and outputs the expected QoE.
To train faster, the initial QoE model is a one-size-fits-all model. We customizes feature selection and criteria at the nodes on each decision tree inside the forest.
To avoid the explosion of input due to the large number of video chunks, we divide the video into 20 parts whose quality is the QoE model input.
The output QoE is bucketized into 10 classes, and it is the class who gets the most votes from the decision trees inside the random forest.} (\ie user engagement) of video quality pattern $v_i$, for video session $i$ we define $v_i$'s importance that we want to maximize as: 
\begin{align}
    \max IMPT_{GreedyOpt}(v_i)=QoE(v_i).
\end{align}

This is promising, because the QoE would gradually improve with a QoE model becoming more accurate. The drawback, however, is that the QoE model may never be accurate enough to realize the full potential of per-user QoE optimization due to the quality bias of the sessions for training QoE model.
For instance,  rebuffering is less common than lower bitrate in YouTube, because YouTube player typically assumes that rebuffering has a greater impact on QoE than low bitrate, so it strives to minimize rebuffering~\cite{anorga2015youtube} by aggressively lowering bitrate whenever bandwidth drops.
This scheme might miss the opportunity to learn the QoE preference of the users who are not sensitive to rebuffering. 


\mypara{Greedy profiling using active learning (GreedyPF)}
Another natural choice is to add quality issues to video sessions in a way that the user's QoE feedback will maximally accelerate QoE modeling, \ie for video session $i$, we want to maximize $v_i$'s importance as
\begin{align}
    \max IMPT_{GreedyPF}(v_i)=Uncertaity(v_i),
\end{align}
where $Uncertainty(v_i)$ quantifies how much a data sample contributes to model training in the context of active learning~\cite{settles2009active,lewis1994}.
Previous works~\cite{chang2018active} show that such a scheme can be used to minimize the number of sessions (QoE samples) needed to build an accurate QoE model;
\eg it only needs $\sim$100 videos to get the per-user QoE model from scratch.

This method is not ideal either. 
Although we can train per-user QoE models quickly and start QoE optimization early, the videos in the training stage might require severely bad quality, because the video quality patterns with the largest uncertainty in the QoE model are usually with bad video quality.
To accelerate per-user QoE modeling, the active learning-based methods tend to encapsulate multiple types of quality issues into one video, and the low video quality can cause tens of billions of dollars profit damage~\cite{convivadamage}.


\mypara{Balancing modeling speed and QoE (Balance)}
We propose a preliminary solution to the shortcomings of the above-mentioned schemes, by maximizing the sum of a video session's uncertainty and QoE, \ie for every session $v_i$ we want
\begin{align}
  \max IMPT_{Balance}(v_i) = QoE(v_i)+Uncertainty(v_i). \label{eq:find_patter}
\end{align}

Another benefit of this scheme is that we do not need to explicit divide the QoE modeling and QoE optimization stages.
Because with more video sessions, the weight of uncertainty diminishes as we can focus more on optimizing user QoE.










==> short_relatedwork.tex <==
\vspace{-0.5em}
\tightsection{Related Work}
\label{sec:short_relatedwork}

\mypara{QoE modeling}
Past work \cite{bampis2018towards,bampis2017qoe,dobrian2011understanding,duanmu2019sqoe4,duanmu2017qoe,duanmu2018quality,duanmu2016sqi,grafl2013representation,tobias2013youtube,tobias2011youtube,ma2019gmad,moorthy2012video,ni2011flicker,pastrana2004sporadic,qi2006effect,rehman2013perceptual,staelens2010assessing} has studied QoE influencing factors by which QoE models are built.
Zhang~{\em et al.}~\cite{zhang2021sensei} study the QoE impact caused by the video content, and Gao~{\em et al.}~ \cite{gao2020personalized} reveal that the context of video viewing (\eg room brightness, viewing devices) is also important to user QoE.
Wang~{\em et al.}~\cite{wang2016data} build the QoE models for the individual users regarding the differences in viewing devices and points of interest.

Recent work~\cite{huo2020meta, duanmu2020assessing} shows significant heterogeneity in QoE preferences across the users.
Duanmu~{\em et al.}~\cite{duanmu2020assessing} show the users could have >20\%  difference in tolerance to the same type of video quality drop (\eg rebuffering events, bitrate drop, and bitrate switch) on average.
Besides the type, users also react differently when a quality drop happens~\cite{duanmu2020assessing}.
We put a comprehensive analysis of user heterogeneity in Appendix~\ref{sec:extend_moti}.

To train and test QoE models, a popular method is to conduct a  lab-based user study~\cite{duanmu2016sqi, bampis2018towards} in which the users gather in the lab and usually need to fill out a survey to provide QoE feedback on the video quality during or after a video session.
To save the cost of user QoE feedback collection, the number of the video sessions for QoE modelings is minimized by clustering users~\cite{gao2020personalized} or active learning~\cite{chang2018active}.
Other than lab-based study, prior work also studied the platforms~\cite{yan2020learning, jimenez2019network} that can collect QoE feedback from remote users.
They usually build their own video streaming services and thus have full control over the video content and quality.

\mypara{QoE-driven video streaming systems}
Early QoE-driven video streaming systems~~\cite{gomez2013towards,jiang2012qoe,ganjam2015c3,liu2012case,chiariotti2016online,mao2017neural,mok2012qdash,spiteri2016bola,yin2015control} adopt a one-size-fits-all optimization criterion, regardless of the video source characteristics, video viewing context, and individual users' quality preferences.
These algorithms are typically optimized offline on a dedicated server and then distributed to the operating point where resource allocation is performed.
Further research efforts mine information about video content~\cite{de2016complexity,toni2015optimal}, device type~\cite{bentaleb2016sdndash,li2016VMAF,rehman2015ssimplus}, and connectivity~\cite{jiang2016cfa,jiang2017pytheas} to optimize QoE at a per-group granularity.
Only until recently does personalized QoE optimization become a hot research topic.
Huo~\textit{et al.}~\cite{huo2020meta} discover the heterogeneity of QoE, manifested as the difference in the viewers' sensitivity to video quality, rebuffering, and quality adaptation.
Building upon the insights, the authors developed a data-driven personalized QoE model and a meta-learning optimization scheme.
As a few individual ratings become available, an optimal adaptive bitrate rule can be quickly determined with respect to the customized QoE model.
An alternative approach~\cite{gao2020personalized,wang2016data} takes the user profile as the input feature to the resource allocation controller, effectively adapting to the individual characteristics at run time.






==> tech_outline.tex <==
\section{Design of \name}


\subsection{Problem formulation}
\begin{itemize}

\item objective: online per-user qoe modeling and optimization: minimum impact on quality (high quality and min sessions needed) during per-use profiling + sufficient information for per-user qoe optimization. (given an illustrative example: quality over time with an ``ideal'' line)
\item why not survey-based user study (many lab studies), offline data analytics (conviva, akamai). they can't be applied online for any new user.

\item we tackle this problem in a specific setting:
\begin{itemize}
    \item control knobs: bandwidth control vs. player instrumentation
    \item qoe feedback: user engagement (view time) vs. exit survey rating
    \item state monitoring: player states (bitrate, buffer, etc) vs. control what/when they watch.
\end{itemize}
\item why is it well-suited for a service provider (isp, cdn, edge router, etc) that manages the bottleneck link of a user? 
\item potential concerns: 
\begin{itemize}
    \item how to get video quality? it's actually not new for service providers to monitor video quality (ask Tarun)
    \item how can qoe be modeled without regarding the video content? p-test!
\end{itemize}

\item in this setting, we envision a bandwidth controller with two logical components:
\begin{itemize}
    \item define {\em quality pattern}: sequence of video quality during a video
    \item {\em quality scheduling}: schedule quality pattern for each session to which the qoe feedback can maximally help per-user qoe modeling while maintaining high qoe (assuming the selected quality can be applied directly to each player)
    \item {\em dynamic rate limiting} to implement the selected quality pattern during each session
\end{itemize}
\end{itemize}


\subsection{Why is per-user qoe modeling challenging?}

\begin{itemize}
\item to highlight the challenge, let's first consider two seemingly natural designs (inspired by prior work). for now, we assume direct control over the player to set any video quality.
\item passive qoe monitoring: what does it do? (explain it with the figure) why is it slow? what prior work has used it and why it makes sense for them but not us?
\item active learning-based quality scheduling: what does it do? (explain it with the figure) why is it fast? why is it damaging to qoe? what prior work has used it and why it makes sense for them but not us?
\end{itemize}

\subsection{How \name schedules video quality per session}

\begin{itemize}
\item the goal of \name's quality scheduler is to balance online qoe modeling (which requires showing suboptimal quality) and qoe optimization (showing ``best-effort'' quality all the time). put the two strawmen into context.
\item our insight is to cast the problem into the well-studied framework of regret-minimization. 
regret of a selected quality is the sum of (1) estimated qoe of current session and (2) uncertainty of the estimation.
why minimizing the regret solves our problem?
(is it exactly UCB1, if not why not)
\item formulate it mathematically.
define action, expected qoe, uncertainty.
where is certainty coming from
\item a feature of this approach is that it gradually starts optimization phase. if qoe modeling converges quickly, optimization starts early
\end{itemize}


\subsection{How \name dynamically limit rate during each session}

\begin{itemize}
\item in our setting, we don't assume direct control over player's quality pattern. instead, we limit throughput during the course of a session to indirectly control quality pattern.
\item following our earlier formulation, we model this indirection as another {\em source of uncertainty}
\item how to profile the player's behavior offline? enumerate the player status, log the choice, etc (simplify and also cite prior papers)
\url{https://www.usenix.org/conference/atc20/presentation/gruener}
\item then we plug in this new uncertainty in the regret minimization formulation: more math
\end{itemize}


\subsection{Reducing controller compute overhead}

\begin{itemize}
\item The overhead is caused by we need to enumerate the video quality in the future.
\item Reduce look-ahead horizon: reduce the number of chunks we need to enumerate.
\item Consider adjacent chunks as a whole: reduce the number of calculation we need to recalculate it bandwidth allocation.
\end{itemize}


\section{User Study Methodology and Deployment}

\subsection{User study methodology}

\begin{itemize}
\item How to test \name and its baselines in the wild? 
\begin{itemize}
    \item why it's hard: we don't control the actual network bottleneck link. instead, we do xxxx.
    \item how to fairly compare \name and baseline: 1. we ensure every session (when \name or other methods are used) uses $\alpha$ fraction of of its full bandwidth.
    2. a/b test (randomized, side-by-side, etc)
\end{itemize} 
\item recruitment of participants.
\item distribution of recruited participants, in terms of age, network plan, isp, throughput, etc
\end{itemize}

\subsection{Client-side browser plugin}
\begin{itemize}
\item high level: we only test \name when users watch youtube video. we strictly follow the setting in \S\ref{??}: no UI change. user is unaware. no information collected on video content
\item quality monitoring
\item dynamic rate limiting
\end{itemize}


